Millimeter Wave Analog Beamforming Codebooks Robust to Self-Interference

This paper develops a novel methodology for designing analog beamforming codebooks for full-duplex millimeter wave (mmWave) transceivers, the first such codebooks to the best of our knowledge. Our design reduces the self-interference coupled by transmit-receive beam pairs and simultaneously delivers high beamforming gain over desired coverage regions, allowing mmWave full-duplex systems to support beam alignment while minimizing self-interference. To do so, our methodology allows some variability in beamforming gain to strategically shape beams that reject self-interference while still having substantial gain. We present an algorithm for approximately solving our codebook design problem while accounting for the non-convexity posed by digitally-controlled phase shifters and attenuators. Numerical results suggest that our design can outperform or nearly match existing codebooks in sum spectral efficiency across a wide range of self-interference power levels. Results show that our design offers an extra 20-50 dB of robustness to self-interference, depending on hardware constraints.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> mathtype.tex <==
\usepackage{bm}

% Vectors
\def\vzero{{\vec{0}}}
\def\vone{{\vec{1}}}
\def\vmu{{\vec{\mu}}}
\def\vtheta{{\vec{\theta}}}
\def\va{{\vec{a}}}
\def\vb{{\vec{b}}}
\def\vc{{\vec{c}}}
\def\vd{{\vec{d}}}
\def\ve{{\vec{e}}}
\def\vf{{\vec{f}}}
\def\vg{{\vec{g}}}
\def\vh{{\vec{h}}}
\def\vi{{\vec{i}}}
\def\vj{{\vec{j}}}
\def\vk{{\vec{k}}}
\def\vl{{\vec{l}}}
\def\vm{{\vec{m}}}
\def\vn{{\vec{n}}}
\def\vo{{\vec{o}}}
\def\vp{{\vec{p}}}
\def\vq{{\vec{q}}}
\def\vr{{\vec{r}}}
\def\vs{{\vec{s}}}
\def\vt{{\vec{t}}}
\def\vu{{\vec{u}}}
\def\vv{{\vec{v}}}
\def\vw{{\vec{w}}}
\def\vx{{\vec{x}}}
\def\vy{{\vec{y}}}
\def\vz{{\vec{z}}}

% Matrix
\def\mA{{\mat{A}}}
\def\mB{{\mat{B}}}
\def\mC{{\mat{C}}}
\def\mD{{\mat{D}}}
\def\mE{{\mat{E}}}
\def\mF{{\mat{F}}}
\def\mG{{\mat{G}}}
\def\mH{{\mat{H}}}
\def\mI{{\mat{I}}}
\def\mJ{{\mat{J}}}
\def\mK{{\mat{K}}}
\def\mL{{\mat{L}}}
\def\mM{{\mat{M}}}
\def\mN{{\mat{N}}}
\def\mO{{\mat{O}}}
\def\mP{{\mat{P}}}
\def\mQ{{\mat{Q}}}
\def\mR{{\mat{R}}}
\def\mS{{\mat{S}}}
\def\mT{{\mat{T}}}
\def\mU{{\mat{U}}}
\def\mV{{\mat{V}}}
\def\mW{{\mat{W}}}
\def\mX{{\mat{X}}}
\def\mY{{\mat{Y}}}
\def\mZ{{\mat{Z}}}
\def\mBeta{{\mat{\beta}}}
\def\mPhi{{\mat{\Phi}}}
\def\mLambda{{\mat{\Lambda}}}
\def\mSigma{{\mat{\Sigma}}}

==> par-notation.tex <==
\subsection{Notation:}
We use the following notation and conventions. 
We use one-indexing unless otherwise specified.
We represent matrices with bold uppercase, $\mat{A}$. 
We represent column vectors with bold lowercase, $\vec{a}$. 
We represent sets with script lettering, $\set{A}$.
We represent scalars with standard lowercase, $a$, standard uppercase, $A$, and sometimes script lettering, $\mathcal{A}$, for important quantities.
We define $\j = \sqrt{-1}$.
% We use $(\cdot)$\trans, $(\cdot)$\ctrans, and \frobenius{\cdot} to represent matrix transpose, conjugate transpose, and Frobenius norm, respectively. 
We use $(\cdot)\trans$, $(\cdot)\ctrans$, and $(\cdot)\conj$ to represent matrix transpose, conjugate transpose, and conjugate, respectively.
We use $\normone{\cdot}$, $\normtwo{\cdot}$, $\norminf{\cdot}$, and $\normfro{\cdot}$ as the $\ell_{1}$, $\ell_{2}$, $\ell_{\infty}$, and Frobenius vector norms and induced matrix norms, respectively.
An induced matrix norm is defined as $\norm{\mat{A}} = \max_{\vec{x}} \norm{\mat{A}\vec{x}} / \norm{\vec{x}}$ where $\norm{\cdot}$ is some vector norm.
We use $\trace{\mat{A}}$, $\vectorize{\mat{A}}$, $\bars{\mat{A}}$, and $\ev{\cdot}$ to represent the trace of \mat{A}, the column vectorization of \mat{A}, the determinant of \mat{A}, and expectation, respectively. 
We overload $\diag{\mat{A}}$ and $\diag{\vec{a}}$ to represent a vector of the main diagonal elements of $\mat{A}$ and a square diagonal matrix with the elements of \vec{a} on the main diagonal, respectively; by this convention, $\diag{\diag{\mA}}$ represents a diagonal matrix whose diagonal elements are the diagonal elements of $\mA$.
We use $\kron$ to represent the Kronecker product.
We use $\card{\set{A}}$ to represent the cardinality of a set $\set{A}$.
We use $\svmax{\mA}$ and $\evmax{\mA}$ to denote the maximum singular value and maximum eigenvalue of \mat{A}, respectively.
We use $\left[\mat{A}\right]_{i,j}$ to denote the element in the $i$th row and $j$th column of \mat{A}. 
We use $\left[\mat{A}\right]_{i,:}$ and $\left[\mat{A}\right]_{:,j}$ to denote the $i$th row and $j$th column of \mat{A}, respectively. 
We use $\mI$ as an identity matrix.
% We use $(\cdot)\todB$ to represent a quantity in unit of \gls{db}. 
We use $\todB{x} = 10 \log_{10}(x)$ to represent $x$ in units of \glspl{db}.
We use $\todBm{x}$ to represent $x$ in units of \glspl{dbm}.
We use $\complexpow{m}{n}$ to represent the set of all $m\times n$ matrices with complex entries.
% Finally, we use \eyevec{N} to denote an $N$-element column vector of ones and \eyemat{N} to denote an $N \times N$ identity matrix.
We use $\cgauss{\vec{m}}{\mat{R}}$ as a multivariate circularly symmetric complex Normal distribution with mean $\vec{m}$ and covariance matrix $\mat{R}$.
We often use set-builder notation when defining sets.
We use $\binom{n}{k} = \frac{n!}{k!(n-k)!}$ to denote the $n$-choose-$k$ binomial coefficient.
% We use $\land$ as a logical AND operation.
% We distinguish matrices and vectors in the time domain as $\mat{A},\vec{a}$ and in the frequency domain as $\matfd{A},\vecfd{a}$.
% We use the term ``beamformer'' most often to refer to a single column (rather than matrix) of beamforming weights.

==> sec-abstract.tex <==
\begin{abstract}

Beamforming codebooks are widely used by \mmwave transceivers, especially for analog beamforming, to configure highly directional beams with low complexity.
Such codebooks are particularly useful when the analog beamformer, which is implemented as a network of phase shifters and attenuators, is subject to its weights having quantized phase and amplitude---a practical constraint imposed by finite resolution phase shifters and attenuators.
Recent works have investigated beamforming-based solutions to achieve in-band full-duplex operation in \mmwave transceivers.
Finite resolution phase and amplitude control, however, make optimization of analog beamforming particularly challenging, leading many existing to designs to rely on beam-selection using conventional codebooks.
This is problematic because conventional codebooks, while highly directional in the far-field, are not necessarily robust in avoiding self-interference.
In this work, we present an analog codebook design methodology that creates a transmit and receive codebook pair that significantly reduces the interference coupled by all transmit-receive beam pairs while maintaining service over a coverage region.
We show that our codebook design, which accounts for finite resolution phase and amplitude control, can achieve orders of magnitude more isolation between all transmit-receive beam pairs while performing comparably to conventional codebooks in a half-duplex setting.

The goal of this design is not to produce codebooks that achieve necessarily \textit{high} amounts of isolation but rather \textit{better} isolation than conventional, off-the-shelf codebooks.
\end{abstract}

==> sec-contribution-i-old.tex <==
\section{Analog Beamforming Codebook Design with Perfect\\Self-Interference Channel Knowledge} \label{sec:contribution-i}

We now outline a codebook design methodology that reduces the self-interference that is coupled between transmit-receive beam pairs while also ensuring transmit beams and receive beams provide sufficient gain to a desired coverage region.
Furthermore, our design accounts for the hardware constraints imposed on beamforming weights due to finite resolution phase shifters and attenuators.
Note that our design does not require that attenuators be present, though it will improve from having such; we will evaluate both cases in our numerical results in \secref{sec:simulation-results}.

\subsection{Quantifying our Codebook Design Criteria}

In both hybrid beamforming and analog-only beamforming systems, the high beamforming gain necessary for wide area \mmwave communication is afforded by analog beamforming.
Therefore, it is essential that our analog beamforming codebook maintain high beamforming gain across a desired coverage region.

\begin{definition}[Transmit coverage region]
Let $\aodset$ be a set of $\Mt$ \glspl{aod} corresponding to the directions that our full-duplex device is interested in transmitting toward (i.e., transmit coverage region).
\begin{align}
	\aodset = \braces{\aod_i : i = 1, \dots, \Mt}
\end{align}
\end{definition}

\begin{definition}[Receive coverage region]
Similarly, let $\aoaset$ be a set of $\Mr$ \glspl{aoa} corresponding to the directions that our full-duplex device is interested in receiving from (i.e., receive coverage region).
\begin{align}
	\aoaset = \braces{\aoa_i : i = 1, \dots, \Mr}
\end{align}
\end{definition}

Let $\atx{\aod} \in \setvectorcomplex{\Nt}$ be the transmit array response vector in the direction of $\aod$, and let $\arx{\aoa} \in \setvectorcomplex{\Nr}$ be the receive array response vector in the direction of $\aoa$.
Let $\Atx$ be a matrix of transmit array response vectors evaluated at the \glspl{aod} in $\aodset$.
\begin{align}
\Atx = 
\begin{bmatrix}
\atx{\aod_1} & \atx{\aod_2} & \cdots & \atx{\aod_{\Mt}}
\end{bmatrix} \in \setmatrixcomplex{\Nt}{\Mt}
\end{align}
%\begin{align}
%\Atx = \blkdiag{\atx{\aod_1}, \atx{\aod_2}, \dots, \atx{\aod_{\Gt}}} \in \setmatrixcomplex{\Nt\Gt}{\Gt}
%\end{align}
Similarly, let $\Arx$ be a matrix of receive array response vectors evaluated at the \glspl{aoa} in $\aoaset$.
\begin{align}
\Arx = 
\begin{bmatrix}
\arx{\aoa_1} & \arx{\aoa_2} & \cdots & \arx{\aoa_{\Mr}}
\end{bmatrix} \in \setmatrixcomplex{\Nr}{\Mr}
\end{align}
%\begin{align}
%\Arx = \blkdiag{\arx{\aoa_1}, \arx{\aoa_2}, \dots, \arx{\aoa_{\Gr}}} \in \setmatrixcomplex{\Nr\Gr}{\Gr}
%\end{align}

Recall that we aim to design an analog precoding codebook $\prerfcbbar$ and an analog combining codebook $\comrfcbbar$.
To serve a device in the direction $\aod \in \aodset$, the transmitter will configure its analog precoder to the corresponding precoder in $\prerfcbbar$. 
Likewise, to serve a device in the direction $\aoa \in \aoaset$, the receiver will configure its analog combiner to the corresponding combiner in $\comrfcbbar$.

With this being said, let us define $\prerfcbbar$ and $\comrfcbbar$ as 
\begin{gather}
	\prerfcbbar = \braces{\vf_1, \dots, \vf_{\Mt}} \subset \prerfcb \\
	\comrfcbbar = \braces{\vw_1, \dots, \vw_{\Mr}} \subset \comrfcb
\end{gather}
where $\vf_\ell$ and $\vw_\ell$ are responsible for transmitting and receiving from $\aod_\ell \in \aodset$ and $\aoa_\ell \in \aoaset$, respectively.
Recall that $\prerfcbbar$ and $\comrfcbbar$ are subsets of the sets of all possible analog precoders $\prerfcb$ and combiners $\comrfcb$, respectively.
Using the entries in $\prerfcbbar$ and $\comrfcbbar$, let us build the analog precoding codebook matrix
\begin{align}
\precbmat = 
\begin{bmatrix}
\vf_1 & \vf_2 & \cdots & \vf_{\Mt}
\end{bmatrix} \in \setmatrixcomplex{\Nt}{\Mt}
\end{align}
and the analog combining codebook matrix
\begin{align}
\comcbmat = 
\begin{bmatrix}
\vw_1 & \vw_2 & \cdots & \vw_{\Mr}
\end{bmatrix} \in \setmatrixcomplex{\Nr}{\Mr}
\end{align}

A device not falling directly on the grid $\aodset$ or $\aoaset$ will be served by the beam that steers closest to it. \edit{Should I write this out explicitly using $\argmin$?}
A device not falling directly on the grid of angles in $\aodset$ or $\aoaset$ can be served by the beam that steers closest to it. Explicitly, a receiving device in the direction of $\aod$ or a transmitting device in the direction of $\aoa$ can be served by the $\ell\parens{\aod}$-th transmit beam or the $\ell\parens{\aoa}$-th receive beam, respectively, where
\begin{align}
\ell\parens{\aod} = \arg \min_{\ell} \bars{\aod - \aod_\ell} \\
\ell\parens{\aoa} = \arg \min_{\ell} \bars{\aoa - \aoa_\ell}
\end{align}


Recall that $\Hsi \in \setmatrixcomplex{\Nr}{\Nt}$ is the over-the-air self-interference channel matrix between the transmit and receive arrays of our full-duplex transceiver.
The coupling between the $m$-th analog precoder $\vf_{m}$ and $n$-th analog combiner $\vw_n$ is
\begin{align}
\vw_n\ctrans \times \Hsi \times \vf_{m} \in \setvectorcomplex{1}
\end{align}
Collecting the coupling between all analog precoding-combining pairs into a matrix $\mM$, we get
\begin{align}
\mM = \comcbmat\ctrans \Hsi \precbmat \in \setmatrixcomplex{\Mr}{\Mt}
\end{align}
where $\entry{\mM}{n,m} = \vw_n\ctrans \times \Hsi \times \vf_{m}$.

To reduce the average coupling across all analog precoding-combining pairs, our design aims to reduce the average energy of the matrix $\mM$.
That is, we aim to minimize $\powersi$
\begin{align}
\powersi = \frac{1}{\Mt\Mr} \cdot \normfro{\mM}^2 = \frac{1}{\Mt\Mr} \cdot \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:power-si}
\end{align}
As discussed, in doing so, our design must ensure that the beams remain useful in serving users in the coverage region; we now quantify this.

Let $\Gtxmax$ and $\Grxmax$ be the maximum linear transmit and receive amplitude gain
\begin{gather}
\Gtxmax = \normtwo{\atx{\aod}} = \Nt \\
\Grxmax = \normtwo{\arx{\aoa}} = \Nr
\end{gather}
which are achieved when $\vf_\ell = \atx{\aod}$ and $\vw_\ell = \arx{\aoa}$, respectively.
Let $\Gtxell$ be the linear transmit amplitude gain afforded by $\vf_\ell$ in the direction of $\aod_\ell$ and $\Grxell$ be the linear receive amplitude gain afforded by $\vw_\ell$ in the direction of $\aoa_\ell$, which can be written as
\begin{gather}
\Gtxell = \atx{\aod_\ell}\ctrans \times \vf_\ell \label{eq:Gtx} \\
\Grxell = \arx{\aoa_\ell}\ctrans \times \vw_\ell \label{eq:Grx}
\end{gather}
where it follows that
\begin{align}
\bars{\Gtxell} \leq \Gtxmax \\
\bars{\Grxell} \leq \Grxmax 
\end{align}

%\begin{definition}[Minimum required transmit and receive beamforming gain]
%	Let $\Gtxmin^2$ and $\Grxmin^2$ be the minimum transmit and receive beamforming power gain for any precoder or combiner, respectively, in the direction it intends to serve; that is to say that $\prerfcbbar$ and $\comrfcbbar$ are required to have beams that satisfy
%	\begin{align}
%		\Gtxell \geq \Gtxmin \ \forall \ \ell \in \braces{1,\dots,\Mt} \label{eq:coverage-constraint-tx} \\
%		\Grxell \geq \Grxmin \ \forall \ \ell \in \braces{1,\dots,\Mr} \label{eq:coverage-constraint-rx}
%	\end{align}
%\end{definition}

\begin{definition}[Target transmit and receive gain.]
	Let $\Gtxtgt$ and $\Grxtgt$ be target transmit and receive beamforming (amplitude) gains for any precoder or combiner, respectively, in the direction it intends to serve. that is to say that $\prerfcbbar$ and $\comrfcbbar$ are required to have beams that satisfy
	\begin{gather}
		\Gtxtgt \approx \Gtxell \ \forall \ \ell \in \braces{1,\dots,\Mt} \\
		\Grxtgt \approx \Grxell \ \forall \ \ell \in \braces{1,\dots,\Mr} 
	\end{gather}

	Let $\Gtxtgt$ and $\Grxtgt$ be defined more conveniently using $0 < \Deltatx \leq 1$ and $0 < \Deltarx \leq 1$ as follows.
	\begin{align}
	\Gtxtgt = \Deltatx \cdot \Gtxmax \\
	\Grxtgt = \Deltarx \cdot \Grxmax
	\end{align}
	where more convenient log-scale expressions are
	\begin{align}
	\todB{\Gtxtgt} = \todB{\Gtxmax} - \todB{\Deltatx} \\
	\todB{\Grxtgt} = \todB{\Grxmax} - \todB{\Deltarx}
	\end{align}
	where $\todB{\Deltatx} \leq 0$ and $\todB{\Deltarx} \leq 0$.
\end{definition}

\begin{definition}[Transmit and receive gain variance.]
	Let $\sigmatx^2 \geq 0$ be the maximum variance tolerated in achieving the target transmit gain $\Gtxtgt$ across beams in the transmit codebook $\prerfcbbar$, normalized to $\Gtxtgt^2$.
	\begin{align}
	\frac{1}{\Mt \cdot \Gtxtgt^2} \cdot \sum_{\ell=1}^{\Mt} \bars{\Gtxtgt - \Gtxell}^2 \leq \sigmatx^2 \label{eq:delta-tx}
	\end{align}
	Similarly, let $\sigmarx^2 \geq 0$ be the maximum variance tolerated in achieving the target receive gain $\Grxtgt$ across all beams in the receive codebook $\comrfcbbar$, normalized to $\Grxtgt^2$.
	\begin{align}
	\frac{1}{\Mr \cdot \Grxtgt^2} \cdot \sum_{\ell=1}^{\Mr} \bars{\Grxtgt - \Grxell}^2 \leq \sigmarx^2  \label{eq:delta-rx}
	\end{align}
\end{definition}


\subsection{Assembling our Codebook Design Problem}

Let $\gtxtgt$ and $\grxtgt$ be vectors containing the target transmit and receive gains at each entry.
\begin{align}
\gtxtgt = \Gtxtgt \cdot \onevec{\Mt} \label{eq:gtx} \\
\grxtgt = \Grxtgt \cdot \onevec{\Mr} \label{eq:grx}
\end{align}

Using this, we can formulate the following constraints on transmit and receive beamforming gain
\begin{align}
\normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:coverage-constraint-tx} \\
\normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:coverage-constraint-rx}
\end{align}
which we capture the coverage constraints of our two codebooks $\prerfcbbar$ and $\comrfcbbar$.

The parameters $\Gtxtgt$, $\Grxtgt$, $\Deltatx$, and $\Deltatx$ can be tuned as desired by system engineers as we will explore in our numerical results in \secref{sec:simulation-results}.
Convenient log-scale representations of $\sigmatx^2$ and $\sigmarx^2$ are 
\begin{align}
\todB{\sigmatx^2} = 10 \cdot \logten{\sigmatx^2} \\
\todB{\sigmatx^2} = 10 \cdot \logten{\sigmatx^2} 
\end{align}
where it practical to take $\todB{\sigmatx^2} \leq 0$ dB (i.e., $\sigmatx^2 \leq 1$) and $\todB{\sigmatx^2} \leq 0$ dB (i.e., $\sigmatx^2 \leq 1$).
Lower $\sigmatx^2$, $\sigmatx^2$ results in stricter constraints (less variance in achieving targets).

With the coverage constraints in hand, let us now formulate our problem as
\begin{subequations} \label{eq:problem-full-1}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:problem-objective-1} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-1} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-1} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-1} \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-1} 
	\end{align}
\end{subequations}

As we will see, permitting $\Gtxtgt$ and $\Grxtgt$ to be lower will relax the constraints of our design, allowing it to better reduce self-interference coupled by our transmit and receive beams; this helps facilitate full-duplexing service to two devices but degrades the service each device experiences.
Furthermore, increasing $\Deltatx$ and $\Deltarx$ will increase the flexibility of our design, but will lessen the coverage guarantee.
We examine this tradeoff in our numerical results in \secref{sec:simulation-results}.

%---
%
%\begin{theorem}
%The objective in problem \eqref{eq:problem-full-1} is convex in $\parens{\precbmat,\comcbmat}$.
%
%\begin{proof}
%\begin{align}
%\normfro{\lambda \comcbmat_1\ctrans \Hsi \lambda \precbmat_1}^2
%\end{align}
%\end{proof}
%\end{theorem}
%
%---



\subsection{Solving for our Codebook Design}
The objective \eqref{eq:problem-objective-1} is convex along with constraints \eqref{eq:problem-coverage-tx-1} and \eqref{eq:problem-coverage-rx-1}.
Constraints \eqref{eq:problem-quantize-tx-1} and \eqref{eq:problem-quantize-rx-1}, of course, are not due to the limited resolution of each phase shifter and attenuator.
Therefore, to solve \eqref{eq:problem-full-1}, we use a projection-based alternating minimization as follows.
% We split \eqref{eq:problem-full-1} into two problems.
% The first aims to solve for $\precbmat$ whereas the second solves for $\comcbmat$.
To begin, we initialize $\comcbmat$ as the so-called (quantized) conjugate beamforming codebook
\begin{align}
\comcbmat = \project{\Arx}{\comrfcb}
\end{align}
which allows us to then solve
\begin{subequations} \label{eq:problem-tx}
	\begin{align}
	\min_{\precbmat} \ & \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:problem-objective-tx} \\
	\st 
	& \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-tx} \\
	% &\ \abs{\vectorize{\precbmat}} \leq \onevec{\Nt\Mt} \label{eq:problem-entry-tx}
	& \bars{\entry{\precbmat}{m,n}} \leq 1 \ \forall \ m,n \label{eq:problem-entry-tx}
	% &\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-tx}
	\end{align}
\end{subequations}
using a convex solver.
The solution to \eqref{eq:problem-tx} is then projected onto the set $\prerfcb$ as
\begin{align}
\precbmat = \project{\precbmat}{\prerfcb} \label{eq:project-pre}
\end{align}
Afterwards, we solve the following for $\comcbmat$ using this updated $\precbmat$.
\begin{subequations} \label{eq:problem-rx}
	\begin{align}
	\min_{\comcbmat} \ & \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:problem-objective-rx} \\
	\st
	& \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-rx} \\
	% & \abs{\vectorize{\comcbmat}} \leq \onevec{\Nr\Mr} \label{eq:problem-entry-rx} \\
	& \bars{\entry{\comcbmat}{m,n}} \leq 1 \ \forall \ m,n \label{eq:problem-entry-rx}
	% &\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-rx} 
	\end{align}
\end{subequations}
Upon solving \eqref{eq:problem-rx}, we project its solution onto the set of possible beamformers in $\comrfcb$ as
\begin{align}
\comcbmat = \project{\comcbmat}{\comrfcb} \label{eq:project-com}
\end{align}
We iteratively execute \eqref{eq:problem-tx}--\eqref{eq:project-com} $\Niter \geq 1$ times.
This alternating minimization approach to designing $\precbmat$ and $\comcbmat$ is summarized in \algref{alg:algorithm-full-altmin}.

\input{alg/algorithm-full-altmin.tex}

%We now introduce an additional tuning parameter that affords engineers another knob to turn in our design.
%It may be desirable to halt the minimization of $\normfro{\comcbmat\ctrans \Hsi \precbmat}^2$ before our coverage constraints are tight.
%That is, we may not want to further degrade the transmit or receive gain at the cost of additional minimization of beam coupling.
%This is especially true in settings where marginal gain is had in minimizing $\normfro{\comcbmat\ctrans \Hsi \precbmat}^2$ at the cost of significant losses to transmit or receive gain.
%Therefore, we introduce a $\powerrfmax$ as the maximum power our design aims to achieve across beam pairs on average.
%More formally, we desire 
%\begin{align}
%\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \leq \powerrfmax \cdot \Gt \cdot \Gr \label{eq:frobenius-rf-constraint}
%\end{align}
%which suggests that the average power contained by entries in $\comcbmat\ctrans \Hsi \precbmat$ is at most $\powerrfmax$.
%
%Using this, we reformulate our objective as
%\begin{align}
%\max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr}
%\end{align}
%leading to
%\begin{subequations} \label{eq:problem-i-full}
%	\begin{align}
%	\min_{\precbmat,\comcbmat} &\ \max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} \\
%	\st 
%	&\ \abs{\diag{\Atx\ctrans \precbmat}}^2 \geq \gtxmin \cdot \onevec{\Gt} \\
%	&\ \abs{\diag{\Arx\ctrans \comcbmat}}^2 \geq \grxmin \cdot \onevec{\Gr} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr 
%	\end{align}
%\end{subequations}
%Problem \eqref{eq:problem-i-full} is non-convex due to the coupling between $\precbmat$ and $\comcbmat$ in the objective and the non-convexity of $\prerfcb$ and $\comrfcb$.
%Taking an alternating minimization approach, we split \eqref{eq:problem-i-full} into
%\begin{subequations} \label{eq:problem-i-full-f}
%	\begin{align}
%	\min_{\precbmat} &\ \max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} \\
%	\st 
%	&\ \abs{\diag{\Atx\ctrans \precbmat}}^2 \geq \gtxmin \cdot \onevec{\Gt} \label{eq:problem-i-full-f-coverage} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-i-full-f-non-convex}
%	\end{align}
%\end{subequations}
%and
%\begin{subequations} \label{eq:problem-i-full-w}
%	\begin{align}
%	\min_{\comcbmat} & \ \max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} \\
%	\st 
%	&\ \abs{\diag{\Arx\ctrans \comcbmat}}^2 \geq \grxmin \cdot \onevec{\Gr} \label{eq:problem-i-full-w-coverage} \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-i-full-w-non-convex}
%	\end{align}
%\end{subequations}
%which have convex objectives but have non-convex constraints per \eqref{eq:problem-i-full-f-non-convex} and \eqref{eq:problem-i-full-w-non-convex}.
%Notice that since
%\begin{align}
%\normfro{\mA} = \normfro{\mA\ctrans}
%\end{align}
%we can see that problems \eqref{eq:problem-i-full-f} and \eqref{eq:problem-i-full-w} are of the same form.
%Thus, an algorithm created to solve one can be used to solve the other, which we present as follows.
%
%Let us define the projection of a vector $\vx$ onto a set of vectors $\set{A}$ as
%\begin{align}
%\project{\vx}{\set{A}} = \arg \min_{\va \in \set{A}} \normtwo{\va - \vx}
%\end{align}
%and overload it to act column-wise on matrices as
%\begin{align}
%\entry{\project{\mX}{\set{A}}}{:,\ell} = \project{\entry{\mX}{:,\ell}}{\set{A}}
%\end{align}
%
%We take a projected gradient descent approach to solving \eqref{eq:problem-i-full-f} and \eqref{eq:problem-i-full-w}.
%We outline our algorithm as follows with notation of \eqref{eq:problem-i-full-f} with the understanding that it can also be used to solve \eqref{eq:problem-i-full-w} with a proper change of variables.
%Our algorithm, which is summarized in \algref{alg:algorithm-full-i}, begins by initializing $\precbmat$ and $\comcbmat$ as
%\begin{gather}
%\precbmat\node{1} = \precbmatinit = \project{\Atx}{\prerfcb} \\
%\comcbmat\node{1} = \comcbmatinit = \project{\Arx}{\comrfcb}
%\end{gather}
%where $\precbmat\node{n}$ and $\comcbmat\node{n}$ denote $\precbmat$ and $\comcbmat$ at the $n$-th gradient step.
%Let $\Niter$ be the number of iterations (gradient steps) that our algorithm takes.
%Let $\mu_\pre$ and $\mu_\com$ be the gradient step size during a gradient step of $\precbmat$ and $\comcbmat$, respectively.
%
%Noting that the gradient of the squared Frobenius norm is
%\begin{align}
%\nabla_{\mX} \normfro{\mA \mX}^2 = 2 \cdot \mA\ctrans \mA \mX
%\end{align}
%Thus, a gradient step on $\precbmat$ is defined as follows
%\begin{align}
%% \precbmat\node{n+1} = \precbmat\node{n} - \mu_{\pre} \cdot \mM_\pre \had \parens{2 \cdot \Hsi\ctrans \comcbmat\node{n} \comcbmat\ctransnode{n} \Hsi \precbmat\node{n}}
%\precbmat\node{n+1} = \precbmat\node{n} - \mu_{\pre} \cdot 2 \cdot \Hsi\ctrans \comcbmat\node{n} \comcbmat\ctransnode{n} \Hsi \precbmat\node{n} \label{eq:pre-gradient-step}
%\end{align}
%% where we refer to $\mM_\pre \in \setmatrixreal{\Nt}{\Gt}$ as a ``gradient mask'' that we will describe shortly.
%We then project $\precbmat\node{n+1}$ as
%\begin{align}
%\precbmat\node{n+1} = \project{\precbmat\node{n+1}}{\prerfcb}
%\end{align}
%Then, to ensure that the recent gradient step does not violate our transmit coverage constraint, we evaluate which beams have fallen below a transmit gain of $\gtxmin$
%\begin{align}
%\set{J}_\pre\node{n+1} = \braces{\ell : \entry{\precbmat\ctransnode{n+1} \Atx \Atx\ctrans \precbmat\node{n+1}}{\ell,\ell} < \gtxmin}
%\end{align}
%Using this index set, we revert columns index by $\set{J}_\pre\node{n+1}$ in $\precbmat\node{n+1}$ to those in the previous iteration.
%% Using this index set, we create a gradient mask matrix
%%\begin{align}
%%\entry{\mM_\pre}{:,\set{J}_\pre\node{n+1}} = \zeromat
%%\end{align}
%%which will be used to freeze the columns of $\precbmat$ that are FIX THIS, using gradient mask like this may be sub-optimal.
%\begin{align}
%\entry{\precbmat\node{n+1}}{:,\set{J}_\pre\node{n+1}} = \entry{\precbmat\node{n}}{:,\set{J}_\pre\node{n+1}} \label{eq:pre-step-back}
%\end{align}
%This ensures that the coverage constraint is maintained by $\precbmat\node{n+1}$, satisfying \eqref{eq:problem-i-full-f-coverage}.
%
%
%We repeat this process on the $n$-th gradient update of $\comcbmat$, which are summarized as follows.
%\begin{gather}
%\comcbmat\node{n+1} = \comcbmat\node{n} - \mu_{\com} \cdot 2 \cdot \Hsi \precbmat\node{n+1} \precbmat\ctransnode{n+1} \Hsi\ctrans \comcbmat\node{n} \label{eq:com-gradient-step} \\
%\comcbmat\node{n+1} = \project{\comcbmat\node{n+1}}{\comrfcb} \\
%\set{J}_\com\node{n+1} = \braces{\ell : \entry{\comcbmat\ctransnode{n+1} \Arx \Arx\ctrans \comcbmat\node{n+1}}{\ell,\ell} < \grxmin} \\
%\entry{\comcbmat\node{n+1}}{:,\set{J}_\com\node{n+1}} = \entry{\comcbmat\node{n}}{:,\set{J}_\com\node{n+1}} \label{eq:com-step-back}
%\end{gather}
%Note that the gradient step of the $n$-th step, as evidenced by \eqref{eq:com-gradient-step}, uses the already-updated $\precbmat\node{n+1}$ according to the alternating minimization approach we have taken.
%
%We now outline the exit criteria for our algorithm.
%At most, our algorithm concludes after $\Niter$ gradient updates.
%Otherwise, our algorithm halts when \eqref{eq:frobenius-rf-constraint} is met or when 
%\begin{align}
%\precbmat\node{n+1} = \precbmat\node{n} \label{eq:exit-criteria-static}
%\end{align}
%Note that \eqref{eq:exit-criteria-static} can happen when
%\begin{align}
%\card{\set{J}_\pre} = \Gt
%\end{align}
%and
%\begin{align}
%\card{\set{J}_\com} = \Gr
%\end{align}
%or when the gradient steps are so small (including zero) that they are effectively nullified during the projections onto $\prerfcb$ and $\comrfcb$.
%This places increased significance on the choices of $\mu_\pre$ and $\mu_\com$ and convergence to good solutions of $\precbmat$ and $\comcbmat$.

\comment{
---

\begin{gather}
\normtwo{\entry{\Atx}{:,\ell}}^2 = \Nt, \quad \ell = 1, \dots, \Mt \\
\normtwo{\entry{\Arx}{:,\ell}}^2 = \Nr, \quad \ell = 1, \dots, \Mr
\end{gather}

\begin{gather}
\normfro{\Atx}^2 = \Nt \cdot \Mt \\
\normfro{\Arx}^2 = \Nr \cdot \Mr
\end{gather}

\begin{gather}
\normtwo{\entry{\precbmat}{:,\ell}}^2 \leq \Nt, \quad \ell = 1, \dots, \Mt \\
\normtwo{\entry{\comcbmat}{:,\ell}}^2 \leq \Nr, \quad \ell = 1, \dots, \Mr
\end{gather}

\begin{gather}
\normfro{\precbmat}^2 \leq \Nt \cdot \Mt \\
\normfro{\comcbmat}^2 \leq \Nr \cdot \Mr
\end{gather}

\begin{gather}
\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \leq \normfro{\comcbmat\ctrans}^2 \cdot \normfro{\Hsi}^2 \cdot \normfro{\precbmat}^2
\end{gather}

Let's say
\begin{gather}
\atx{\aod_\ell}\ctrans \vf_\ell = \Gtxtgt \ \forall \ \ell = 1, \dots, \Mt \\
\arx{\aoa_\ell}\ctrans \vw_\ell = \Grxtgt \ \forall \ \ell = 1, \dots, \Mr
\end{gather}

Then
\begin{align}
\normtwo{\arx{\aoa_\ell}\ctrans \vw_\ell} &= \Grxtgt \\
&\leq \normtwo{\arx{\aoa_\ell}} \cdot \normtwo{\vw_\ell}
\end{align}
so
\begin{align}
\normtwo{\vw_\ell} 
&\geq \frac{\Grxtgt}{\normtwo{\arx{\aoa_\ell}}} \\
&= \frac{\Grxtgt}{\sqrt{\Nr}} 
\end{align}
---
}

% \input{alg/algorithm-gradient-step.tex}

% \input{alg/algorithm-full-i.tex}

==> sec-contribution-i.tex <==
\section{Analog Beamforming Codebook Design} \label{sec:contribution-i}

% We now outline an analog beamforming codebook design methodology that reduces the self-interference that is coupled between transmit-receive beam pairs while also ensuring transmit beams and receive beams provide sufficient gain to a desired coverage region.
We now outline an analog beamforming codebook design methodology construct $\precbbar$ and $\comcbbar$ with reduced self-interference coupling between transmit-receive beam pairs while also ensuring the transmit and receive beams remain useful in serving users.
In this section, we assume perfect channel knowledge of $\mH$ is had along with the assumption that the self-interference channel remains sufficiently static as previously described.
% Our design accounts for the hardware constraints imposed on beamforming weights due to finite resolution phase shifters and attenuators.
% Note that our design does not require that attenuators be present, though it will improve from having such; we will evaluate both cases in our numerical results in \secref{sec:simulation-results}.

\subsection{Quantifying our Codebook Design Criteria}

High beamforming gain afforded by dense analog beamforming arrays is essential for wide area \mmwave communication.
Therefore, it is critical that our analog beamforming codebook maintain high beamforming gain across a desired coverage region.

\begin{definition}[Transmit and receive coverage regions]
Let $\dirtxset$ be a set of $\Mtx$ transmit directions---or a \textit{transmit coverage region}---that our codebook aims to transmit toward.
Similarly, let $\dirtxset$ be a set of $\Mrx$ receive directions---or a \textit{receive coverage region}---that our codebook aims to receive from.
\begin{gather}
	\dirtxset = \braces{\dirtx\idx{i} : i = 1, \dots, \Mtx} \\
	\dirrxset = \braces{\dirrx\idx{j} : j = 1, \dots, \Mrx}
\end{gather}
\end{definition}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.2\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_00}
	\caption{Example discretized transmit and receive coverage regions $\dirtxset$ and $\dirrxset$ comprised of $\Mtx = \Mrx = 45$ points spaced uniformly in azimuth from $-60^\circ$ to $60^\circ$ with $15^\circ$ spacing and in elevation from $-30^\circ$ to $30^\circ$ with $15^\circ$ spacing. The directions $\dirtx\idx{i}$ and $\dirrx\idx{j}$ are shown here as their respective projections onto the $y$-$z$ plane, where looking into the page represents steering outward from each array (the positive $x$ direction).}
	\label{fig:dirset}
\end{figure}

% Corresponding to each of these transmit and receive directions, 

% Let $\atx{\dirtx} \in \setvectorcomplex{\Nt}$ be the transmit array response vector in the direction of $\aod$, and let $\arx{\aoa} \in \setvectorcomplex{\Nr}$ be the receive array response vector in the direction of $\aoa$.
Let $\Atx \in \setmatrixcomplex{\Nt}{\Mtx}$ be the matrix of transmit array response vectors evaluated at the directions in $\dirtxset$, and let $\Arx \in \setmatrixcomplex{\Nr}{\Mrx}$ be the matrix of receive array response vectors evaluated at the directions in $\dirrxset$.
\begin{align}
\Atx &= 
\begin{bmatrix}
\atx{\dirtx\idx{1}} & \atx{\dirtx\idx{2}} & \cdots & \atx{\dirtx\idx{\Mtx}}
\end{bmatrix}  \\
\Arx &= 
\begin{bmatrix}
\arx{\dirrx\idx{1}} & \arx{\dirrx\idx{2}} & \cdots & \arx{\dirrx\idx{\Mrx}}
\end{bmatrix}
\end{align}
%\begin{align}
%\Arx = \blkdiag{\arx{\aoa_1}, \arx{\aoa_2}, \dots, \arx{\aoa_{\Gr}}} \in \setmatrixcomplex{\Nr\Gr}{\Gr}
%\end{align}

Let us index the beams in $\precbbar$ and $\comcbbar$ according to $\dirtxset$ and $\dirrxset$, respectively, as
\begin{gather}
\precbbar = \braces{\vf_1, \dots, \vf_{\Mtx}} \\
\comcbbar = \braces{\vw_1, \dots, \vw_{\Mrx}}
\end{gather}
where $\vf_i \in \precb$ is responsible for transmitting toward $\dirtx\idx{i}$ and $\vw_j \in \comcb$ is responsible for receiving from $\dirrx\idx{j}$.
Using this notation, we build the matrix $\precbmat$ by stacking all transmit beams $\vf_i$ as
\begin{align}
\precbmat = 
\begin{bmatrix}
\vf_1 & \vf_2 & \cdots & \vf_{\Mtx}
\end{bmatrix} \in \setmatrixcomplex{\Nt}{\Mtx}
\end{align}
and the matrix $\comcbmat$ by stacking all receive beams $\vw_j$ as
\begin{align}
\comcbmat = 
\begin{bmatrix}
\vw_1 & \vw_2 & \cdots & \vw_{\Mrx}
\end{bmatrix} \in \setmatrixcomplex{\Nr}{\Mrx}
\end{align}

%A device not falling directly on the grid $\aodset$ or $\aoaset$ will be served by the beam that steers closest to it. \edit{Should I write this out explicitly using $\argmin$?}
%A device not falling directly on the grid of angles in $\aodset$ or $\aoaset$ can be served by the beam that steers closest to it. Explicitly, a receiving device in the direction of $\aod$ or a transmitting device in the direction of $\aoa$ can be served by the $\ell\parens{\aod}$-th transmit beam or the $\ell\parens{\aoa}$-th receive beam, respectively, where
%\begin{align}
%\ell\parens{\aod} = \arg \min_{\ell} \bars{\aod - \aod_\ell} \\
%\ell\parens{\aoa} = \arg \min_{\ell} \bars{\aoa - \aoa_\ell}
%\end{align}

% Recall that $\Hsi \in \setmatrixcomplex{\Nr}{\Nt}$ is the over-the-air self-interference channel matrix between the transmit and receive arrays of our full-duplex transceiver.
%The coupling between the $m$-th analog precoder $\vf_{m}$ and $n$-th analog combiner $\vw_n$ is
%\begin{align}
%\vw_n\ctrans \times \Hsi \times \vf_{m} \in \setvectorcomplex{1}
%\end{align}
%Collecting the coupling between all analog precoding-combining pairs into a matrix $\mM$, we get
%\begin{align}
%\mM = \comcbmat\ctrans \Hsi \precbmat \in \setmatrixcomplex{\Mr}{\Mt}
%\end{align}
%where $\entry{\mM}{n,m} = \vw_n\ctrans \times \Hsi \times \vf_{m}$.

The coupling between the $i$-th transmit beam $\vf_i$ and the $j$-th receive beam $\vw_j$ can be captured simply by the matrix product $\comcbmat\ctrans \mH \precbmat \in \setmatrixcomplex{\Mrx}{\Mtx}$.
To reduce the coupling across beam pairs, our design aims to minimize the \textit{average}\footnote{Other objectives, such as minimizing the worst-case coupling, may also be useful.} energy of $\comcbmat\ctrans \mH \precbmat$, which we denote $E$ and write as follows.
\begin{align}
E = \frac{1}{\Mtx\Mrx} \cdot \normfro{\comcbmat\ctrans \mH \precbmat}^2 \label{eq:power-si}
\end{align}
In our design's attempt to minimize $E$, we must ensure that the beams in $\precbmat$ and $\comcbmat$ remain useful in serving users within the coverage region; of course, unconstrained, $\precbmat$ and $\comcbmat$ minimize $E$ when driven to $\zeromat$.
Notice that our definition of $E$ neglects the large-scale channel gain $G$, which would merely scale $E$.
We now quantify a means to constrain our design to ensure it can maintain service.

Let $\Gtxmax^2 = \Nt^2$ and $\Grxmax^2 = \Nr^2$ be the maximum transmit and receive power gain supplied our arrays, which can be achieved toward $\dir$ with \textit{conjugate beamformers} $\vf = \atx{\dir}$ and $\vw = \arx{\dir}$, respectively.
Let $\Gtx^2\parens{\dirtx\idx{i}}$ be the transmit power gain afforded by $\vf_i$ in the direction of $\dirtx\idx{i}$ and $\Grx^2\parens{\dirrx\idx{j}}$ be the receive power gain afforded by $\vw_j$ in the direction of $\dirrx\idx{j}$, which can be written as
\begin{align}
\Gtx^2\parens{\dirtx\idx{i}} &= \bars{\atx{\dirtx\idx{i}}\ctrans \times \vf_i}^2 \leq \Gtxmax^2 \label{eq:Gtx} \\
\Grx^2\parens{\dirrx\idx{j}} &= \bars{\arx{\dirrx\idx{j}}\ctrans \times \vw_j}^2 \leq \Grxmax^2 \label{eq:Grx}
\end{align}

\begin{figure*}
	\centering
	\subfloat[A conventional codebook.]{\includegraphics[width=0.47\linewidth]{plots/v01/generate_v01_process_v01_fig_09_tgt-1}
		\label{fig:matrix-cbf}}
	\quad
	\subfloat[Our codebook.]{\includegraphics[width=0.47\linewidth]{plots/v01/generate_v01_process_v01_fig_09_ours}
		\label{fig:matrix-ours}}
	\caption{The magnitude squared (in dB) of the beam coupling matrix $\comcbmat\ctrans \mH \precbmat$ for a conventional codebook and a codebook output by our design. Each transmit and receive codebook contains $45$ beams.}
	\label{fig:matrix}
\end{figure*}

%\begin{definition}[Minimum required transmit and receive beamforming gain]
%	Let $\Gtxmin^2$ and $\Grxmin^2$ be the minimum transmit and receive beamforming power gain for any precoder or combiner, respectively, in the direction it intends to serve; that is to say that $\prerfcbbar$ and $\comrfcbbar$ are required to have beams that satisfy
%	\begin{align}
%		\Gtxell \geq \Gtxmin \ \forall \ \ell \in \braces{1,\dots,\Mt} \label{eq:coverage-constraint-tx} \\
%		\Grxell \geq \Grxmin \ \forall \ \ell \in \braces{1,\dots,\Mr} \label{eq:coverage-constraint-rx}
%	\end{align}
%\end{definition}

To offer our design flexibility in reducing $E$, we will tolerate some degradation in beamforming gain toward our desired directions; in other words, we will aim for some beamforming gain less than $\Gtxmax^2$ and $\Grxmax^2$ in exchange for improved self-interference rejection.
The beamforming gains we will aim for we term our \textit{target} transmit and receive beamforming gain.

\begin{definition}[Target transmit and receive gain.]
	Let $\Gtxtgt^2$ and $\Grxtgt^2$ be the \textit{target} transmit and receive beamforming gains for any transmit beam $\vf_i$ or receive beam $\vw_j$, respectively, in the direction it intends to serve. In other words, that is to say that 
	\begin{gather}
		\Gtxtgt^2 \approx \Gtx^2\parens{\dirtx\idx{i}} \ \forall \ i \in \braces{1,\dots,\Mtx} \label{eq:target-gain-tx-approx} \\
		\Grxtgt^2 \approx \Grx^2\parens{\dirrx\idx{j}} \ \forall \ j \in \braces{1,\dots,\Mrx} \label{eq:target-gain-rx-approx}
	\end{gather}
	which we will more precisely quantify shortly.
	Note that specific target gains for each beam in each codebook can be defined uniquely, though we use a common target codebook-wide for simplicity.
	Let $\Gtxtgt^2$ and $\Grxtgt^2$ be defined conveniently using $0 < \Deltatx^2 \leq 1$ and $0 < \Deltarx^2 \leq 1$ as follows.
	\begin{align}
	\Gtxtgt^2 = \Deltatx^2 \cdot \Gtxmax^2 \\
	\Grxtgt^2 = \Deltarx^2 \cdot \Grxmax^2
	\end{align}
	$\Deltatx^2$ and $\Deltarx^2$ capture the loss in beamforming gain that we tolerate as part of our design.
%	More convenient log-scale expressions are
%	\begin{align}
%	\todB{\Gtxtgt^2} = \todB{\Gtxmax^2} + \todB{\Deltatx^2} \\
%	\todB{\Grxtgt^2} = \todB{\Grxmax^2} + \todB{\Deltarx^2}
%	\end{align}
%	where $\todB{\Deltatx^2} \leq 0$ and $\todB{\Deltarx^2} \leq 0$.
	The tolerated losses $\Deltatx^2$ and $\Deltarx^2$ are design parameters that can be determined by system engineers.
\end{definition}


\begin{definition}[Transmit and receive gain variance.]
	To quantify approximately meeting the target gains in \eqref{eq:target-gain-tx-approx} and \eqref{eq:target-gain-rx-approx}, we introduce a variance tolerance.
	Let $\sigmatx^2 \geq 0$ be the maximum variance tolerated in achieving the target transmit (amplitude) gain  $\Gtxtgt$ across beams in the transmit codebook $\precbbar$, normalized to $\Gtxtgt^2$.
	\begin{align}
	\frac{1}{\Mtx} \cdot \sum_{i=1}^{\Mtx} \frac{\bars{\Gtxtgt - \Gtx\parens{\dirtx\idx{i}}}^2}{\Gtxtgt^2} \leq \sigmatx^2 \label{eq:sigma-tx}
	\end{align}
	Similarly, let $\sigmarx^2 \geq 0$ be the maximum variance tolerated in achieving the target receive (amplitude) gain $\Grxtgt$ across all beams in the receive codebook $\comcbbar$, normalized to $\Grxtgt^2$.
	\begin{align}
	\frac{1}{\Mrx} \cdot \sum_{j=1}^{\Mrx} \frac{\bars{\Grxtgt - \Grx\parens{\dirrx\idx{j}}}^2}{\Grxtgt^2} \leq \sigmarx^2  \label{eq:sigma-rx}
	\end{align}
	More variance across transmit and receive gain provided by our beams may increase the disparity of service seen across users, though would also allow our design more flexibility in its attempt to reduce self-interference.
\end{definition}

\subsection{Assembling our Codebook Design Problem}
With expressions for our codebook design criteria in hand, we now turn our attention to assembling a formal design problem.
Let $\gtxtgt = \Gtxtgt \cdot \onevec{\Mtx}$ and $\grxtgt = \Grxtgt \cdot \onevec{\Mrx}$ be vectors containing the target transmit and receive gains at each entry.
%\begin{align}
%\gtxtgt = \Gtxtgt \cdot \onevec{\Mtx} \label{eq:gtx} \\
%\grxtgt = \Grxtgt \cdot \onevec{\Mrx} \label{eq:grx}
%\end{align}
Using this, the expressions of \eqref{eq:sigma-tx} and \eqref{eq:sigma-rx} can be equivalently written as follows, which we refer to as our \textit{coverage constraints},
\begin{align}
\normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mtx \label{eq:coverage-constraint-tx} \\
\normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mrx \label{eq:coverage-constraint-rx}
\end{align}
where the $(i,i)$-th entry of $\Atx\ctrans \precbmat$ has magnitude $\Gtx\parens{\dirtx\idx{i}}$ and the $(j,j)$-th entry of $\Arx\ctrans \comcbmat$ has magnitude $\Grx\parens{\dirrx\idx{j}}$.
By satisfying \eqref{eq:coverage-constraint-tx} and \eqref{eq:coverage-constraint-rx}, we can ensure that our codebooks $\precbbar$ and $\comcbbar$ adequately serve our coverage regions.
% Note that these two constraints capture the gain and coverage constraints of our two codebooks $\prerfcbbar$ and $\comrfcbbar$.

% The parameters $\Gtxtgt$ and $\Grxtgt$ (equivalently $\Deltatx$ and $\Deltatx$) along with $\sigmatx^2$ and $\sigmatx^2$ can be tuned as desired by system engineers. 
% We will explore their impact on the design our numerical results in \secref{sec:simulation-results}.
%Convenient log-scale representations of $\sigmatx^2$ and $\sigmarx^2$ are 
%\begin{align}
%\todB{\sigmatx^2} = 10 \cdot \logten{\sigmatx^2} \\
%\todB{\sigmatx^2} = 10 \cdot \logten{\sigmatx^2} 
%\end{align}
%where it practical to take $\todB{\sigmatx^2} \leq 0$ dB (i.e., $\sigmatx^2 \leq 1$) and $\todB{\sigmatx^2} \leq 0$ dB (i.e., $\sigmatx^2 \leq 1$).
%Lower $\sigmatx^2$, $\sigmatx^2$ results in stricter constraints (less variance in achieving targets).

With the coverage constraints in hand, let us now formulate our problem as
\begin{subequations} \label{eq:problem-full-1}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \mH \precbmat}^2 \label{eq:problem-objective-1} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mtx \label{eq:problem-coverage-tx-1} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mrx \label{eq:problem-coverage-rx-1} \\
	&\ \entry{\precbmat}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-1} \\
	&\ \entry{\comcbmat}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-1} 
	\end{align}
\end{subequations}
The parameters $\Gtxtgt$ and $\Grxtgt$ (equivalently $\Deltatx$ and $\Deltatx$) along with $\sigmatx^2$ and $\sigmatx^2$ can be tuned as desired by system engineers. 
As we will see, permitting $\Gtxtgt$ and $\Grxtgt$ to be lower will relax the constraints of our design, allowing it to better reduce self-interference coupled by our transmit and receive beams; this helps facilitate full-duplexing service to two devices but degrades the service each device experiences.
Furthermore, increasing $\sigmatx^2$ and $\sigmarx^2$ will increase the flexibility of our design, but will lessen the coverage guarantee.
We examine this tradeoff in our numerical results in \secref{sec:simulation-results}.


\subsection{Capturing Self-Interference Channel Errors}
Abiding by the scope of this work, it is reasonable to assume the self-interference channel $\mH$ may not be perfectly estimated and may vary slowly over time.
Small changes in $\mH$ may render designs of $\precbmat$ and $\comcbmat$ far less useful if not designed for such, especially since self-interference is likely overwhelmingly strong.
Suppose instead of having perfect knowledge of true over-the-air channel, $\mH$ is an estimate of the true channel $\bar{\mH}$ and knowledge of an estimation error bound.
Specifically, let us define the set of all possible $\bar{\mH}$ as
\begin{align}
\Hsiset = \braces{\bar{\mH} = \mH + \sqrt{\Nt \Nr} \cdot \mDelta : \normfro{\mDelta} \leq \epsilon}
\end{align}
where the matrix $\mDelta$ captures the error in our estimate $\mH$ and is bounded by its Frobenius norm as $\normfro{\mDelta} \leq \epsilon$.
Note that other norm-bound errors can be encapsulated by appropriate choice of $\epsilon$ via norm equivalence.
We take a worst-case optimization approach to design $\precbmat$ and $\comcbmat$ in the presence of channel error $\mDelta$, leading to problem \eqref{eq:problem-full-2}.
\begin{subequations} \label{eq:problem-full-2}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \max_{\normfro{\mDelta} \leq \epsilon} \ \normfro{\comcbmat\ctrans \parens{\mH + \sqrt{\Nt \Nr} \cdot \mDelta} \precbmat} \label{eq:problem-objective-2} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mtx \label{eq:problem-coverage-tx-2} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mrx \label{eq:problem-coverage-rx-2} \\
	&\ \entry{\precbmat}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-2} \\
	&\ \entry{\comcbmat}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-2} 
	\end{align}
\end{subequations}

\begin{theorem} \label{thm:error-upper-bound}
	The objective in \eqref{eq:problem-objective-2} is upper bounded by 
	\begin{align}
	\max_{\normfro{\mDelta} \leq \epsilon} \normfro{\comcbmat\ctrans \parens{\mH + \sqrt{\Nt \Nr} \cdot \mDelta} \precbmat}
	% &= \normfro{\comcbmat\ctrans \mH \precbmat} + \normfro{\comcbmat\ctrans \mDelta \precbmat} \\
	&\leq \normfro{\comcbmat\ctrans \mH \precbmat} + \epsilon \cdot \sqrt{\Nt \Nr} \cdot \normtwo{\comcbmat} \cdot \normtwo{\precbmat}
	\end{align}
	which does not depend on $\mDelta$ but merely $\epsilon$.
\begin{proof}
	\begin{align}
	\mU_{\mA} \mSigma_{\mA} \mV_{\mA} = \svdop{\mA} 
	\end{align}
	\begin{align}
	\normfro{\comcbmat\ctrans \parens{\mH + \mDelta} \precbmat} 
	&= \normfro{\mU_{\mW} \mSigma_{\mW} \mV_{\mW}\ctrans \parens{\mH + \mDelta} \mU_{\mF} \mSigma_{\mF} \mV_{\mF}\ctrans} \\
	&= \normfro{\mSigma_{\mW} \mV_{\mW}\ctrans \parens{\mH + \mDelta} \mU_{\mF} \mSigma_{\mF}} \\
	&= \normfro{\mSigma_{\mW} \mV_{\mW}\ctrans \mH \mU_{\mF} \mSigma_{\mF} + \mSigma_{\mW} \mV_{\mW}\ctrans \mDelta \mU_{\mF} \mSigma_{\mF}} \\
	&= \normfro{\mA + \mSigma_{\mW} \mV_{\mW}\ctrans \mDelta \mU_{\mF} \mSigma_{\mF}} \\
	&= \normfro{\mU_{\mA} \mSigma_{\mA} \mV_{\mA}\ctrans + \mSigma_{\mW} \mV_{\mW}\ctrans \mDelta \mU_{\mF} \mSigma_{\mF}} \\
	&= \normfro{\mU_{\mA} \mSigma_{\mA} \mV_{\mA}\ctrans + \mU_{\mA} \mSigma_{\mDelta} \mV_{\mA}\ctrans} \\
	&\leq \normfro{\mU_{\mA} \mSigma_{\mA} \mV_{\mA}\ctrans + \vu_{\mA} \vv_{\mA}\ctrans \cdot \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat}} \\
	&\leq \normfro{\mU_{\mA} \mSigma_{\mA} \mV_{\mA}\ctrans} + \normfro{\vu_{\mA} \vv_{\mA}\ctrans \cdot \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat}} \\
	&= \normfro{\mU_{\mA} \mSigma_{\mA} \mV_{\mA}\ctrans} + \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat} \\
	&= \normfro{\mU_{\mW} \mU_{\mA} \mSigma_{\mA} \mV_{\mA}\ctrans \mV_{\mF}\ctrans} + \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat} \\
	&= \normfro{\comcbmat\ctrans \mH \precbmat} + \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat}
	\end{align}
	\comment{
	Equality is obtained when $\mA$ has rank one since
	\begin{align}
	\normfro{\mA + \epsilon \cdot \mA} 
	&= \normfro{\parens{1 + \epsilon} \cdot \mA} \\
	&= \parens{1+\epsilon} \cdot \normfro{\mA} \\
	&= \normfro{\mA} + \epsilon \cdot \normfro{\mA} \\
	&= \normfro{\mA} + \normfro{\epsilon \cdot \mA}
	\end{align}}
\end{proof}
\end{theorem}

Using \thmref{thm:error-upper-bound}, problem \eqref{eq:problem-full-2} can be reformulated to the slightly different problem \eqref{eq:problem-full-3} as follows, which takes a familiar regularizing form.
Instead of using $\epsilon$ directly, we use $\tilde{\epsilon} \leq \epsilon$, which can be chosen to better handle general channel errors, rather than strictly the worst-case one.
\begin{subequations} \label{eq:problem-full-3}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \mH \precbmat} + \tilde{\epsilon} \cdot \sqrt{\Nt \Nr} \cdot \normtwo{\precbmat} \cdot \normtwo{\comcbmat} \label{eq:problem-objective-3} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mtx \label{eq:problem-coverage-tx-3} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mrx \label{eq:problem-coverage-rx-3} \\
	&\ \entry{\precbmat}{:,i} \in \precb \ \forall \ i = 1, \dots, \Mtx \label{eq:problem-quantize-tx-3} \\
	&\ \entry{\comcbmat}{:,j} \in \comcb \ \forall \ j = 1, \dots, \Mrx \label{eq:problem-quantize-rx-3} 
	\end{align}
\end{subequations}
Problem \eqref{eq:problem-full-3} is much more straightforwardly solved than problem \eqref{eq:problem-full-2} since it does not require optimization over $\mDelta$.
By solving problem \eqref{eq:problem-full-3}, codebooks $\precbbar$ and $\comcbbar$ will contain beams that are more robust to channel errors due to estimation or slight variations over time.
Note that problem \eqref{eq:problem-full-2} and problem \eqref{eq:problem-full-3} are identical when $\tilde{\epsilon} = 0$.

%channel error $\mDelta$ that contributes the most significant error to our objective is found to be
%\begin{align}
%\mDelta = \epsilon \cdot \vu \times \vv\ctrans
%\end{align}
%where $\vu$ is the right singular vector of $\comcbmat$ corresponding to its strongest singular value and $\vv$ is the left singular vector of $\precbmat$ corresponding to its strongest singular value.
%This results in
%\begin{align}
%\max_{\normfro{\mDelta} \leq \epsilon} \normfro{\comcbmat\ctrans \parens{\mH + \mDelta} \precbmat} 
%% &= \normfro{\comcbmat\ctrans \mH \precbmat} + \normfro{\comcbmat\ctrans \mDelta \precbmat} \\
%&= \normfro{\comcbmat\ctrans \mH \precbmat} + \epsilon \cdot \normtwo{\comcbmat} \cdot \normtwo{\precbmat}
%% &= \normfro{\comcbmat\ctrans \mH \precbmat} + \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat} = \epsilon \cdot \normtwo{\comcbmat} \cdot \normtwo{\precbmat}
%\end{align}
%
%T
%
%\begin{align}
%\normfro{\epsilon \comcbmat\ctrans \vu \vv\ctrans \precbmat} 
%&= \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat} = \epsilon \cdot \normtwo{\comcbmat} \cdot \normtwo{\precbmat}
%\end{align}
%
%This leads
% by creating problem \eqref{eq:problem-full-4}.





% ---

%A common approach in worst-case robust optimization is to greatly simplify the problem by writing the resulting worst-case error in a closed-form fashion to eliminate the error term itself.
%We take a similar approach.
%It is difficult to find the error $\Hsierror$ that maximizes 
%\begin{align}
%\normfro{\comcbmat\ctrans \parens{\Hsiest + \Hsierror} \precbmat}
%\end{align}
%for a given $\precbmat$ and $\comcbmat$ due to the sandwiching of $\Hsi = \Hsiest + \Hsierror$.
%Via the triangle identity, we have
%\begin{align}
%\normfro{\comcbmat\ctrans \parens{\Hsiest + \Hsierror} \precbmat} \leq \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \normfro{\comcbmat\ctrans \Hsierror \precbmat}
%\end{align}
%which allows us to adjust our problem to 
%\begin{subequations} \label{eq:problem-full-4}
%	\begin{align}
%	\min_{\precbmat,\comcbmat} &\ \max_{\normfro{\Hsierror} \leq \epsilon} \ \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \normfro{\comcbmat\ctrans \Hsierror \precbmat} \label{eq:problem-objective-4} \\
%	\st 
%	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-4} \\
%	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-4} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-4} \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-4} 
%	\end{align}
%\end{subequations}
%which is will produce a solution that is more robust than the original problem.
%Using the inequality
%\begin{align}
%\normfro{\mA \mB} \leq \normtwo{\mA} \cdot \normfro{\mB}
%\end{align}
%we can see that an upper bound can be written as
%\begin{align}
%\max_{\normfro{\Hsierror} \leq \epsilon} \ \normfro{\comcbmat\ctrans \Hsierror \precbmat} \leq \normtwo{\comcbmat} \cdot \normfro{\Hsierror} \cdot \normtwo{\precbmat}
%\end{align}
%which can be achieved when
%\begin{align}
%\Hsierror = \epsilon \cdot \vu \times \vv\ctrans
%\end{align}
%where $\vu$ is the right singular vector of $\comcbmat$ corresponding to its strongest singular value and $\vv$ is the left singular vector of $\precbmat$ corresponding to its strongest singular value.
%This results in
%\begin{align}
%\normfro{\epsilon \comcbmat\ctrans \vu \vv\ctrans \precbmat} 
%&= \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat} \\
%&= \epsilon \cdot \normtwo{\comcbmat} \cdot \normtwo{\precbmat}
%\end{align}
%
%Therefore, we reformulate our problem \eqref{eq:problem-full-4} as
%\begin{subequations} \label{eq:problem-full-5}
%	\begin{align}
%	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \epsilon \cdot \normtwo{\comcbmat} \normtwo{\precbmat} \label{eq:problem-objective-5} \\
%	\st 
%	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-5} \\
%	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-5} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-5} \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-5} 
%	\end{align}
%\end{subequations}
%which is only a function of $\epsilon$ and no longer a function of $\Hsierror$.
%Note that our robust problem has taken on a regularizing form, as is common in handling worst-case robust optimization involving norms.

\comment{
\subsection{Solving for our Codebook Design}
The objective \eqref{eq:problem-objective-1} is convex along with constraints \eqref{eq:problem-coverage-tx-1} and \eqref{eq:problem-coverage-rx-1}.
Constraints \eqref{eq:problem-quantize-tx-1} and \eqref{eq:problem-quantize-rx-1}, of course, are not due to the limited resolution of each phase shifter and attenuator.
Therefore, to solve \eqref{eq:problem-full-1}, we use a projection-based alternating minimization as follows.
% We split \eqref{eq:problem-full-1} into two problems.
% The first aims to solve for $\precbmat$ whereas the second solves for $\comcbmat$.
To begin, we initialize $\comcbmat$ as the so-called (quantized) conjugate beamforming codebook
\begin{align}
\comcbmat = \project{\Arx}{\comrfcb}
\end{align}
which allows us to then solve
\begin{subequations} \label{eq:problem-tx}
	\begin{align}
	\min_{\precbmat} \ & \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:problem-objective-tx} \\
	\st 
	& \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-tx} \\
	% &\ \abs{\vectorize{\precbmat}} \leq \onevec{\Nt\Mt} \label{eq:problem-entry-tx}
	& \bars{\entry{\precbmat}{m,n}} \leq 1 \ \forall \ m,n \label{eq:problem-entry-tx}
	% &\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-tx}
	\end{align}
\end{subequations}
using a convex solver.
The solution to \eqref{eq:problem-tx} is then projected onto the set $\prerfcb$ as
\begin{align}
\precbmat = \project{\precbmat}{\prerfcb} \label{eq:project-pre}
\end{align}
Afterwards, we solve the following for $\comcbmat$ using this updated $\precbmat$.
\begin{subequations} \label{eq:problem-rx}
	\begin{align}
	\min_{\comcbmat} \ & \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:problem-objective-rx} \\
	\st
	& \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-rx} \\
	% & \abs{\vectorize{\comcbmat}} \leq \onevec{\Nr\Mr} \label{eq:problem-entry-rx} \\
	& \bars{\entry{\comcbmat}{m,n}} \leq 1 \ \forall \ m,n \label{eq:problem-entry-rx}
	% &\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-rx} 
	\end{align}
\end{subequations}
Upon solving \eqref{eq:problem-rx}, we project its solution onto the set of possible beamformers in $\comrfcb$ as
\begin{align}
\comcbmat = \project{\comcbmat}{\comrfcb} \label{eq:project-com}
\end{align}
We iteratively execute \eqref{eq:problem-tx}--\eqref{eq:project-com} $\Niter \geq 1$ times.
This alternating minimization approach to designing $\precbmat$ and $\comcbmat$ is summarized in \algref{alg:algorithm-full-altmin}.

\input{alg/algorithm-full-altmin.tex}
}

%We now introduce an additional tuning parameter that affords engineers another knob to turn in our design.
%It may be desirable to halt the minimization of $\normfro{\comcbmat\ctrans \Hsi \precbmat}^2$ before our coverage constraints are tight.
%That is, we may not want to further degrade the transmit or receive gain at the cost of additional minimization of beam coupling.
%This is especially true in settings where marginal gain is had in minimizing $\normfro{\comcbmat\ctrans \Hsi \precbmat}^2$ at the cost of significant losses to transmit or receive gain.
%Therefore, we introduce a $\powerrfmax$ as the maximum power our design aims to achieve across beam pairs on average.
%More formally, we desire 
%\begin{align}
%\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \leq \powerrfmax \cdot \Gt \cdot \Gr \label{eq:frobenius-rf-constraint}
%\end{align}
%which suggests that the average power contained by entries in $\comcbmat\ctrans \Hsi \precbmat$ is at most $\powerrfmax$.
%
%Using this, we reformulate our objective as
%\begin{align}
%\max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr}
%\end{align}
%leading to
%\begin{subequations} \label{eq:problem-i-full}
%	\begin{align}
%	\min_{\precbmat,\comcbmat} &\ \max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} \\
%	\st 
%	&\ \abs{\diag{\Atx\ctrans \precbmat}}^2 \geq \gtxmin \cdot \onevec{\Gt} \\
%	&\ \abs{\diag{\Arx\ctrans \comcbmat}}^2 \geq \grxmin \cdot \onevec{\Gr} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr 
%	\end{align}
%\end{subequations}
%Problem \eqref{eq:problem-i-full} is non-convex due to the coupling between $\precbmat$ and $\comcbmat$ in the objective and the non-convexity of $\prerfcb$ and $\comrfcb$.
%Taking an alternating minimization approach, we split \eqref{eq:problem-i-full} into
%\begin{subequations} \label{eq:problem-i-full-f}
%	\begin{align}
%	\min_{\precbmat} &\ \max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} \\
%	\st 
%	&\ \abs{\diag{\Atx\ctrans \precbmat}}^2 \geq \gtxmin \cdot \onevec{\Gt} \label{eq:problem-i-full-f-coverage} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-i-full-f-non-convex}
%	\end{align}
%\end{subequations}
%and
%\begin{subequations} \label{eq:problem-i-full-w}
%	\begin{align}
%	\min_{\comcbmat} & \ \max\braces{0,\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} \\
%	\st 
%	&\ \abs{\diag{\Arx\ctrans \comcbmat}}^2 \geq \grxmin \cdot \onevec{\Gr} \label{eq:problem-i-full-w-coverage} \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-i-full-w-non-convex}
%	\end{align}
%\end{subequations}
%which have convex objectives but have non-convex constraints per \eqref{eq:problem-i-full-f-non-convex} and \eqref{eq:problem-i-full-w-non-convex}.
%Notice that since
%\begin{align}
%\normfro{\mA} = \normfro{\mA\ctrans}
%\end{align}
%we can see that problems \eqref{eq:problem-i-full-f} and \eqref{eq:problem-i-full-w} are of the same form.
%Thus, an algorithm created to solve one can be used to solve the other, which we present as follows.
%
%Let us define the projection of a vector $\vx$ onto a set of vectors $\set{A}$ as
%\begin{align}
%\project{\vx}{\set{A}} = \arg \min_{\va \in \set{A}} \normtwo{\va - \vx}
%\end{align}
%and overload it to act column-wise on matrices as
%\begin{align}
%\entry{\project{\mX}{\set{A}}}{:,\ell} = \project{\entry{\mX}{:,\ell}}{\set{A}}
%\end{align}
%
%We take a projected gradient descent approach to solving \eqref{eq:problem-i-full-f} and \eqref{eq:problem-i-full-w}.
%We outline our algorithm as follows with notation of \eqref{eq:problem-i-full-f} with the understanding that it can also be used to solve \eqref{eq:problem-i-full-w} with a proper change of variables.
%Our algorithm, which is summarized in \algref{alg:algorithm-full-i}, begins by initializing $\precbmat$ and $\comcbmat$ as
%\begin{gather}
%\precbmat\node{1} = \precbmatinit = \project{\Atx}{\prerfcb} \\
%\comcbmat\node{1} = \comcbmatinit = \project{\Arx}{\comrfcb}
%\end{gather}
%where $\precbmat\node{n}$ and $\comcbmat\node{n}$ denote $\precbmat$ and $\comcbmat$ at the $n$-th gradient step.
%Let $\Niter$ be the number of iterations (gradient steps) that our algorithm takes.
%Let $\mu_\pre$ and $\mu_\com$ be the gradient step size during a gradient step of $\precbmat$ and $\comcbmat$, respectively.
%
%Noting that the gradient of the squared Frobenius norm is
%\begin{align}
%\nabla_{\mX} \normfro{\mA \mX}^2 = 2 \cdot \mA\ctrans \mA \mX
%\end{align}
%Thus, a gradient step on $\precbmat$ is defined as follows
%\begin{align}
%% \precbmat\node{n+1} = \precbmat\node{n} - \mu_{\pre} \cdot \mM_\pre \had \parens{2 \cdot \Hsi\ctrans \comcbmat\node{n} \comcbmat\ctransnode{n} \Hsi \precbmat\node{n}}
%\precbmat\node{n+1} = \precbmat\node{n} - \mu_{\pre} \cdot 2 \cdot \Hsi\ctrans \comcbmat\node{n} \comcbmat\ctransnode{n} \Hsi \precbmat\node{n} \label{eq:pre-gradient-step}
%\end{align}
%% where we refer to $\mM_\pre \in \setmatrixreal{\Nt}{\Gt}$ as a ``gradient mask'' that we will describe shortly.
%We then project $\precbmat\node{n+1}$ as
%\begin{align}
%\precbmat\node{n+1} = \project{\precbmat\node{n+1}}{\prerfcb}
%\end{align}
%Then, to ensure that the recent gradient step does not violate our transmit coverage constraint, we evaluate which beams have fallen below a transmit gain of $\gtxmin$
%\begin{align}
%\set{J}_\pre\node{n+1} = \braces{\ell : \entry{\precbmat\ctransnode{n+1} \Atx \Atx\ctrans \precbmat\node{n+1}}{\ell,\ell} < \gtxmin}
%\end{align}
%Using this index set, we revert columns index by $\set{J}_\pre\node{n+1}$ in $\precbmat\node{n+1}$ to those in the previous iteration.
%% Using this index set, we create a gradient mask matrix
%%\begin{align}
%%\entry{\mM_\pre}{:,\set{J}_\pre\node{n+1}} = \zeromat
%%\end{align}
%%which will be used to freeze the columns of $\precbmat$ that are FIX THIS, using gradient mask like this may be sub-optimal.
%\begin{align}
%\entry{\precbmat\node{n+1}}{:,\set{J}_\pre\node{n+1}} = \entry{\precbmat\node{n}}{:,\set{J}_\pre\node{n+1}} \label{eq:pre-step-back}
%\end{align}
%This ensures that the coverage constraint is maintained by $\precbmat\node{n+1}$, satisfying \eqref{eq:problem-i-full-f-coverage}.
%
%
%We repeat this process on the $n$-th gradient update of $\comcbmat$, which are summarized as follows.
%\begin{gather}
%\comcbmat\node{n+1} = \comcbmat\node{n} - \mu_{\com} \cdot 2 \cdot \Hsi \precbmat\node{n+1} \precbmat\ctransnode{n+1} \Hsi\ctrans \comcbmat\node{n} \label{eq:com-gradient-step} \\
%\comcbmat\node{n+1} = \project{\comcbmat\node{n+1}}{\comrfcb} \\
%\set{J}_\com\node{n+1} = \braces{\ell : \entry{\comcbmat\ctransnode{n+1} \Arx \Arx\ctrans \comcbmat\node{n+1}}{\ell,\ell} < \grxmin} \\
%\entry{\comcbmat\node{n+1}}{:,\set{J}_\com\node{n+1}} = \entry{\comcbmat\node{n}}{:,\set{J}_\com\node{n+1}} \label{eq:com-step-back}
%\end{gather}
%Note that the gradient step of the $n$-th step, as evidenced by \eqref{eq:com-gradient-step}, uses the already-updated $\precbmat\node{n+1}$ according to the alternating minimization approach we have taken.
%
%We now outline the exit criteria for our algorithm.
%At most, our algorithm concludes after $\Niter$ gradient updates.
%Otherwise, our algorithm halts when \eqref{eq:frobenius-rf-constraint} is met or when 
%\begin{align}
%\precbmat\node{n+1} = \precbmat\node{n} \label{eq:exit-criteria-static}
%\end{align}
%Note that \eqref{eq:exit-criteria-static} can happen when
%\begin{align}
%\card{\set{J}_\pre} = \Gt
%\end{align}
%and
%\begin{align}
%\card{\set{J}_\com} = \Gr
%\end{align}
%or when the gradient steps are so small (including zero) that they are effectively nullified during the projections onto $\prerfcb$ and $\comrfcb$.
%This places increased significance on the choices of $\mu_\pre$ and $\mu_\com$ and convergence to good solutions of $\precbmat$ and $\comcbmat$.

\comment{
---

\begin{gather}
\normtwo{\entry{\Atx}{:,\ell}}^2 = \Nt, \quad \ell = 1, \dots, \Mt \\
\normtwo{\entry{\Arx}{:,\ell}}^2 = \Nr, \quad \ell = 1, \dots, \Mr
\end{gather}

\begin{gather}
\normfro{\Atx}^2 = \Nt \cdot \Mt \\
\normfro{\Arx}^2 = \Nr \cdot \Mr
\end{gather}

\begin{gather}
\normtwo{\entry{\precbmat}{:,\ell}}^2 \leq \Nt, \quad \ell = 1, \dots, \Mt \\
\normtwo{\entry{\comcbmat}{:,\ell}}^2 \leq \Nr, \quad \ell = 1, \dots, \Mr
\end{gather}

\begin{gather}
\normfro{\precbmat}^2 \leq \Nt \cdot \Mt \\
\normfro{\comcbmat}^2 \leq \Nr \cdot \Mr
\end{gather}

\begin{gather}
\normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \leq \normfro{\comcbmat\ctrans}^2 \cdot \normfro{\Hsi}^2 \cdot \normfro{\precbmat}^2
\end{gather}

Let's say
\begin{gather}
\atx{\aod_\ell}\ctrans \vf_\ell = \Gtxtgt \ \forall \ \ell = 1, \dots, \Mt \\
\arx{\aoa_\ell}\ctrans \vw_\ell = \Grxtgt \ \forall \ \ell = 1, \dots, \Mr
\end{gather}

Then
\begin{align}
\normtwo{\arx{\aoa_\ell}\ctrans \vw_\ell} &= \Grxtgt \\
&\leq \normtwo{\arx{\aoa_\ell}} \cdot \normtwo{\vw_\ell}
\end{align}
so
\begin{align}
\normtwo{\vw_\ell} 
&\geq \frac{\Grxtgt}{\normtwo{\arx{\aoa_\ell}}} \\
&= \frac{\Grxtgt}{\sqrt{\Nr}} 
\end{align}
---
}

% \input{alg/algorithm-gradient-step.tex}

% \input{alg/algorithm-full-i.tex}


==> sec-contribution-ii-old.tex <==
\section{Robust Analog Beamforming Codebook Design under Imperfect Self-Interference Channel Knowledge} \label{sec:contribution-ii}

\subsection{Capturing Self-Interference Channel Errors}

In the previous section, our design relied on perfect channel knowledge of $\Hsi$.
Suppose instead of having direct knowledge of true over-the-air channel $\Hsi$, we have knowledge of its estimate $\Hsiest$ and knowledge of an estimation error bound.
Specifically, let us define the set of all possible $\Hsi$ as
\begin{align}
\Hsiset = \braces{\Hsi = \Hsiest + \Hsierror : \normfro{\Hsierror} \leq \epsilon}
\end{align}
where the matrix $\Hsierror$ captures the error in our estimate $\Hsiest$ and is bounded by its Frobenius norm as $\normfro{\Hsierror} \leq \epsilon$.
Note that other norm-bound errors can be encapsulated by appropriate choice of $\epsilon$ via norm equivalence.

\subsection{Assembling our Robust Codebook Design Problem}

Using this error model, we adjust our original design problem to take on the following minimax form, whereby we aim to minimize our objective (beam coupling) in the worst-case sense over all possible $\Hsi \in \Hsiset$.
%\begin{subequations} \label{eq:problem-full-2}
%	\begin{align}
%	\min_{\precbmat,\comcbmat} &\ \max_{\Hsi \in \Hsiset} \ \normfro{\comcbmat\ctrans \Hsi \precbmat}^2 \label{eq:problem-objective-2} \\
%	\st 
%	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-2} \\
%	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-2} \\
%	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-2} \\
%	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-2} 
%	\end{align}
%\end{subequations}
\begin{subequations} \label{eq:problem-full-2}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \max_{\normtwo{\Hsierror} \leq \epsilon} \ \normfro{\comcbmat\ctrans \parens{\Hsiest + \Hsierror} \precbmat} \label{eq:problem-objective-2} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-2} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-2} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-2} \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-2} 
	\end{align}
\end{subequations}
By solving \eqref{eq:problem-full-2}, $\precbmat$ and $\comcbmat$ will be designed such that they minimize the worst-case channel $\Hsi \in \Hsiset$ for a given $\Hsiest$ and $\epsilon$.
Note that only the objective depends on the $\Hsierror$ and that we have dropped the squared term from the objective for simplicity, which does not change the problem solution.
Unfortunately, \eqref{eq:problem-full-2} is difficult to solve due to the sandwiching of $\Hsi$ between $\comcbmat$ and $\precbmat$.
To approximately solve \eqref{eq:problem-full-2}, we take the following approach, which again relies on alternating minimization.

Let us first consider the design of $\precbmat$ for a fixed $\comcbmat$, which is captured in the following problem.
\begin{subequations} \label{eq:problem-full-3}
	\begin{align}
	\min_{\precbmat} &\ \max_{\normtwo{\Delta_{\channel}} \leq \epsilon} \ \normfro{\comcbmat\ctrans \parens{\Hsiest + \Delta_{\channel}} \precbmat} \label{eq:problem-objective-3} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-3} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-3}
	\end{align}
\end{subequations}
It is still difficult to solve this problem efficiently due to the coupling of $\comcbmat$ and $\Delta_{\channel}$.
% To remedy this, we make a slight adjustment to our problem as follows.

A common approach in worst-case robust optimization is to greatly simplify the problem by writing the resulting worst-case error in a closed-form fashion to eliminate the error term itself.
We take a similar approach.
It is difficult to find the error $\Hsierror$ that maximizes 
\begin{align}
\normfro{\comcbmat\ctrans \parens{\Hsiest + \Hsierror} \precbmat}
\end{align}
for a given $\precbmat$ and $\comcbmat$ due to the sandwiching of $\Hsi = \Hsiest + \Hsierror$.
Via the triangle identity, we have
\begin{align}
\normfro{\comcbmat\ctrans \parens{\Hsiest + \Hsierror} \precbmat} \leq \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \normfro{\comcbmat\ctrans \Hsierror \precbmat}
\end{align}
which allows us to adjust our problem to 
\begin{subequations} \label{eq:problem-full-4}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \max_{\normfro{\Hsierror} \leq \epsilon} \ \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \normfro{\comcbmat\ctrans \Hsierror \precbmat} \label{eq:problem-objective-4} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-4} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-4} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-4} \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-4} 
	\end{align}
\end{subequations}
which is will produce a solution that is more robust than the original problem.
Using the inequality
\begin{align}
\normfro{\mA \mB} \leq \normtwo{\mA} \cdot \normfro{\mB}
\end{align}
we can see that an upper bound can be written as
\begin{align}
\max_{\normfro{\Hsierror} \leq \epsilon} \ \normfro{\comcbmat\ctrans \Hsierror \precbmat} \leq \normtwo{\comcbmat} \cdot \normfro{\Hsierror} \cdot \normtwo{\precbmat}
\end{align}
which can be achieved when
\begin{align}
\Hsierror = \epsilon \cdot \vu \times \vv\ctrans
\end{align}
where $\vu$ is the right singular vector of $\comcbmat$ corresponding to its strongest singular value and $\vv$ is the left singular vector of $\precbmat$ corresponding to its strongest singular value.
This results in
\begin{align}
\normfro{\epsilon \comcbmat\ctrans \vu \vv\ctrans \precbmat} 
&= \epsilon \cdot \svmax{\comcbmat} \cdot \svmax{\precbmat} \\
&= \epsilon \cdot \normtwo{\comcbmat} \cdot \normtwo{\precbmat}
\end{align}

Therefore, we reformulate our problem \eqref{eq:problem-full-4} as
\begin{subequations} \label{eq:problem-full-5}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \epsilon \cdot \normtwo{\comcbmat} \normtwo{\precbmat} \label{eq:problem-objective-5} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-5} \\
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-5} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-5} \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-5} 
	\end{align}
\end{subequations}
which is only a function of $\epsilon$ and no longer a function of $\Hsierror$.
Note that our robust problem has taken on a regularizing form, as is common in handling worst-case robust optimization involving norms.

\subsection{Solving for our Robust Codebook}

We approach solving \eqref{eq:problem-full-5} with the same motivations from \secref{sec:contribution-i} where we take an projected alternating minimization methodology.
We split \eqref{eq:problem-full-5} into
\begin{subequations} \label{eq:problem-full-6}
	\begin{align}
	\min_{\precbmat} &\ \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \epsilon \cdot \normtwo{\comcbmat} \normtwo{\precbmat} \label{eq:problem-objective-6} \\
	\st 
	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mt \label{eq:problem-coverage-tx-6} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \label{eq:problem-quantize-tx-6}
	\end{align}
\end{subequations}
and
\begin{subequations} \label{eq:problem-full-7}
	\begin{align}
	\min_{\comcbmat} &\ \normfro{\comcbmat\ctrans \Hsiest \precbmat} + \epsilon \cdot \normtwo{\comcbmat} \normtwo{\precbmat} \label{eq:problem-objective-7} \\
	\st 
	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mr \label{eq:problem-coverage-rx-7} \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr \label{eq:problem-quantize-rx-7} 
	\end{align}
\end{subequations}
which are then iteratively solved a desired number of times, with projections in between as in \secref{sec:contribution-i}.
For the sake of brevity and with the similarities of the previous design methodology in mind, we summarize our robust design using the following algorithm.

\input{alg/algorithm-full-ii.tex}

==> sec-contribution-ii.tex <==
\section{Solving our Codebook Design} \label{sec:contribution-ii}

Having arrived at our design problem \eqref{eq:problem-full-3}, which can be used when considering both perfect ($\epsilon = 0$) and imperfect channel knowledge ($\epsilon > 0$), we now set out to solve for our design.
Unfortunately, problem \eqref{eq:problem-full-3} is non-convex due to the limited resolution of our digitally-controlled phase shifters and attenuators used for analog beamforming, captured by \eqref{eq:problem-quantize-tx-3} and \eqref{eq:problem-quantize-rx-3}.
\edit{Is the objective jointly convex?}

In general, we cannot handle this non-convexity by merely ignoring it, solving, and then projecting the solutions $\precbmat$ and $\comcbmat$ onto $\precb$ and $\comcb$, respectively, though this may offer reasonable results when $\bitsphase$ and $\bitsamp$ are sufficiently high (e.g., $8$ bits each).
To present a single, more general approach to handling this non-convexity when solving for our codebooks, we present the following alternating minimization.

We begin by separating problem \eqref{eq:problem-full-3} into problems \eqref{eq:problem-full-4a} and \eqref{eq:problem-full-4b}, which solve for the $i$-th transmit beam and $j$-th receive beam, respectively.
Problems \eqref{eq:problem-full-4a} and \eqref{eq:problem-full-4b}, which are of the same form, are convex since they remove the hardware constraints and can be readily solved using a convex solver (e.g., CVX was used in our numerical results).
In our implementation, we approximately solve problem \eqref{eq:problem-full-3} by solving for the entire codebook beam-by-beam. 
Let us define $\project{\mA}{\mathcal{A}}$ as the projection of the elements of $\mA$ onto the set $\mathcal{A}$.

Our design begins by initializing $\precbmat$ and $\comcbmat$ as the projections of scaled $\Atx$ and $\Arx$ onto $\precb$ and $\comcb$, respectively, effectively quantizing their entries according to the limited resolution of the phase shifters and attenuators used by the analog beamforming networks.
\begin{gather}
\precbmat \leftarrow \project{\Atx \cdot \Deltatx}{\precb} \\
\comcbmat \leftarrow \project{\Arx \cdot \Deltarx}{\comcb} 
\end{gather}
This initializes our transmit and receive beams to achieve gains $\Gtxtgt^2$ and $\Grxtgt^2$ in all transmit directions in $\dirtxset$ and receive directions in $\dirrxset$.

We solve for the $i$-th transmit beam $\vf_i$ by solving problem \eqref{eq:problem-full-4a}, where the first transmit beam uses the initialization of $\comcbmat$.
Note that we have introduced the constraint \eqref{eq:problem-entry-tx-4a} to ensure our beamforming weights can be implemented using attenuators.
\begin{subequations} \label{eq:problem-full-4a}
	\begin{align}
	\min_{\vf_i} &\ \normtwo{\comcbmat\ctrans \mH \vf_i} + \tilde{\epsilon} \cdot \sqrt{\Nt \Nr} \cdot \normtwo{\vf_i} \cdot \normtwo{\comcbmat} \label{eq:problem-objective-4a} \\
	\st 
	&\ \bars{\Gtxtgt - \atx{\dirtx\idx{i}}\ctrans \vf_i}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \label{eq:problem-coverage-tx-4a} \\
	&\ \bars{\entry{\vf_i}{n}} \leq 1 \ \forall \ n = 1, \dots, \Nt \label{eq:problem-entry-tx-4a}
	\end{align}
\end{subequations}
Then, the solution $\vf_i$ is projected onto the set $\precb$ before updating it in the matrix $\precbmat$.
\begin{align}
\entry{\precbmat}{:,i} \leftarrow \project{\vf_i}{\precb}
\end{align}
The updated $\precbmat$ is then used when solving for the $j$-th receive beam in problem \eqref{eq:problem-full-4b}.
\begin{subequations} \label{eq:problem-full-4b}
	\begin{align}
	\min_{\vw_j} &\ \normtwo{\vw_j\ctrans \mH \precbmat} + \tilde{\epsilon} \cdot \sqrt{\Nt \Nr} \cdot \normtwo{\precbmat} \cdot \normtwo{\vw_j} \label{eq:problem-objective-4b} \\
	\st 
	&\ \bars{\Grxtgt - \arx{\dirrx\idx{j}}\ctrans \vw_j}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \label{eq:problem-coverage-rx-4b} \\
	&\ \bars{\entry{\vw_j}{n}} \leq 1 \ \forall \  = 1, \dots, \Nr \label{eq:problem-entry-rx-4b} 
	\end{align}
\end{subequations}
The solution $\vw_j$ is then projected onto $\comcb$ before updating $\comcbmat$.
\begin{align}
\entry{\comcbmat}{:,j} \leftarrow \project{\vw_j}{\comcb}
\end{align}
We then iteratively solve for the $(i+1)$-th transmit beam and then the $(j+1)$-th receive beam until all $\Mtx$ and $\Mrx$ beams are solved for.
When $\Mtx = \Mrx$, the transmit and receive beams can be solved one after another.
When $\Mtx \neq \Mrx$, the remaining transmit/receive beams can be solved for after $\minop{\Mtx,\Mrx}$ iterations.

\subsection{Remarks}
We now present a few remarks on this approach and communicate our motivations and design decisions.
First, one benefit of this design is that it iteratively solves each transmit beam and receive beam one after another, rather than all transmit beams followed by all receive beams.
Empirically, we found that a full-fledged projected alternating minimization approach (i.e., solve for $\precbmat$, quantize, solve for $\comcbmat$, quantize, solve for $\precbmat$, quantize, ...), while seemingly superior, resulted in a bias since the first minimization (e.g., over the entire transmit codebook) would carry most of the weight in minimizing our objective.
This was worsened by projection-based quantization, which would trap our solutions in a solution that it could not escape even with more alternating minimization iterations.
Secondly, as mentioned, other designs that quantize the entire codebook at once can suffer more severely from quantization versus our solution which gradually incorporates quantization beam-by-beam, allowing later beams to react to the quantization imposed on earlier beams.

One of the artifacts of this design it does not jointly utilize the total codebook variance but rather satisfies a per-beam variance, meaning it has access to less flexibility in its codebook design but maintains the total variance nonetheless.

Furthermore, the nature of our design allows for two convenient features that may be useful in practice.
First, since our design has the ability to solve for individual beams while preserving the rest, it can be used to periodically update select beams.
This may be useful to account for service updates (e.g., increasing or decreasing gain/variance) or to incorporate updated channel information.
Secondly, an ordering of the codebook may be useful for engineers since it allows them to prioritize certain beams.
For example, transmit beams toward the end of the codebook enjoy the fact that many receive beams have already undergone their design to reduce interference, lessening its load and optimizing it for a receive codebook $\comcbmat$ that is close to the final one.
 
\input{alg/algorithm-v2.tex}

%\begin{subequations} \label{eq:problem-full-4a}
%	\begin{align}
%	\min_{\precbmat} &\ \normfro{\comcbmat\ctrans \mH \precbmat} + \epsilon \cdot \normtwo{\precbmat} \cdot \normtwo{\comcbmat} \label{eq:problem-objective-4a} \\
%	\st 
%	&\ \normtwo{\gtxtgt - \diag{\Atx\ctrans \precbmat}}^2 \leq \sigmatx^2 \cdot \Gtxtgt^2 \cdot \Mtx \label{eq:problem-coverage-tx-4a} \\
%	&\ \bars{\entry{\precbmat}{m,n}} \leq 1 \ \forall \ m,n \label{eq:problem-entry-tx-4a}
%	\end{align}
%\end{subequations}
%\begin{subequations} \label{eq:problem-full-4b}
%	\begin{align}
%	\min_{\comcbmat} &\ \normfro{\comcbmat\ctrans \mH \precbmat} + \epsilon \cdot \normtwo{\precbmat} \cdot \normtwo{\comcbmat} \label{eq:problem-objective-4b} \\
%	\st 
%	&\ \normtwo{\grxtgt - \diag{\Arx\ctrans \comcbmat}}^2 \leq \sigmarx^2 \cdot \Grxtgt^2 \cdot \Mrx \label{eq:problem-coverage-rx-4b} \\
%	&\ \bars{\entry{\comcbmat}{m,n}} \leq 1 \ \forall \ m,n \label{eq:problem-entry-rx-4b} 
%	\end{align}
%\end{subequations}

==> sec-contribution.tex <==
\section{Contribution I: Under a Per-Antenna Received Power Constraint} \label{sec:contribution}

Let us assume the $\aodset$ and $\aoaset$ are such that $\aod_1$ and $\aoa_1$ are the least important, meaning they can suffer from a potentially greater loss of beamforming gain.

\subsection{Under a per-antenna received power constraint, $\powerantmax < \infty$}
The entries of the product $\channel_{ii} \precbmat \in \setmatrixcomplex{\Nr\node{i}}{\Gt}$ represent the complex gains from the analog beamformer input to the antennas of the receive array at $i$.
To completely minimize the amount of self-interference reaching the receive array of $i$, the codebook \precbmat would be designed such that
\begin{align}
\channel_{ii} \precbmat = \zeromat \label{eq:ideal-cancel}
\end{align}
In other words, ever single \rf beamforming vector would completely avoid inflicting self-interference onto the receive array of $i$.
Such a design, however, likely leads to beams that are not useful for transmitting to $j$.
In fact, satisfying \eqref{eq:ideal-cancel} may be impossible even when $\precbmat$ is unconstrained (beyond the trivial $\precbmat = \zeromat$) since $\channel_{ii}$ does not necessarily have a null space.
The fact that we have not assumed a model for $\channel_{ii}$, means we must design $\precbmat$ without the expectation that it will be able to \textit{completely} eliminate self-interference.

An alternative approach would be to restrict the maximum power coupled by any antenna for any analog beamforming vector, resulting in the constraint
\begin{align}
\normmax{\channel_{ii} \precbmat}^2 \leq \powerantmax
\end{align}
where
\begin{align}
\normmax{\mA} = \max_{m,n} \ \bars{\entry{\mA}{m,n}}
\end{align}
is the magnitude of the maximum entry in a matrix $\mA$.
The $\mathrm{max}$-norm somewhat difficult to design over and may lead to a poor overall design of $\precbmat$.

With that being said, we choose to relax our objective by instead desiring that
\begin{align}
\normfro{\channel_{ii} \precbmat}^2 \leq \Nr\node{i} \cdot \Gt \cdot \powerantmax
\end{align}
where $\powerantmax$ is the average maximum power would like to couple per-antenna for each analog beamforming vector.


\subsection{Free from a per-antenna received power constraint, $\powerantmax = \infty$}
We also impose a constraint on the maximum power reaching the  that can be coupled by precoding and combining pairs.
Again, we would like our choices of 
In matrix form, we write this as
\begin{align}
\normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 \leq \powerrfmax
\end{align}


\subsection{Maintaining Transmission and Reception}
To ensure that transmission in the direction of $\aod_\ell$ is not degraded, we require that
\begin{align}
\bars{\atx{\aod_\ell}\ctrans \vf_\ell}^2 \geq \gtxmin \ \forall \ \ell = 1, \dots, \Gt
\end{align}
To ensure that reception in the direction of $\aoa_\ell$ is not degraded, we require that
\begin{align}
\bars{\arx{\aoa_\ell}\ctrans \vw_\ell}^2 \geq \grxmin \ \forall \ \ell = 1, \dots, \Gr
\end{align}


%\begin{subequations}
%	\begin{align}
%	\min_{\precbmat} &\ \max \braces{0,\normfro{\channel_{ii} \precbmat}^2 - \Nr\node{i} \cdot \Gt \cdot \powerantmax} \\
%	\st 
%	&\ \bars{\atx{\aod_\ell}\ctrans \vf_\ell}^2 \leq \gtx \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \vf_\ell \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt
%	\end{align}
%\end{subequations}
%
%
%\begin{subequations}
%	\begin{align}
%	\min_{\precbmat} &\ \normfro{\channel_{ii} \precbmat}^2 \\
%	\st 
%	&\ \bars{\atx{\aod_\ell}\ctrans \vf_\ell}^2 \leq \gtx \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \vf_\ell \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt
%	\end{align}
%\end{subequations}
%
%
%\begin{subequations}
%	\begin{align}
%	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 \\
%	\st 
%	&\ \bars{\atx{\aod_\ell}\ctrans \vf_\ell}^2 \leq \gtx \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \bars{\arx{\aoa_\ell}\ctrans \vw_\ell}^2 \leq \grx \ \forall \ \ell = 1, \dots, \Gr \\
%	&\ \vf_\ell \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \vw_\ell \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr
%	\end{align}
%\end{subequations}
%
%
%\begin{subequations}
%	\begin{align}
%	\min_{\comcbmat} &\ \normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 \\
%	\st 
%	&\ \bars{\arx{\aoa_\ell}\ctrans \vw_\ell}^2 \leq \grx \ \forall \ \ell = 1, \dots, \Gr \\
%	&\ \vw_\ell \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr
%	\end{align}
%\end{subequations}
%
%
%\begin{subequations}
%	\begin{align}
%	\min_{\precbmat} &\ \normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 \\
%	\st 
%	&\ \bars{\atx{\aod_\ell}\ctrans \vf_\ell}^2 \leq \etatx \ \forall \ \ell = 1, \dots, \Gt \\
%	&\ \vf_\ell \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt
%	\end{align}
%\end{subequations}


We define projection of a vector $\vx$ onto a set of vectors $\set{A}$ as
\begin{align}
\project{\vx}{\set{A}} = \arg \min_{\va \in \set{A}} \normtwo{\va - \vx}
\end{align}
and overload it to act column-wise on matrices as
\begin{align}
\entry{\project{\mX}{\set{A}}}{:,\ell} = \project{\entry{\mX}{:,\ell}}{\set{A}}
\end{align}

%\begin{align}
%\project{\mX}{\set{A}} = 
%\arg \min_{\mA} 
%& \ \normfro{\mA - \mX} \\
%\st & \ \entry{\mA}{:,\ell} \in \set{A} \ \forall \ \ell
%\end{align}

Ideally, we would like to solve the following optimization problem, which minimizes the total self-interference power coupled by all combinations of our \rf precoders and \rf combiners.
\begin{subequations}
	\begin{align}
	\min_{\precbmat,\comcbmat} &\ \normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 \\
	\st 
	&\ \abs{\diag{\Atx\ctrans \precbmat}} \geq \gtxmin \cdot \onevec{\Gt} \\
	&\ \abs{\diag{\Arx\ctrans \comcbmat}} \geq \grxmin \cdot \onevec{\Gr} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr 
	\end{align}
\end{subequations}
This is non-convex since the objective is non-convex when optimizing over $\precbmat$ and $\comcbmat$ together and $\prerfcb$ and $\comrfcb$ are not convex sets.

Since minimizing the total power in $\comcbmat\ctrans \channel_{ii} \precbmat$ may see diminishing returns as sacrifices are made in transmit and receive gain, we introduce a power threshold $\powerrfmax$ and aim to minimize
\begin{align}
\max \braces{0,\normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr} 
\end{align}
where $\powerrfmax$ is the maximum average power coupled by pairs of beams in $\precbmat$ and $\comcbmat$.
This objective will be minimized (equal $0$) when
\begin{align}
\normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 \leq \powerrfmax \cdot \Gt \cdot \Gr
\end{align}
halting the prices paid in transmit gain and receive gain.

Using this modified objective, we can rewrite our optimization problem as
\begin{subequations}
	\begin{align}
	\min_{\precbmat,\comcbmat} \ & \max \braces{0,\normfro{\comcbmat\ctrans \channel_{ii} \precbmat}^2 - \powerrfmax \cdot \Gt \cdot \Gr}  \\
	\st 
	&\ \abs{\diag{\Atx\ctrans \precbmat}} \geq \gtxmin \cdot \onevec{\Gt} \\
	&\ \abs{\diag{\Arx\ctrans \comcbmat}} \geq \grxmin \cdot \onevec{\Gr} \\
	&\ \entry{\precbmat}{:,\ell} \in \prerfcb \ \forall \ \ell = 1, \dots, \Gt \\
	&\ \entry{\comcbmat}{:,\ell} \in \comrfcb \ \forall \ \ell = 1, \dots, \Gr 
	\end{align}
\end{subequations}
As before, this problem remains non-convex.
In light of this, we present a method for approximately solving this problem.

We begin by making the following initializations.
\begin{gather}
\precbmat = \project{\Atx}{\prerfcb} \\
\comcbmat = \project{\Arx}{\comrfcb}
\end{gather}
We then decompose our problem as follows.

Let the following problem be used to solve for the $\ell$-th beamformer in $\precbmat$.
\begin{subequations} \label{eq:problem-f}
	\begin{align} 
	\entry{\precbmat}{:,\ell} = \arg \ \min_{\vf} \ & \max \braces{0,\normtwo{\comcbmat\ctrans \channel_{ii} \vf}^2 - \powerrfmax \cdot \Gr}  \\
	\st 
	&\ \abs{\atx{\aod_\ell}\ctrans \vf} \geq \gtxmin \\
	&\ \vf \in \prerfcb
	\end{align}
\end{subequations}
Similarly, let the following problem be used to solve for the $\ell$-th beamformer in $\comcbmat$.
\begin{subequations} \label{eq:problem-w}
	\begin{align} 
	\entry{\comcbmat}{:,\ell} = \arg \ \min_{\vw} \ & \max \braces{0,\normtwo{\vw\ctrans \channel_{ii} \precbmat}^2 - \powerrfmax \cdot \Gt}  \\
	\st 
	&\ \abs{\arx{\aoa_\ell}\ctrans \vw} \geq \grxmin \\
	&\ \vw \in \comrfcb
	\end{align}
\end{subequations}

Notice that \eqref{eq:problem-f} and \eqref{eq:problem-w} are of the same form, meaning a single algorithm can be used to solve them, though they are both non-convex.
We now outline our algorithm with the context of \eqref{eq:problem-f} in mind and the understanding that \eqref{eq:problem-w} could also be solved with slight adjustments.
We will explicitly state these adjustments after presenting our algorithm.

Our algorithm is summarized in \algref{alg:algorithm}.
We use a projected gradient descent approach to solve \eqref{eq:problem-f}.
Note that
\begin{align}
\normtwo{\comcbmat\ctrans \channel_{ii} \vf}^2 = \vf\ctrans \channel_{ii}\ctrans \comcbmat \comcbmat\ctrans \channel_{ii} \vf
\end{align}
The gradient of our objective is
\begin{align}
\nabla_{\vf} \ \vf\ctrans \channel_{ii}\ctrans \comcbmat \comcbmat\ctrans \channel_{ii} \vf = \channel_{ii}\ctrans \comcbmat \comcbmat\ctrans \channel_{ii} \vf
\end{align}
Let $\mu > 0$ be our gradient step size.
Let $\Niter > 0$ be the number of iterations (gradient steps) we will take.
Let $\vf\node{n}$ denote $\vf$ at the $n$-th iteration.
Our gradient update rule takes a familiar form as
\begin{align}
\vf\node{n+1} = \vf\node{n} - \mu \cdot \channel_{ii}\ctrans \comcbmat \comcbmat\ctrans \channel_{ii} \vf\node{n}
\end{align}
After applying the gradient update, project $\vf\node{n+1}$ onto $\prerfcb$ to ensure it satisfies our hardware constraints.
\begin{align}
\vf\node{n+1} = \project{\vf\node{n+1}}{\prerfcb}
\end{align}
We then evaluate the following
\begin{gather}
\bars{\entry{\Atx}{:,\ell}\ctrans \vf\node{n+1}} < \gtxmin \label{eq:stop-gain}\\
\normtwo{\comcbmat\ctrans \channel_{ii} \vf\node{n+1}}^2 \leq \Nr\node{i} \cdot \powerrfmax \label{eq:stop-power}
\end{gather}
If either \eqref{eq:stop-gain} or \eqref{eq:stop-power} are true or if the maximum number of iterations is reached, we end the optimization.
If \eqref{eq:stop-gain} is true, we take
\begin{align}
\entry{\precbmat}{:,\ell} = \vf\node{n}
\end{align}
to ensure the beamforming gain does not fall below $\gtxmin$.
Otherwise, we take
\begin{align}
\entry{\precbmat}{:,\ell} = \vf\node{n+1}
\end{align}

\input{alg/algorithm-v1.tex}

==> sec-introduction.tex <==
\section{Introduction} \label{sec:introduction}

Codebook-based analog beamforming is a critical component to the deployment of \mmwave systems.
Rather than measure the over-the-air channel and subsequently configure analog beamformers, practical \mmwave systems typically employ beam alignment to identify directions where energy should be steered to close the link between two devices.
Once promising directions have been identified, the analog beamforming network---which is comprised of many digitally controlled phase shifters and possibly attenuators---is configured via a lookup from a codebook of beams.
This offers a reduction in complexity and execution time versus setting each of the dozens of phase shifters (and attenuators) one-by-one.

Designing analog beamforming codebooks is relatively straightforward for half-duplex systems.
Depending on the phase shifter and attenuator resolution, number of antennas, and desired steering resolution, a set of highly directional beams that span the desired coverage region can be fairly easily designed.
Conjugate beamforming, for example, is a simple way to construct a set of beams that serve desired directions and only requires phase shifters, not attenuators.
With sufficient phase resolution, conjugate beams can provide full array gain in any desired direction.
Other designs leverage attenuators to shape beams that, for example, yield wider main lobes and suppress side lobes, which can help avoid loss due to beam misalignment and reduce interference, respectively.

Using analog beamforming codebooks that were designed for half-duplex settings may be undesirable in full-duplex settings.
This is because, at a full-duplex transceiver, the transmit and receive beams couple together via the self-interference channel. 
Off-the-shelf analog beamforming codebooks used for half-duplex, however, do not necessarily offer resilience to rejecting this self-interference---after all, they weren't designed for such.
This motivates us to design analog beamforming codebooks for full-duplex in mind; that is, codebooks that reject the self-interference channel between all transmit-receive beam pairs.
By doing so, improved isolation between the transmitter and receiver of a full-duplex device can improve the degree of self-interference mitigation afforded by analog beamforming.


---

Recent work on \mmwave full-duplex has shown that mitigating self-interference via beamforming alone is theoretically possible, meaning it may be feasible to achieve simultaneous transmission and reception in-band with little to no need for conventional strategies like analog or digital self-interference cancellation. 
To achieve this, many designs leverage both analog and digital beamforming.
However, a key bottleneck and impracticality for these designs is the configuration of analog beamformers.

As we will elaborate on, this motivates us design analog beamforming codebooks for \mmwave full-duplex.

In full-duplex transceivers, the transmit and receive beams couple together via the self-interference channel between its transmit and receive arrays.
Off-the-shelf analog beamforming codebooks used for half-duplex, however, do not necessarily offer resilience to rejecting self-interference.

---

Rather than measure the over-the-air channel, practical \mmwave systems typically employ beam alignment, whereby is configured to transmit or receive with high directional gain after identifying directions that 
the analog beamforming network 

---

\subsection{Prior Work and Motivation}



Do not account for beam alignment, assume perfect channel knowledge: 

Account for beam alignment: 

Phase shifters only: 

Infinite resolution phase shifters:



\subsection{Contributions}


\subsection{Notation}

==> sec-keywords.tex <==
\begin{keywords}
Millimeter-wave
\end{keywords}

==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

==> sec-problem-formulation-v2.tex <==
\section{Problem Formulation and Motivation} \label{sec:problem-formulation}

%\begin{figure}
%	\centering
%	\subfloat[Conventional codebook.]{\includegraphics[width=0.47\linewidth]{fig/placeholder}
%		\label{fig:matrix-cbf}}
%	\quad
%	\subfloat[Conventional codebook.]{\includegraphics[width=0.47\linewidth]{fig/placeholder}
%		\label{fig:matrix-cbf-2}} \\
%	\subfloat[Conventional codebook.]{\includegraphics[width=0.47\linewidth]{fig/placeholder}
%		\label{fig:matrix-cbf-3}}
%	\quad
%	\subfloat[Our codebook.]{\includegraphics[width=0.47\linewidth]{fig/placeholder}
%		\label{fig:matrix-ours}}
%	\caption{The magnitude of the beam coupling matrix $\comcbmat\ctrans \mH \precbmat$ for various codebooks.}
%	\label{fig:matrix}
%\end{figure}

Analog beamforming codebooks have become critical to successful deployment of \mmwave communication systems.
Rather than create beams arbitrarily throughout deployment, practical systems rely on relatively small sets of beams, from which a beam can be selected to serve a specific user.
While transmit beams $\vf$ are fundamentally limited to come from $\precb$ and likewise $\vw$ from $\comcb$, engineers establish smaller sets $\precbbar \subset \precb$ and $\comcbbar \subset \comcb$ from which $\vf$ and $\vw$ will be drawn, respectively.
We refer to the sizes of these codebooks as $\card{\precbbar} = \Mtx$ and $\card{\comcbbar} = \Mrx$, which are much smaller than their counterparts $\precb$ and $\comcb$. % given that
%\begin{gather}
%\card{\precbbar} = \Mtx \ll \card{\precb} = 2^{\Nt\cdot\parens{\bitsphase + \bitsamp}} \\
%\card{\comcbbar} = \Mrx \ll \card{\comcb} = 2^{\Nr\cdot\parens{\bitsphase + \bitsamp}}
%\end{gather}
The beams comprising the codebooks \precbbar and \comcbbar supply high beamforming gain to combat severe \mmwave path loss and achieve sufficient link margin.\footnote{In hierarchical codebooks, which are often used for initial access and beam alignment, $\precbbar$ and $\comcbbar$ refer to the finest tier of beams that are used for service.}
As such, a codebook of beams must provide adequate coverage over some service region to ensure that the location of a user within that region does not prevent it from being served.

Off-the-shelf codebooks for conventional half-duplex \mmwave systems are relatively straightforward to create and have been designed and implemented widely.
These codebooks, however, do not necessarily offer much robustness to self-interference since they were not designed with full-duplex in mind.
A transmit beam $\vf$ and receive beam $\vw$, chosen from codebooks $\precbbar$ and $\comcbbar$, couple together via the self-interference channel $\mH$.
Each transmit-receive beam pair will couple uniquely together, leading to various levels of self-interference.
Those well-aligned with the self-interference channel are prone to inflict and couple self-interference while those poorly aligned will naturally reject self-interference.
% Since transmit and receive beams are coupled through the self-interference channel, the two 
Intuitively, it seems that conventional codebooks would have beams that resist self-interference given the highly directional beams that dense \mmwave arrays can produce.
While somewhat accurate, this is not true for two key reasons:
\begin{itemize}
	\item Transmit and receive beams are coupled via self-interference channel $\mH$, meaning the orthogonality of interest is actually that between the beams and the channel rather than the beams themselves.
	\item The highly directional beams we are accustomed to are ``highly directional'' in the far-field but are not necessarily so in the near-field, where the transmit and receive arrays of a full-duplex device likely live.
\end{itemize}
This motivates us to design the codebooks $\precbbar$ and $\comcbbar$ with full-duplex in mind, such that self-interference is better rejected across all transmit-receive beam pairs.

To justify the construction of these codebooks, which are traditionally used as-is and are not often updated, we assume the self-interference channel $\mH$---much of which is unknown---satisfies one of the following:
\begin{itemize}
	\item The self-interference channel is estimated perfectly and is static. The matrix $\mH$ is known and remains fixed over time.
	\item The self-interference channel is estimated perfectly and is static over sufficiently long periods. The matrix $\mH$ can be perfectly estimated occasionally, remaining fixed over many service periods (e.g., hundreds or thousands of time slots).
	\item The self-interference channel is estimated accurately and is approximately static over sufficiently long periods. The matrix $\mH$ may change but does so relatively mildly over many service periods.
\end{itemize}
Practically, we imagine conducting thorough estimation of $\mH$ and execution of our design during initial installation/setup of the transceiver, where significant infrastructure and environmental factors can be implicitly accounted for in $\mH$.
Moreover, we imagine occasional, incremental updates can be made to our design and to the estimate of $\mH$, perhaps through creative full-duplex-inspired approaches that reduce resource overhead.
We imagine that laboratory testing and calibration along with thorough electromagnetic modeling/simulation and reliable self-interference channel models can aid and accelerate our design and reduce its associated overhead once deployed.
To summarize, we expect inspired future work can supplement and improve the design herein, which is relatively idealized and still distant from a deployment-ready solution.




==> sec-problem-formulation.tex <==
\section{Problem Formulation and Motivation} \label{sec:problem-formulation}



\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{fig/alignment/alignment_type_03.pdf}
	\caption{An illustration of the coverage regions that the transmitter and receiver aim to serve.}
	\label{fig:aod-aoa}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/nf_patterns_v3.eps}
	\caption{While extremely narrow beams produced by dense antenna arrays are ``extremely narrow'' in the far-field, they are not necessarily so in the near-field.}
	\label{fig:nf-patterns}
\end{figure}

% Analog beamforming codebooks are used for beam alignment in \fg cellular systems and IEEE 802.11ad/ay.

Rather than obtaining over-the-air channel knowledge between two devices in order to configure $\prerf$ and $\comrf$, practical systems like \fg cellular and IEEE 802.11ad/ay have turned to codebook-based beam alignment.
By taking this approach, promising analog beams (e.g., those that offer high \gls{snr}) are identified by searching through the codebook and measuring the power delivered to a device being served.
This results in a significant complexity reduction in designing $\prerf$ and $\comrf$ and simplifies channel estimation and initial access.
Clearly, searching through $\prerfcb$ or $\comrfcb$ exhaustively during beam alignment is highly impractical.
Therefore, it is much more practical to build significantly reduced codebooks $\prerfcbbar$ and $\comrfcbbar$ from which analog precoders and combiners are drawn.
With this being said, one can see that a codebook-based analog beamforming leaves very little room for optimization: the only flexibility the system has in configuring its analog beamformers is choosing from the entries in the codebook. \edit{Improve.}

Consider our full-duplex setting where the analog precoder couples with the analog combiner via the self-interference channel.
Some transmit-receive beam pairs will inherently afford more isolation than others.
To reduce the amount of self-interference reaching the receiver, it would be ideal if all beam pairs afforded high isolation.
It is unlikely, however, for this to be the case when using ``off-the-shelf'' codebooks---after all, they were not designed with full-duplex in mind.
One may be inclined to believe that the extremely narrow beams that have become ubiquitous in \mmwave would offer robustness to coupling because of their pencil-like shape.
This is, however, not necessarily the case because these extremely narrow beams are only ``extremely narrow'' in the far-field and not necessarily so in near-field.
This is evidenced by \figref{fig:nf-patterns}, where BLANK.
This motivates us to design an analog precoding codebook $\prerfcbbar$ and combining codebook $\comrfcbbar$ that together offer high isolation across all transmit-receive beam pairs to ensure that no matter which directions a device transmits and receives from, it sees a relatively low degree of coupled self-interference.

En route to reducing the amount of self-interference coupled by the analog precoding and combining codebooks, we must ensure that the beams within the codebooks remain useful in their ability to serve users.
Since \mmwave communication relies on high analog beamforming gains for sufficient link margin, beams are only useful if they offer high gain.
Additionally, since users may exist anywhere within a service region, a codebook of beams must collectively maintain coverage to the service region.
Conventional codebooks certainly satisfy this definition of ``usefulness'' by design as exhibited by \figref{fig:conventional-codebooks}, but do not offer much robustness to self-interference as exhibited by 

With $\bitsamp$ bits of amplitude control per attenuator and $\bitsphase$ bits of phase control per phase shifter, there are a total of $2^{\bitsamp + \bitsphase}$ different ways to configure a \textit{single} analog beamforming weight.
With $\Na$ antennas, there are $2^{\Na\cdot\parens{\bitsamp+\bitsphase}}$ different ways to configure an analog beamforming vector.
With $L$ \rf chains, there are $2^{L\cdot\Na\cdot\parens{\bitsamp+\bitsphase}}$ different ways to configure an analog beamforming matrix.
To design our codebook, clearly searching exhaustively through $\prerfcb$ or $\comrfcb$ for beams that supply good coverage with reduced self-interference coupling is impractical.
This motivates us to develop a systematic methodology to efficiently build our codebook, which we present in \secref{sec:design}.

\begin{figure*}[!t]
	\centering
	\subfloat[Precoding.]{\includegraphics[width=0.47\linewidth,height=0.9\textheight,keepaspectratio]{plots/5_bits/beams_1_tx.eps}}
	\quad
	\subfloat[Combining.]{\includegraphics[width=0.47\linewidth,height=0.9\textheight,keepaspectratio]{plots/5_bits/beams_1_rx.eps}}
	\caption{Example of conventional analog precoding and combining codebooks for a coverage region $[-60,60]$ degrees, where $\bitsphase = \bitsamp = 5$ bits. Each beam offers high gain and the collection of beams in a given codebook serves the coverage region.}
	\label{fig:conventional-codebooks}
\end{figure*}


%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/5_bits/matrix.eps}
%	\caption{Example demonstrating our codebook design, where $\Nt = \Nr = 32$, $\bitsamp = \bitsphase = 5$, $\channel_{ii}$ is Rayleigh faded, $5$ dB of BF loss allowed.}
%	\label{fig:matrix}
%\end{figure}
%
%
%\begin{figure*}[!t]
%	\centering
%	\subfloat[Conventional codebook.]{\includegraphics[width=0.47\linewidth,height=0.9\textheight,keepaspectratio]{plots/5_bits/beams_1_tx.eps}}
%	\quad
%	\subfloat[My codebook.]{\includegraphics[width=0.47\linewidth,height=0.9\textheight,keepaspectratio]{plots/5_bits/beams_2_tx.eps}}
%	\caption{5 bits.}
%\end{figure*}
%
%
%\begin{figure*}[!t]
%	\centering
%	\subfloat[Conventional codebook.]{\includegraphics[width=0.47\linewidth,height=0.9\textheight,keepaspectratio]{plots/5_bits/beams_1_rx.eps}}
%	\quad
%	\subfloat[My codebook.]{\includegraphics[width=0.47\linewidth,height=0.9\textheight,keepaspectratio]{plots/5_bits/beams_2_rx.eps}}
%	\caption{5 bits.}
%\end{figure*}
%
%
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/8_bits/matrix.eps}
%	\caption{8 bits.}
%\end{figure}
%
%
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/3_bits/matrix.eps}
%	\caption{3 bits.}
%\end{figure}
%
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.35\textheight,keepaspectratio]{plots/8_bits/cdf.eps}
%	\caption{8 bits.}
%\end{figure}
%
%
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.35\textheight,keepaspectratio]{plots/3_bits/cdf.eps}
%	\caption{3 bits.}
%\end{figure}
%
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/quant.eps}
%	\caption{Each of the possible complex values that a beamforming weight can take when $\bitsphase = \bitsamp = 5$ bits.}
%	\label{fig:}
%\end{figure}

==> sec-simulation-results-old.tex <==
\section{Numerical Results} \label{sec:simulation-results}

Show that this does better in full-duplex setting than conventional codebooks.
Show that this does well in half-duplex setting versus conventional codebooks.

% Show $\Ns = 1$ case. Show subarray case. Show fully-connected case.

Can show how it works as a function of $\kappa$ and in Rayleigh-faded channels.
Can also show how it works when $\kappa = -\infty$ for varying number of rays.

See how it does when only designing over NF portion but the true channel has NF + FF.

---

\subsection{Simulation}

To assess our design in a variety of conditions, we simulated it in a Monte Carlo fashion.
We used $32$-element, half-wavelength uniform linear arrays at the transmitter and receiver of our full-duplex device.

Since the self-interference channel currently lacks a confident model, we consider multiple channel types when when evaluating our design.

\subsubsection{Rayleigh-Faded Channel}
The consider the case when $\Hsi$ has Rayleigh-faded entries as
\begin{align}
\entry{\Hsi^{\mathrm{Ray}}}{m,n} \sim \distcgauss{0}{1} \ \forall \ m,n
\end{align}

\subsubsection{Spherical-Wave Near-Field Channel}
We also consider the following model, which has been a popular choice in existing \mmwave full-duplex literature to capture the close proximity that a transmit array and receive array are likely to exhibit.
\begin{align} \label{eq:si-channel-los}
\entry{\Hsi^{\mathrm{NF}}}{m,n} = \frac{\gamma}{r_{n,m}}\exp \left(-\j 2 \pi \frac{r_{n,m}}{\lambda} \right)
\end{align}
where $r_{n,m}$ is the distance between the $n$-th transmit antenna and the $m$-th receive antenna, $\lambda$ is the carrier wavelength, and $\gamma$ ensures that the channel is normalized such that $\normfro{\Hsi}^2 = \Nt\Nr$. 
Note that this near-field model is deterministic for a given relative array geometry.

\subsubsection{Reflective Far-Field Channel}
We also consider the case where the environment induces $\numrays$ reflections from the transmit array onto the receive array, which can be modelled as
\begin{align}
\Hsi^{\mathrm{FF}} = \sqrt{\frac{1}{\numrays}}
\sum_{u=1}^{\numrays} 
\beta_{u} \ 
\arx{\theta_{u}}
\atx{\phi_{u}}\ctrans
\end{align}
where $\beta_u$, $\theta_{u}$, and $\phi_{u}$ are the complex gain, \gls{aoa}, and \gls{aod} of the $u$-th reflection off the environment.


\subsubsection{Near-Field/Far-Field Rician Mixture}
\begin{align} \label{eq:si-channel-rice}
\Hsi^{\mathrm{mix}} = \sqrt{\frac{\kappa}{\kappa + 1}} \Hsi^{\mathrm{NF}} + \sqrt{\frac{1}{\kappa + 1}} \Hsi^{\mathrm{FF}}
\end{align}
where the Rician factor $\kappa$ captures the amount of power in the near-field portion relative to the far-field portion.
The near-field component is modeled using a spherical-wave model as $\left[\channel^{\textrm{NF}}_{ii}\right]_{v,u} = \frac{\gamma}{r_{u,v}}\exp \left(-\j 2 \pi \frac{r_{u,v}}{\lambda} \right)$, 

The far-field component captures reflections from the environment and is modeled using \eqref{eq:desired-channel} with $\numrays \sim \distuniform{1}{15}$.
The transmit and receive channels are modeled with $\numrays \sim \distuniform{4}{15}$.
For both channel models, each ray's \gls{aod} and \gls{aoa} are drawn from $\distuniform{-\pi/2}{\pi/2}$.

Recall that this work is not aiming to provide a codebook that can necessarily enable \mmwave full-duplex on its own but rather one that mitigates self-interference better than conventional codebooks.
Our codebook, for example, can be used in conjunction with a variety \mmwave full-duplex solutions such as:
\begin{itemize}
	\item hybrid beamforming approaches where digital precoding and combining can be used to supply additional self-interference mitigation
	\item approaches employing reduced-size analog self-interference cancellation
	\item approaches involving digital self-interference cancellation
\end{itemize}

\subsubsection{Conjugate Beamforming Codebook}

\subsubsection{Tapered Conjugate Beamforming Codebook}

% \subsection{Comparing our Design }

% \subsection{Evaluating our Design under Various Self-Interference Channel Models}

% \subsection{Confirming our Codebooks are Useful in a Half-Duplex Sense}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_v1-1.eps}
	\caption{Rayleigh-faded channel, averaged over 200 channels.}
	\label{fig:results-batch-v2-v1-1}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_v2-1.eps}
	\caption{Rayleigh-faded channel, averaged over 3 SI channels, 100 transmit channels.}
	\label{fig:results-batch-v2-v2-1}
\end{figure}

---

\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v2_process_v1-1.eps}
	\caption{Rayleigh-faded SI channel, averaged over 200 channels.}
	\label{fig:results-batch-v2-process-v1-1}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v2_process_v2-2.eps}
	\caption{Rayleigh-faded SI channel, averaged over 25 SI channels, 100 transmit channels.}
	\label{fig:results-batch-v2-process-v2-2}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v2_process_v2-4.eps}
	\caption{Rayleigh-faded SI channel, averaged over 25 SI channels, 100 receive channels.}
	\label{fig:results-batch-v2-process-v2-4}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v3_process_v1-1.eps}
	\caption{Mixed self-interference channel, averaged over 10 SI channels, $\sigma^2 = -30$ dB.}
	\label{fig:results-batch-v3-process-v1-1}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v3_process_v1-2.eps}
	\caption{Mixed self-interference channel, averaged over 10 SI channels, $\sigma^2 = -25$ dB.}
	\label{fig:results-batch-v3-process-v1-2}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v3_process_v1-3.eps}
	\caption{Mixed self-interference channel, averaged over 10 SI channels, $\sigma^2 = -20$ dB.}
	\label{fig:results-batch-v3-process-v1-3}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v3_process_v1-4.eps}
	\caption{Mixed self-interference channel, averaged over 10 SI channels, $\sigma^2 = -15$ dB.}
	\label{fig:results-batch-v3-process-v1-4}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v3_process_v1-5.eps}
	\caption{Mixed self-interference channel, averaged over 10 SI channels, $\sigma^2 = -10$ dB.}
	\label{fig:results-batch-v3-process-v1-5}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/results_batch_v4_process_v1-1.eps}
	\caption{Rayleigh-faded self-interference channel, averaged over 90 SI channels, $\Delta = -3$ dB, $\sigma^2 = -20$ dB.}
	\label{fig:results-batch-v4-process-v1-1}
\end{figure}

==> sec-simulation-results-v2.tex <==
\section{Numerical Results} \label{sec:simulation-results}
Now, we present a variety of numerical results from simulation to evaluate our design.
We begin this section by describing the details of our simulation and the self-interference channel models used.
Then, we introduce the metrics by which we will assess our design and existing codebook approaches that we will compare our design against.
We present numerical results under perfect self-interference channel knowledge, followed by presence of channel estimation errors.
Finally, we conclude with a summary of the key findings from these results.

\subsection{Simulation Details}
To assess our design in a variety of conditions, we simulated it in a Monte Carlo fashion.
We used $8 \times 8$ half-wavelength \upas for transmission and reception at our full-duplex transceiver.
Our default transmit and receive coverage regions are comprised of uniformly spaced points in azimuth from $-60^\circ$ to $60^\circ$ with $15^\circ$ spacing and in elevation from $-30^\circ$ to $30^\circ$ with $15^\circ$ spacing, which is illustrated in \figref{fig:dirset}.
This amounts to $\Mtx = \Mrx = 9 \times 5 = 45$ total directions in $\dirtxset$ and in $\dirrxset$.
We have assumed the analog beamforming networks use log-stepped attenuators with $0.25$ dB of (power) attenuation per \gls{lsb}.

% \subsection{Self-Interference Channel Models}
The choice of a particular self-interference channel model is a difficult one to justify practically given there currently lacks a well-accepted, measurement-backed model.
As such, we consider two channel models: (i) a Rayleigh-faded channel and (2) an idealized near-field model.
To ensure the channels are compared fairly, they each satisfy $\ev{\normfro{\mH}^2} = \Nt \Nr$, meaning only their spatial characteristics dictate our design's ability to reduce the coupling of self-interference, rather than the energy contained therein.

\subsubsection{Rayleigh-Faded Channel}
The first channel we have considered is a Rayleigh-faded channel described as 
\begin{align}
\entry{\mH}{m,n} \sim \distcgauss{0}{1} \ \forall \ m, n
\end{align}
Statistically, such a channel is a difficult one to design our codebook for.
This is because, statistically, its energy is evenly distributed over its spatial components and $\rank{\mH} = \minop{\Nt,\Nr}$ with probability 1.
Consequently, its input space spans $\setvectorcomplex{\Nt}$ and its output space spans $\setvectorcomplex{\Nr}$, making it difficult for our codebooks to avoid coupling with the self-interference channel at its input and its output.

\subsubsection{Idealized Near-Field Channel}
Given the likely close proximity of dense transmit and receive arrays within a full-duplex transceiver, there likely exists some near-field propagation between the two.
As a result, much existing \mmwave full-duplex work has relied on the spherical-wave channel model of \cite{spherical_2005} to capture ideal near-field coupling between elements of the arrays.
This model is deterministic for a given relative geometry between the transmit and receive arrays and can be summarized as
\begin{align}
\entry{\mH}{m,n} = \frac{\gamma}{r_{n,m}}\exp \left(-\j 2 \pi \frac{r_{n,m}}{\lambda} \right)
\end{align}
where $r_{n,m}$ is the distance between the $n$-th transmit antenna and the $m$-th receive antenna, $\lambda$ is the carrier wavelength, and $\gamma$ is a normalizing factor to satisfy $\normfro{\mH}^2 = \Nt\Nr$.
To realize such a channel, we have separated our transmit and receive arrays by $10 \lambda$ horizontally (in the azimuth plane).
While this model may not hold in practice, it provides us a sensible starting point to evaluate our design when the self-interference channel is dominated by near-field interaction.
In addition, it motivates the possibility that our design be executed on some deterministic or well estimated near-field model while treating imperfections (e.g., stemming from far-field reflections) as channel estimation error.


% to prevent these numerical results from being dominated by any spatial structure that may be inherent to other models (which themselves may be highly tied to a choice of relative transmit and receive array geometry).
% Other \mmwave full-duplex work has relied on a highly idealized spherical-wave model to capture near-field coupling between antennas and extensions that incorporate sparse reflections from the environment.
% In this work, we have chosen to use a Rayleigh-faded channel described as $\entry{\mH}{m,n} \sim \distcgauss{0}{1}$ to prevent these numerical results from being dominated by any spatial structure that may be inherent to other models (which themselves may be highly tied to a choice of relative transmit and receive array geometry).
% Other models may see performance improvement or degradation compared to the results shown herein; more relevant channel models can be used in future work to potentially modify and evaluate our design.


% -------------------------------------------------------------------------------------------------
% Metrics.
% -------------------------------------------------------------------------------------------------
\subsection{Metrics}

To quantitatively evaluate our design, we primarily use the following metrics:
\begin{itemize}
    \item $E$, the average coupling between beam pairs.
    \item $\Gtx^2(\theta)$ and $\Grx^2(\theta)$, the maximum transmit gain and receive gain delivered by our codebooks in a particular direction $\theta$.
\end{itemize}

The average beam coupling $E$, defined in \eqref{eq:power-si}, describes how much self-interference power is coupled by a transmit beam and receive beam from our codebook on average.
Recall that minimizing $E$ was the objective of our design approach.
In addition to the \textit{average} beam coupling, we will also look at the distribution of beam coupling across all pairs.

We refer to the maximum transmit gain delivered in the direction $\theta$ as $\Gtx^2(\theta)$, where $\theta$ is a direction encompassed by our transmit service region $\dirtxset$. 
In other words, if our codebook were to serve a user in the direction $\theta$ within the transmit service region, $\Gtx^2(\theta)$ is the gain provided by the gain-maximizing beam from our transmit codebook $\precbbar$ (i.e., $\precbmat$).
The maximum receive gain $\Grx^2(\theta)$ is defined analogously at the receiver.
$\Gtx^2(\theta)$ and $\Grx^2(\theta)$ can be expressed simply as
\begin{align}
\Gtx^2\parens{\theta} &= \max_{i} \bars{\entry{\atx{\theta}\ctrans\precbmat}{i}}^2 \\
\Grx^2\parens{\theta} &= \max_{j} \bars{\entry{\arx{\theta}\ctrans\comcbmat}{j}}^2
\end{align}
We emphasize that, for both, $\theta$ need not be a direction explicitly within $\dirtxset$ or $\dirrxset$, but rather be encompassed by the respective region.


% -------------------------------------------------------------------------------------------------
% Benchmarks.
% -------------------------------------------------------------------------------------------------
\subsection{Benchmarks}
Considering ours is the first known codebook design for \mmwave full-duplex, we evaluate our codebook design against the following three conventional codebooks:
\begin{itemize}
    \item conjugate beamforming (CBF)
    \item conjugate beamforming with Taylor windowing for $20$ dB of side lobe attenuation (CBF+Tay-20)
    \item conjugate beamforming with Taylor windowing for $40$ dB of side lobe attenuation (CBF+Tay-40)
\end{itemize}
Conjugate beamforming offers maximum beamforming gain with a narrow main lobe but exhibits high side lobe levels.
Taylor windowing reduces the side lobe levels at the cost of lessened beamforming gain and a wider main lobe.
% It is important to note that conjugate beamforming does not require amplitude control.
The beam pattern of each of our three codebooks is shown in \figref{fig:benchmarks-a}.
In \figref{fig:benchmarks-b}, we illustrate $\Gtx^2(\theta)$ (equivalently $\Grx^2(\theta)$) for each across the transmit coverage region.
Notice that CBF+Tay-20 and CBF+Tay-40 pay about $2$ dB and $5$ dB in beamforming gain, respectively.
To compare these benchmarks to our design, we can trivially scale them according to $\Deltatx^2$ and $\Deltarx^2$, which fairly accounts for the beamforming loss we permit our codebook to tolerate.
This will be more clear shortly.

% -------------------------------------------------------------------------------------------------
% Benchmarks' beam patterns, coverage plots.
% -------------------------------------------------------------------------------------------------

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_01}
%	\caption{The azimuth cut of a broadside beam from each of our three benchmark codebooks. Given our symmetric \upas, the azimuth and elevation cuts are identical.}
%	\label{fig:benchmarks}
%\end{figure}

\begin{figure*}
	\centering
	\subfloat[Azimuth beam pattern.]{\includegraphics[width=0.575\linewidth,height=0.34\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_01}
		\label{fig:benchmarks-a}}
	\qquad
	\subfloat[Coverage.]{\includegraphics[width=0.375\linewidth,height=0.36\textheight,keepaspectratio]{plots/v08/generate_v01_process_v08_fig_10}
		\label{fig:benchmarks-b}}
	\caption{The (a) azimuth beam patterns (elevation is identical) and (b) coverage offered by our benchmark codebooks.}
	\label{fig:benchmarks}
\end{figure*}


% -------------------------------------------------------------------------------------------------
% Perfect CSI.
% -------------------------------------------------------------------------------------------------
\subsection{Results under Perfect Channel Knowledge, $\epsilon = 0$}
We begin presenting our numerical results by considering perfect self-interference channel knowledge of $\mH$.
%
% -------------------------------------------------------------------------------------------------
% Delta vs E for various Sigma. Fixed bits.
% -------------------------------------------------------------------------------------------------
Let us first examine the performance of our design against various choices of $\Deltatx^2 = \Deltarx^2$ and $\sigmatx^2 = \sigmarx^2$, where $\bitsphase = \bitsamp = 5$ bits, in \figref{fig:batman}.
We have shown results for the Rayleigh and spherical-wave channels.
The three benchmarks are shown as dashed lines having slope of $2$ in this log-log scale.
This is simply because the average coupling $E$ decays by $2$ dB for each $1$ dB decrease in $\Deltatx^2 = \Deltarx^2$.
These benchmarks offer similar levels of $E$ across both channel types, which is not necessarily the case for all channel types \edit{(something to do with codebooks being full rank, spanning space)}.
The gap between the three benchmarks is similar but slightly more spread out in the Rayleigh channel.

In both channels, we can see that our design sees the steepest reduction in $E$ per $\Deltatx^2 = \Deltarx^2$ for $\Deltatx^2 = \Deltarx^2$ close to zero.
The slope is significantly sharper in both channels as compared to that of the conventional codebooks, suggesting that our design much better use of the tolerated beamforming loss in reducing self-interference.
This is thanks to the degrees of freedom that are made available to our design by even slight decreases in $\Deltatx^2 = \Deltarx^2$, which can be used to tackle self-interference.
Similarly, increasing the variances $\sigmatx^2 = \sigmarx^2$ provides even more flexibility to our design as it attempts to reshape beams that reduce coupling interference.

Once so many degrees of freedom are made available, the gains beyond which diminish to the point interference is no longer significantly reduced at the cost of $\Deltatx^2 = \Deltarx^2$.
One may ask why our design does not offer at least a slope of $2$ once arriving at a particular design---after all, couldn't our design merely scale with $\Deltatx^2 = \Deltarx^2$ to maintain a slope of $2$?
This would be the case when $\bitsamp \to \infty$ and is observed to be the case for even small increases beyond $\bitsamp = 5$ bits.

We can see that significantly more reduction in $E$ is possible in the spherical-wave channel; shortly, we will see even more is possible with increased $\bitsphase = \bitsamp$.
This is largely thanks to the fact that there exists more diversity in the strength of its spatial components, offering left and right null spaces (and relatively weak components) along which our design can attempt to pack our codebooks' beams.
The Rayleigh channel, on the other hand, will statistically distribute its energy across the entire input and output spaces.

\begin{figure*}
	\centering
	\subfloat[Rayleigh channel.]{\includegraphics[width=0.48\linewidth,height=0.27\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_03}\label{fig:batman-a}}
	\quad
	\subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.27\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_03}\label{fig:batman-b}}
	\caption{The average self-interference coupling $E$ as a function of $\Deltatx^2 = \Deltarx^2$ for various $\sigmatx^2 = \sigmarx^2$, where $\bitsphase = \bitsamp = 5$ bits. We are resolution-limited in (b) I think amplitude.}
	\label{fig:batman}
\end{figure*}


% -------------------------------------------------------------------------------------------------
% CDFs of coupling.
% -------------------------------------------------------------------------------------------------

%\begin{figure*}
%    \centering
%    \subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_12}\label{fig:hulk-a}}
%    \quad
%    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_12}\label{fig:hulk-b}}
%    \caption{The \gls{cdf} of beam coupling that our design achieves over combinations of $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
%    \label{fig:hulk}
%\end{figure*}


% -------------------------------------------------------------------------------------------------
% Coverage plots for various sigma. Fixed Delta, bits.
% -------------------------------------------------------------------------------------------------
Let us now look at the coverage supplied by a realization of our design in \figref{fig:spiderman}, which shows only the transmit coverage due to space constraints (receive coverage is very similar).
We have fixed $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.
For the Rayleigh channel, which is shown in \figref{fig:spiderman-a}, we can immediately see that a portion of the increased variance is used to reduce the gain delivered by all our beams.
This can be attributed to the fact that Rayleigh channels more evenly spread out energy over space.
Beams are being packed across the service region with much more non-uniformity as the variance increases.
Consequently, deeper nulls are present, which may be problematic when serving users.

In the spherical-wave channel, usage of the increased variance is more targeted, as some beams are reduced while others are preserved.
We can see that our transmit codebook is clearly reducing the energy steered in directions in front of the array but preserves those toward the left and right.
While perhaps somewhat counter-intuitive, steering in and around broadside happens to inflict more self-interference into this spherical-wave channel, even though our arrays are side-by-side.
This further illustrates the point made in \cite{roberts_wcm} that emphasizes that the notion of beam shapes deteriorates in near-field regimes.

\begin{figure*}
	\centering
	\subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.35\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_13b}\label{fig:spiderman-a}}
	\quad
	\subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.35\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_06b}\label{fig:spiderman-b}}
	\caption{The coverage supplied by a realization of our transmit codebook over the transmit service region $\dirtxset$ for various $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
	\label{fig:spiderman}
\end{figure*}


% -------------------------------------------------------------------------------------------------
% Coverage CDFs for various sigma. Fixed Delta, bits.
% -------------------------------------------------------------------------------------------------
While the scale used in the coverage plots of our benchmarks in \figref{fig:benchmarks-b} and of our design in \figref{fig:spiderman} is the same, it difficult to accurately compare the two.
As such, we have plotted the \gls{cdf} of this coverage in \figref{fig:superman} both channel types.
Coverage in the Rayleigh channel, shown in \figref{fig:superman-a}, we can see that our design does comparably well to the conventional codebooks, outperforming CBF+Tay-40 by nearly all accounts and CBF+Tay-20 by most accounts.
With low variance, our beams are required to deliver the target gain with little room for error, leading us to nearly match the coverage supplied by CBF.





\begin{figure*}
	\centering
	\subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_04}\label{fig:superman-a}}
	\quad
	\subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_04}\label{fig:superman-b}}
	\caption{The coverage \glspl{cdf} of a realization of our transmit codebook over the transmit service region $\dirtxset$ for various $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
	\label{fig:superman}
\end{figure*}


% -------------------------------------------------------------------------------------------------
% Median coverage vs E for various bits.
% -------------------------------------------------------------------------------------------------
Having outperformed our benchmarks in terms of $E$ and closely matching them in terms of coverage, we can see that our design is showing promise in \textit{simultaneously} delivering on both, which the benchmarks seem to fall short of: they can either offer high coverage at the cost of high $E$ or low $E$ at the cost of low coverage.
To better evaluate this, we plot $E$ versus median transmit gain $\Gtx^2(\theta)$ for our codebook over combinations of $\sigmatx^2 = \sigmarx^2$ and $\Deltatx^2 = \Deltarx^2$ for various $\bitsphase = \bitsamp$.
Each data point is reached by some choice of $\Deltatx^2 = \Deltarx^2$, $\sigmatx^2 = \sigmarx^2$, and $\bitsphase = \bitsamp$, where we have connected and colored dots based on $\bitsphase = \bitsamp$.
It is preferable to have a design that offers down (low $E$) and to the right (high median transmit gain).
We include the benchmark codebooks, which again decay at a rate of $2$ for the same reasoning as before (scaling the codebook also scales the median transmit gain).
Again, we show only transmit-side coverage for space considerations, though receive-side is observed to be nearly identical.
First, we can see that appreciable gains can be had by increasing $\bitsphase = \bitsamp$, particularly when more coverage loss is tolerated, for both channel types.

For the Rayleigh channel in \figref{fig:ironman-a}, we can see that maintaining a slope of $2$ can be achieved with $\bitsphase = \bitsamp \geq 7$ bits (particularly $\bitsamp$) and nearly so with $6$ bits.
This relationship of median transmit gain versus $E$ provide useful insights.
If a system requires a certain level of $E$ to reliably operate in a full-duplex fashion, we can see that our design can do so while offering much higher median transmit gain (and likewise receive gain).
For example, if $E = 20$ dB is required, our design achieves this while supplying median transmit gain of around $31$ dB while convention codebooks only offer around $26$ dB.
As the level of required $E$ decreases, the gap grows significantly until our design meets the ``$2$-slope'' or ``sub-$2$-slope'' regions.
If $E$ is required to be below $10$ dB, we can see that the transmit gain costs are quite high when $\bitsphase = \bitsamp = 5$ bits.
In such cases, we can see that it would be attractive to use $\bitsphase = \bitsamp \geq 6$ bits to preserve transmit gain.

Looking now at the spherical-wave channel in \figref{fig:ironman-b}, we can see that our design sees significant reduction in $E$ at the cost of transmit gain.
Notice that the $x$ and $y$ scales here are different than in in \figref{fig:ironman-a} and indicate that much more reduction in $E$ can be achieved and at less median transmit gain cost.
Again, higher resolution phase shifters and attenuators offer appreciable performance improvements, but the designs do not seem to reach a steady $2$-slope region.
This is likely due to any given design taking advantage of most (if not all) of the attenuators' dynamic range, meaning the cannot be merely scaled down indefinitely.
This does not seem to really be an issue because operation because our design severely outperforms conventional codebooks for practical requirements on median $\Gtx^2(\theta)$.

This leads us to another way to use this plot.
By defining a minimum median $\Gtx^2(\theta)$, we can observe the level of $E$ that our design can provide versus conventional codebooks.
For example, if $32$ dB of median transmit gain is required, our design can achieve more than $30$ dB of improvement in $E$ versus conventional codebooks.
The gap is even more substantial if $30$ dB of median transmit gain is tolerable and we have $\bitsphase = \bitsamp \geq 6$ bits.
We can see that higher resolution phase shifters and attenuators are only justified if the median transmit gain is less than $32$--$33$ dB.

\begin{figure*}
	\centering
	\subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v08/generate_v08_process_v01_fig_11}\label{fig:ironman-a}}
	\quad
	\subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_10}\label{fig:ironman-b}}
	\caption{The median transmit gain $\Gtx^2\parens{\theta}$ versus average coupling $E$ that our transmit codebook achieves over combinations of $\sigmatx^2 = \sigmarx^2$ and $\Deltatx^2 = \Deltarx^2$ for various $\bitsphase = \bitsamp$.}
	\label{fig:ironman}
\end{figure*}


% -------------------------------------------------------------------------------------------------
% Imperfect CSI.
% -------------------------------------------------------------------------------------------------
\subsection{Results under Imperfect Self-Interference Channel Estimation, $\epsilon > 0$}
We now consider the case of imperfect knowledge of the self-interference channel $\mH$.
%
% -------------------------------------------------------------------------------------------------
% Median coverage vs E for various bits.
% -------------------------------------------------------------------------------------------------
To do so concisely, we directly consider \figref{fig:bane}, which shows median transmit gain versus $E$ for various levels of channel uncertainty $\epsilon$.
To produce a design for a given $\epsilon$, we evaluated multiple $\tilde{\epsilon}$ to choose the one offering the best robustness on average.
We found that $\tilde{\epsilon}$ was typically $10$--$15$ lower than $\epsilon$, which is an artifact of our worst-case design approach, as mentioned in outlining our design.
In practice, this can be experimented with offline to better choose $\tilde{\epsilon}$ directly based on an estimate of $\epsilon$.

We can see that our design does show some robustness to channel uncertainty in both channel 

Hopefully the self-interference channel can be accurately estimated during calibration/installation and throughout system deployment, leveraging the fact that feedback is free between the transmit and receive arrays of the full-duplex transceiver, the strength of the self-interference channel to yield high-\gls{snr} measurements, and perhaps by taking advantage of novel, low-overhead channel estimation strategies during half-duplex operation.

\begin{figure*}
    \centering
    \subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_07}\label{fig:bane-a}}
    \quad
    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v30/generate_v30_process_v01_fig_07}\label{fig:bane-b}}
    \caption{The median transmit gain $\Gtx^2\parens{\theta}$ versus average coupling $E$ that our transmit codebook achieves over combinations of $\sigmatx^2 = \sigmarx^2$ and $\Deltatx^2 = \Deltarx^2$ for various $\epsilon$.}
    \label{fig:bane}
\end{figure*}



==> sec-simulation-results-v3.tex <==
\section{Numerical Results} \label{sec:simulation-results}
Now, we present a variety of numerical results from simulation to evaluate our design.
We begin this section by describing the details of our simulation and the self-interference channel models used.
Then, we introduce the metrics by which we will assess our design and existing codebook approaches that we will compare our design against.
We present numerical results under perfect self-interference channel knowledge, followed by presence of channel estimation errors.
Finally, we conclude with a summary of the key findings from these results.

\subsection{Simulation Details}
To assess our design in a variety of conditions, we simulated it in a Monte Carlo fashion.
We used $8 \times 8$ half-wavelength \upas for transmission and reception at our full-duplex transceiver.
Our default transmit and receive coverage regions are comprised of uniformly spaced points in azimuth from $-60^\circ$ to $60^\circ$ with $15^\circ$ spacing and in elevation from $-30^\circ$ to $30^\circ$ with $15^\circ$ spacing, which is illustrated in \figref{fig:dirset}.
This amounts to $\Mtx = \Mrx = 9 \times 5 = 45$ total directions in $\dirtxset$ and in $\dirrxset$.
We have assumed the analog beamforming networks use log-stepped attenuators with $0.25$ dB of (power) attenuation per \gls{lsb}.

% \subsection{Self-Interference Channel Models}
The choice of a particular self-interference channel model is a difficult one to justify practically given there currently lacks a well-accepted, measurement-backed model.
As such, we consider two channel models: (i) a Rayleigh-faded channel and (2) an idealized near-field model.
To ensure the channels are compared fairly, they each satisfy $\ev{\normfro{\mH}^2} = \Nt \Nr$, meaning only their spatial characteristics dictate our design's ability to reduce the coupling of self-interference, rather than the energy contained therein.

\subsubsection{Rayleigh-Faded Channel}
The first channel we have considered is a Rayleigh-faded channel described as 
\begin{align}
\entry{\mH}{m,n} \sim \distcgauss{0}{1} \ \forall \ m, n
\end{align}
Statistically, such a channel is a difficult one to design our codebook for.
This is because, statistically, its energy is evenly distributed over its spatial components and $\rank{\mH} = \minop{\Nt,\Nr}$ with probability 1.
Consequently, its input space spans $\setvectorcomplex{\Nt}$ and its output space spans $\setvectorcomplex{\Nr}$, making it difficult for our codebooks to avoid coupling with the self-interference channel at its input and its output.

\subsubsection{Idealized Near-Field Channel}
Given the likely close proximity of dense transmit and receive arrays within a full-duplex transceiver, there likely exists some near-field propagation between the two.
As a result, much existing \mmwave full-duplex work has relied on the spherical-wave channel model of \cite{spherical_2005} to capture ideal near-field coupling between elements of the arrays.
This model is deterministic for a given relative geometry between the transmit and receive arrays and can be summarized as
\begin{align}
\entry{\mH}{m,n} = \frac{\gamma}{r_{n,m}}\exp \left(-\j 2 \pi \frac{r_{n,m}}{\lambda} \right)
\end{align}
where $r_{n,m}$ is the distance between the $n$-th transmit antenna and the $m$-th receive antenna, $\lambda$ is the carrier wavelength, and $\gamma$ is a normalizing factor to satisfy $\normfro{\mH}^2 = \Nt\Nr$.
To realize such a channel, we have separated our transmit and receive arrays by $10 \lambda$ horizontally (in the azimuth plane).
While this model may not hold in practice, it provides us a sensible starting point to evaluate our design when the self-interference channel is dominated by near-field interaction.
In addition, it motivates the possibility that our design be executed on some deterministic or well estimated near-field model while treating imperfections (e.g., stemming from far-field reflections) as channel estimation error.


% to prevent these numerical results from being dominated by any spatial structure that may be inherent to other models (which themselves may be highly tied to a choice of relative transmit and receive array geometry).
% Other \mmwave full-duplex work has relied on a highly idealized spherical-wave model to capture near-field coupling between antennas and extensions that incorporate sparse reflections from the environment.
% In this work, we have chosen to use a Rayleigh-faded channel described as $\entry{\mH}{m,n} \sim \distcgauss{0}{1}$ to prevent these numerical results from being dominated by any spatial structure that may be inherent to other models (which themselves may be highly tied to a choice of relative transmit and receive array geometry).
% Other models may see performance improvement or degradation compared to the results shown herein; more relevant channel models can be used in future work to potentially modify and evaluate our design.

% -------------------------------------------------------------------------------------------------
% Metrics.
% -------------------------------------------------------------------------------------------------
\subsection{Metrics}

\begin{align}
\setxfd &= \logtwo{1 + \frac{\snrtx}{\Nt} \bars{\vhtx\ctrans \vf}^2}
\end{align}

\begin{align}
	\serxfd &= \logtwo{1 + \frac{\snrrx \cdot \bars{\vw\ctrans \vhrx}^2}{1 + \inr \cdot \bars{\vw\ctrans \mH \vf}^2}}
\end{align}

\begin{align}
\inr = \frac{P \cdot G^2}{\noisevar}
\end{align}

\begin{align}
	\sinrrx = \frac{\snrrx}{1 + \inr}
\end{align}

% -------------------------------------------------------------------------------------------------
% Metrics.
% -------------------------------------------------------------------------------------------------
\subsection{Metrics}

To quantitatively evaluate our design, we primarily use the following metrics:
\begin{itemize}
    \item $E$, the average coupling between beam pairs.
    \item $\Gtx^2(\theta)$ and $\Grx^2(\theta)$, the maximum transmit gain and receive gain delivered by our codebooks in a particular direction $\theta$.
\end{itemize}

The average beam coupling $E$, defined in \eqref{eq:power-si}, describes how much self-interference power is coupled by a transmit beam and receive beam from our codebook on average.
Recall that minimizing $E$ was the objective of our design approach.
In addition to the \textit{average} beam coupling, we will also look at the distribution of beam coupling across all pairs.

We refer to the maximum transmit gain delivered in the direction $\theta$ as $\Gtx^2(\theta)$, where $\theta$ is a direction encompassed by our transmit service region $\dirtxset$. 
In other words, if our codebook were to serve a user in the direction $\theta$ within the transmit service region, $\Gtx^2(\theta)$ is the gain provided by the gain-maximizing beam from our transmit codebook $\precbbar$ (i.e., $\precbmat$).
The maximum receive gain $\Grx^2(\theta)$ is defined analogously at the receiver.
$\Gtx^2(\theta)$ and $\Grx^2(\theta)$ can be expressed simply as
\begin{align}
\Gtx^2\parens{\theta} &= \max_{i} \bars{\entry{\atx{\theta}\ctrans\precbmat}{i}}^2 \\
\Grx^2\parens{\theta} &= \max_{j} \bars{\entry{\arx{\theta}\ctrans\comcbmat}{j}}^2
\end{align}
We emphasize that, for both, $\theta$ need not be a direction explicitly within $\dirtxset$ or $\dirrxset$, but rather be encompassed by the respective region.


% -------------------------------------------------------------------------------------------------
% Benchmarks.
% -------------------------------------------------------------------------------------------------
\subsection{Benchmarks}
Considering ours is the first known codebook design for \mmwave full-duplex, we evaluate our codebook design against the following three conventional codebooks:
\begin{itemize}
    \item conjugate beamforming (CBF)
    \item conjugate beamforming with Taylor windowing for $20$ dB of side lobe attenuation (CBF+Tay-20)
    \item conjugate beamforming with Taylor windowing for $40$ dB of side lobe attenuation (CBF+Tay-40)
\end{itemize}
Conjugate beamforming offers maximum beamforming gain with a narrow main lobe but exhibits high side lobe levels.
Taylor windowing reduces the side lobe levels at the cost of lessened beamforming gain and a wider main lobe.
% It is important to note that conjugate beamforming does not require amplitude control.
The beam pattern of each of our three codebooks is shown in \figref{fig:benchmarks-a}.
In \figref{fig:benchmarks-b}, we illustrate $\Gtx^2(\theta)$ (equivalently $\Grx^2(\theta)$) for each across the transmit coverage region.
Notice that CBF+Tay-20 and CBF+Tay-40 pay about $2$ dB and $5$ dB in beamforming gain, respectively.
To compare these benchmarks to our design, we can trivially scale them according to $\Deltatx^2$ and $\Deltarx^2$, which fairly accounts for the beamforming loss we permit our codebook to tolerate.
This will be more clear shortly.

% -------------------------------------------------------------------------------------------------
% Benchmarks' beam patterns, coverage plots.
% -------------------------------------------------------------------------------------------------

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.25\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_01}
%	\caption{The azimuth cut of a broadside beam from each of our three benchmark codebooks. The elevation cuts are identical.}
%	\label{fig:benchmarks}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v02_fig_08.eps}
    \caption{The azimuth cut of a broadside beam from each of our three benchmark codebooks. The elevation cuts are identical.}
    \label{fig:benchmarks}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v02_fig_07.eps}
    \caption{Caption.}
    \label{fig:}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v02_fig_03.pdf}
    \caption{Caption.}
    \label{fig:}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v02_fig_04.pdf}
    \caption{Caption.}
    \label{fig:}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v02_fig_05.pdf}
	\caption{Caption.}
	\label{fig:}
\end{figure}

%\begin{figure*}
%    \centering
%    \subfloat[Azimuth beam pattern.]{\includegraphics[width=0.575\linewidth,height=0.34\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_01}
%        \label{fig:benchmarks-a}}
%    \qquad
%    \subfloat[Coverage.]{\includegraphics[width=0.375\linewidth,height=0.36\textheight,keepaspectratio]{plots/v08/generate_v01_process_v08_fig_10}
%        \label{fig:benchmarks-b}}
%    \caption{The (a) azimuth beam patterns (elevation is identical) and (b) coverage offered by our benchmark codebooks.}
%    \label{fig:benchmarks}
%\end{figure*}


% -------------------------------------------------------------------------------------------------
% Perfect CSI.
% -------------------------------------------------------------------------------------------------
\subsection{Results under Perfect Channel Knowledge, $\epsilon = 0$}
We begin presenting our numerical results by considering perfect self-interference channel knowledge of $\mH$.
%
% -------------------------------------------------------------------------------------------------
% Delta vs E for various Sigma. Fixed bits.
% -------------------------------------------------------------------------------------------------
Let us first examine the performance of our design against various choices of $\Deltatx^2 = \Deltarx^2$ and $\sigmatx^2 = \sigmarx^2$, where $\bitsphase = \bitsamp = 5$ bits, in \figref{fig:batman}.
We have shown results for the Rayleigh and spherical-wave channels.
The three benchmarks are shown as dashed lines having slope of $2$ in this log-log scale.
This is simply because the average coupling $E$ decays by $2$ dB for each $1$ dB decrease in $\Deltatx^2 = \Deltarx^2$.
These benchmarks offer similar levels of $E$ across both channel types, which is not necessarily the case for all channel types \edit{(something to do with codebooks being full rank, spanning space)}.
The gap between the three benchmarks is similar but slightly more spread out in the Rayleigh channel.

In both channels, we can see that our design sees the steepest reduction in $E$ per $\Deltatx^2 = \Deltarx^2$ for $\Deltatx^2 = \Deltarx^2$ close to zero.
The slope is significantly sharper in both channels as compared to that of the conventional codebooks, suggesting that our design much better use of the tolerated beamforming loss in reducing self-interference.
This is thanks to the degrees of freedom that are made available to our design by even slight decreases in $\Deltatx^2 = \Deltarx^2$, which can be used to tackle self-interference.
Similarly, increasing the variances $\sigmatx^2 = \sigmarx^2$ provides even more flexibility to our design as it attempts to reshape beams that reduce coupling interference.

Once so many degrees of freedom are made available, the gains beyond which diminish to the point interference is no longer significantly reduced at the cost of $\Deltatx^2 = \Deltarx^2$.
One may ask why our design does not offer at least a slope of $2$ once arriving at a particular design---after all, couldn't our design merely scale with $\Deltatx^2 = \Deltarx^2$ to maintain a slope of $2$?
This would be the case when $\bitsamp \to \infty$ and is observed to be the case for even small increases beyond $\bitsamp = 5$ bits.

We can see that significantly more reduction in $E$ is possible in the spherical-wave channel; shortly, we will see even more is possible with increased $\bitsphase = \bitsamp$.
This is largely thanks to the fact that there exists more diversity in the strength of its spatial components, offering left and right null spaces (and relatively weak components) along which our design can attempt to pack our codebooks' beams.
The Rayleigh channel, on the other hand, will statistically distribute its energy across the entire input and output spaces.

%\begin{figure*}
%    \centering
%    \subfloat[Rayleigh channel.]{\includegraphics[width=0.48\linewidth,height=0.27\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_03}\label{fig:batman-a}}
%    \quad
%    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.27\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_03}\label{fig:batman-b}}
%    \caption{The average self-interference coupling $E$ as a function of $\Deltatx^2 = \Deltarx^2$ for various $\sigmatx^2 = \sigmarx^2$, where $\bitsphase = \bitsamp = 5$ bits. We are resolution-limited in (b) I think amplitude.}
%    \label{fig:batman}
%\end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_03}
    \caption{The average self-interference coupling $E$ as a function of $\Deltatx^2 = \Deltarx^2$ for various $\sigmatx^2 = \sigmarx^2$, where $\bitsphase = \bitsamp = 5$ bits. We are resolution-limited in (b) I think amplitude.}
    \label{fig:batman-b}
\end{figure}

% -------------------------------------------------------------------------------------------------
% CDFs of coupling.
% -------------------------------------------------------------------------------------------------

%\begin{figure*}
%    \centering
%    \subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_12}\label{fig:hulk-a}}
%    \quad
%    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_12}\label{fig:hulk-b}}
%    \caption{The \gls{cdf} of beam coupling that our design achieves over combinations of $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
%    \label{fig:hulk}
%\end{figure*}


% -------------------------------------------------------------------------------------------------
% Coverage plots for various sigma. Fixed Delta, bits.
% -------------------------------------------------------------------------------------------------
Let us now look at the coverage supplied by a realization of our design in \figref{fig:spiderman}, which shows only the transmit coverage due to space constraints (receive coverage is very similar).
We have fixed $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.
For the Rayleigh channel, which is shown in \figref{fig:spiderman-a}, we can immediately see that a portion of the increased variance is used to reduce the gain delivered by all our beams.
This can be attributed to the fact that Rayleigh channels more evenly spread out energy over space.
Beams are being packed across the service region with much more non-uniformity as the variance increases.
Consequently, deeper nulls are present, which may be problematic when serving users.

In the spherical-wave channel, usage of the increased variance is more targeted, as some beams are reduced while others are preserved.
We can see that our transmit codebook is clearly reducing the energy steered in directions in front of the array but preserves those toward the left and right.
While perhaps somewhat counter-intuitive, steering in and around broadside happens to inflict more self-interference into this spherical-wave channel, even though our arrays are side-by-side.
This further illustrates the point made in \cite{roberts_wcm} that emphasizes that the notion of beam shapes deteriorates in near-field regimes.

%\begin{figure*}
%    \centering
%    \subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.35\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_13b}\label{fig:spiderman-a}}
%    \quad
%    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.35\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_06b}\label{fig:spiderman-b}}
%    \caption{The coverage supplied by a realization of our transmit codebook over the transmit service region $\dirtxset$ for various $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
%    \label{fig:spiderman}
%\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_06b}
    \caption{The coverage supplied by a realization of our transmit codebook over the transmit service region $\dirtxset$ for various $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
    \label{fig:spiderman-b}
\end{figure}

% -------------------------------------------------------------------------------------------------
% Coverage CDFs for various sigma. Fixed Delta, bits.
% -------------------------------------------------------------------------------------------------
%While the scale used in the coverage plots of our benchmarks in \figref{fig:benchmarks-b} and of our design in \figref{fig:spiderman} is the same, it difficult to accurately compare the two.
%As such, we have plotted the \gls{cdf} of this coverage in \figref{fig:superman} both channel types.
%Coverage in the Rayleigh channel, shown in \figref{fig:superman-a}, we can see that our design does comparably well to the conventional codebooks, outperforming CBF+Tay-40 by nearly all accounts and CBF+Tay-20 by most accounts.
%With low variance, our beams are required to deliver the target gain with little room for error, leading us to nearly match the coverage supplied by CBF.





%\begin{figure*}
%    \centering
%    \subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_04}\label{fig:superman-a}}
%    \quad
%    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_04}\label{fig:superman-b}}
%    \caption{The coverage \glspl{cdf} of a realization of our transmit codebook over the transmit service region $\dirtxset$ for various $\sigmatx^2 = \sigmarx^2$, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.}
%    \label{fig:superman}
%\end{figure*}


% -------------------------------------------------------------------------------------------------
% Median coverage vs E for various bits.
% -------------------------------------------------------------------------------------------------
Having outperformed our benchmarks in terms of $E$ and closely matching them in terms of coverage, we can see that our design is showing promise in \textit{simultaneously} delivering on both, which the benchmarks seem to fall short of: they can either offer high coverage at the cost of high $E$ or low $E$ at the cost of low coverage.
To better evaluate this, we plot $E$ versus median transmit gain $\Gtx^2(\theta)$ for our codebook over combinations of $\sigmatx^2 = \sigmarx^2$ and $\Deltatx^2 = \Deltarx^2$ for various $\bitsphase = \bitsamp$.
Each data point is reached by some choice of $\Deltatx^2 = \Deltarx^2$, $\sigmatx^2 = \sigmarx^2$, and $\bitsphase = \bitsamp$, where we have connected and colored dots based on $\bitsphase = \bitsamp$.
It is preferable to have a design that offers down (low $E$) and to the right (high median transmit gain).
We include the benchmark codebooks, which again decay at a rate of $2$ for the same reasoning as before (scaling the codebook also scales the median transmit gain).
Again, we show only transmit-side coverage for space considerations, though receive-side is observed to be nearly identical.
First, we can see that appreciable gains can be had by increasing $\bitsphase = \bitsamp$, particularly when more coverage loss is tolerated, for both channel types.

For the Rayleigh channel in \figref{fig:ironman-a}, we can see that maintaining a slope of $2$ can be achieved with $\bitsphase = \bitsamp \geq 7$ bits (particularly $\bitsamp$) and nearly so with $6$ bits.
This relationship of median transmit gain versus $E$ provide useful insights.
If a system requires a certain level of $E$ to reliably operate in a full-duplex fashion, we can see that our design can do so while offering much higher median transmit gain (and likewise receive gain).
For example, if $E = 20$ dB is required, our design achieves this while supplying median transmit gain of around $31$ dB while convention codebooks only offer around $26$ dB.
As the level of required $E$ decreases, the gap grows significantly until our design meets the ``$2$-slope'' or ``sub-$2$-slope'' regions.
If $E$ is required to be below $10$ dB, we can see that the transmit gain costs are quite high when $\bitsphase = \bitsamp = 5$ bits.
In such cases, we can see that it would be attractive to use $\bitsphase = \bitsamp \geq 6$ bits to preserve transmit gain.

Looking now at the spherical-wave channel in \figref{fig:ironman-b}, we can see that our design sees significant reduction in $E$ at the cost of transmit gain.
Notice that the $x$ and $y$ scales here are different than in in \figref{fig:ironman-a} and indicate that much more reduction in $E$ can be achieved and at less median transmit gain cost.
Again, higher resolution phase shifters and attenuators offer appreciable performance improvements, but the designs do not seem to reach a steady $2$-slope region.
This is likely due to any given design taking advantage of most (if not all) of the attenuators' dynamic range, meaning the cannot be merely scaled down indefinitely.
This does not seem to really be an issue because operation because our design severely outperforms conventional codebooks for practical requirements on median $\Gtx^2(\theta)$.

This leads us to another way to use this plot.
By defining a minimum median $\Gtx^2(\theta)$, we can observe the level of $E$ that our design can provide versus conventional codebooks.
For example, if $32$ dB of median transmit gain is required, our design can achieve more than $30$ dB of improvement in $E$ versus conventional codebooks.
The gap is even more substantial if $30$ dB of median transmit gain is tolerable and we have $\bitsphase = \bitsamp \geq 6$ bits.
We can see that higher resolution phase shifters and attenuators are only justified if the median transmit gain is less than $32$--$33$ dB.

%\begin{figure*}
%    \centering
%    \subfloat[Rayleigh.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v08/generate_v08_process_v01_fig_11}\label{fig:ironman-a}}
%    \quad
%    \subfloat[Spherical-wave channel.]{\includegraphics[width=0.48\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_10}}
%    \caption{The median transmit gain $\Gtx^2\parens{\theta}$ versus average coupling $E$ that our transmit codebook achieves over combinations of $\sigmatx^2 = \sigmarx^2$ and $\Deltatx^2 = \Deltarx^2$ for various $\bitsphase = \bitsamp$.}
%    \label{fig:ironman}
%\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_10}
    \caption{The median transmit gain $\Gtx^2\parens{\theta}$ versus average coupling $E$ that our transmit codebook achieves over combinations of $\sigmatx^2 = \sigmarx^2$ and $\Deltatx^2 = \Deltarx^2$ for various $\bitsphase = \bitsamp$.}
    \label{fig:ironman-b}
\end{figure}



==> sec-simulation-results.tex <==
\section{Numerical Results} % \label{sec:simulation-results}

% \subsection{Simulation}
To assess our design in a variety of conditions, we simulated it in a Monte Carlo fashion.
We used $8 \times 8$ half-wavelength \upas for transmission and reception at our full-duplex transceiver.
Our default transmit and receive coverage regions are comprised of uniformly spaced points in azimuth from $-60^\circ$ to $60^\circ$ with $15^\circ$ spacing and in elevation from $-30^\circ$ to $30^\circ$ with $15^\circ$ spacing.
This amounts to a total of $\Mtx = \Mrx = 9 \times 5 = 45$ total directions in $\dirtxset$ and in $\dirrxset$.
\figref{fig:dirset} illustrates this.

The choice of a particular self-interference channel model is a difficult one to practically justify given there lacks a well-accepted, measurement-backed model.
Other \mmwave full-duplex work has relied on a highly idealized spherical-wave model to capture near-field coupling between antennas and extensions that incorporate sparse reflections from the environment.
In this work, we have chosen to use a Rayleigh-faded channel described as $\entry{\mH}{m,n} \sim \distcgauss{0}{1}$ to prevent these numerical results from being dominated by any spatial structure that may be inherent to other models (which themselves may be highly tied to a choice of relative transmit and receive array geometry).
Other models may see performance improvement or degradation compared to the results shown herein; more relevant channel models can be used in future work to potentially modify and evaluate our design.



%\begin{figure}
%	\centering
%	\subfloat[Azimuth cut.]{\includegraphics[width=0.47\linewidth]{fig/placeholder}
%		\label{fig:codebook-azimuth}}
%	\quad
%	\subfloat[Elevation cut.]{\includegraphics[width=0.47\linewidth]{fig/placeholder}
%		\label{fig:codebook-elevation}}
%	\caption{Azimuth and elevation cuts of an example codebook produced by our design.}
%	\label{fig:codebook}
%\end{figure}



\subsection{Key Metrics and Baselines}

\subsubsection{Off-The-Shelf Codebook Benchmarks}
We evaluate our codebook design against the following three conventional codebooks:
\begin{itemize}
	\item conjugate beamforming (CBF)
	\item conjugate beamforming with Taylor windowing for $20$ dB of side lobe attenuation (CBF-20)
	\item conjugate beamforming with Taylor windowing for $40$ dB of side lobe attenuation (CBF-40)
\end{itemize}
These array pattern of a broadside beam from each of these three codebooks can be seen in \figref{fig:benchmarks}.
When considering tolerated transmit and receive losses $\Deltatx^2$ and $\Deltarx^2$, we account for the trivial approach of merely scaling down these conventional codebooks accordingly.
For instance, if $\Deltatx^2 = \Deltarx^2$ are reduced from $0$ dB to $-3$ dB, one would expect the average coupling $E$ of conventional codebooks to reduce by $-3 + -3 = -6$ dB since transmission and reception are each reduced.
% This can be clearly seen from the dashed lines in \figref{fig:E-vs-delta-for-various-sigma}.

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.3\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_01}
%	\caption{The azimuth cut of a broadside beam from each of our three benchmark codebooks. Given our symmetric \upas, the azimuth and elevation cuts are identical.}
%	\label{fig:benchmarks-old}
%\end{figure}


\subsubsection{Coverage Metric}
Our codebook design is based on discretizing the service region into $\Mtx$ or $\Mrx$ directions.
However, to gain an understanding of a codebook's service to users in \textit{any} direction in the entire service region, we evaluate the gain offered in $N \gg \Mtx, \Mrx$ equally spaced directions.
The beam offering the maximum gain in each of the $N$ directions can be used to compute the average beamforming gain across the entire region.
Explicitly, the gain that our codebook offers in a particular direction $\theta$ can be written simply as
\begin{align}
\Gtx^2\parens{\theta} &= \max_{i} \bars{\entry{\atx{\theta}\ctrans\precbmat}{i}}^2 \\
\Grx^2\parens{\theta} &= \max_{j} \bars{\entry{\arx{\theta}\ctrans\comcbmat}{j}}^2
\end{align}
which is achieved by choosing the beam from our codebook that offers the maximum gain.
%The mean transmit and receive gains across entire service region can be approximated by effectively numerically integrating over the service region with $N$ points via
%\begin{align}
%\mathrm{mean}\parens{\Gtx^2} = \frac{1}{N} \sum_{n=1}^{N} \Gtx^2\parens{\theta\idx{n}} \\
%\mathrm{mean}\parens{\Grx^2} = \frac{1}{N} \sum_{n=1}^{N} \Grx^2\parens{\theta\idx{n}}
%\end{align}


% \subsection{Analysis \#1: Varying $\Deltatx$, $\Deltarx$, $\sigmatx^2$, and $\sigmarx^2$.}

\subsection{Summary of Our Codebook Design's Performance}
We begin examining our numerical results by investigating the impact our design parameters $\Deltatx^2$, $\Deltarx^2$, $\sigmatx^2$, and $\sigmarx^2$ have on average beam coupling $E$.
To do so, we varied $\Deltatx^2 = \Deltarx^2$ from $0$ dB to $-12$ dB and varied $\sigmatx^2 = \sigmarx^2$ from $-30$ dB to $-10$ dB.
We initially set the phase shifter and attenuator resolution to $\bitsphase = \bitsamp = 5$ bits and assumed log-stepped attenuators with $-0.25$ dB of power attenuation per \gls{lsb}.

The results of this are shown in \figref{fig:E-vs-delta-for-various-sigma-bits-a}.
Firstly, we highlight that our conventional codebooks, shown as dashed lines, offer varying degrees of $E$.
CBF yields the most coupling $E$ while CBF+Tay-20 and CBF+Tay-40 show about $4$ dB and $7$ dB improvement, respectively.
By simply scaling these conventional codebooks according to the allotted $\Deltatx^2$ and $\Deltarx^2$, the level of coupling $E$ decreases by a factor of $\Deltatx^2 \times \Deltarx^2$.
Thus, the conventional codebooks see a slope of $2$ dB increase in $E$ per $1$ dB increase in $\Deltatx^2 = \Deltarx^2$.

With our codebook design, we can see appreciable improvements over conventional codebooks, especially on the range $\Deltatx^2, \Deltarx^2 \geq -6$ dB.
At $\Deltatx^2 = \Deltarx^2 = -3$ dB, for instance, we can see approximately $5$ to $15$ dB of improvement over CBF+Tay-40.
Across choices of $\sigmatx^2 = \sigmarx^2$, we see more self-interference mitigation can be achieved with higher variance as expected.
This can be attributed to the fact that more flexibility is offered to our design, allowing $\precbmat$ and $\comcbmat$ to more creatively play with the shape of their beams to reduce coupling with the matrix $\mH$.
This higher variance comes at a cost of lower beam gain and less uniformity in beam gain across the codebook.
We explore this later.

It is clear that---for any $\sigmatx^2 = \sigmarx^2$---there are two regions for our design, as further decreasing $\Deltatx^2 = \Deltarx^2$ shows diminishing returns.
Consider $\sigmatx^2 = \sigmarx^2 = 20$ dB.
The two design regions are
\begin{enumerate}
	\item $\Deltatx^2 = \Deltarx^2 \geq -4$ dB: We see around $4$--$5$ dB of decrease in $E$ for each dB of decrease in $\Deltatx^2 = \Deltarx^2$. This is over twice the rate of return offered by merely scaling down the conventional codebooks.
	\item $\Deltatx^2 = \Deltarx^2 < -4$ dB: We observe that the returns have starkly diminished, offering less than one dB of decrease in $E$ for each dB of decrease in $\Deltatx^2 = \Deltarx^2$.
\end{enumerate}
The first region sees promising performance gains thanks to the degrees of freedom that are made available when decreasing $\Deltatx^2 = \Deltarx^2$ from $0$ dB, which are free to tackle self-interference rather than fighting for beamforming gain.
To explain the second design region, we need to examine \figref{fig:E-vs-delta-for-various-sigma-bits-b}, which fixes $\sigmatx^2 = \sigmarx^2 = -20$ dB and varies $\bitsphase$ and $\bitsamp$.
We see immediately that having only $3$ bits of either phase or amplitude control is not fruitful here, especially when $\Deltatx^2 = \Deltarx^2 \leq -3$ dB.

At the very least, one would expect the second region to scale with a slope of $2$, the same slope as our conventional codebooks, since we could merely scale down the codebook design from the first design region indefinitely.
Such would maintain a constant gap between the conventional codebooks as $\Deltatx^2 = \Deltarx^2$ are decreased indefinitely.
This is not the case, however, due to limited amplitude control.
Our attenuators have a limited dynamic range, meaning they cannot scale down a design indefinitely, causing a sort of floor to be reached.
As shown in \figref{fig:E-vs-delta-for-various-sigma-bits-b}, higher resolution attenuators ($\bitsamp = 8$ bits) offer a higher dynamic range and maintain this scaling (though a floor would eventually be hit beyond $\Deltatx^2 = \Deltarx^2 \leq -12$ dB).
Note that the optional variable attenuator shown in our system model in \figref{fig:system} could be used to widen the effective dynamic range of our attenuators.

Notice that the knee at which region one transitions to region two is largely based on the phase shifter resolution $\bitsphase$.
Considering \figref{fig:E-vs-delta-for-various-sigma-bits-a}, we can see that the knee also depends on $\sigmatx^2 = \sigmarx^2$: higher variance shifts the knee to the right.
It is worth noting that having $\bitsphase = 5$ bits versus $\bitsphase = 8$ does not make significant difference in this case except when $\Deltatx^2 = \Deltarx^2 \leq -5$ dB.
Clearly, with $\bitsphase = \bitsamp = 8$, we see significant improvement in this region.
For most of this analysis henceforth, we assume a reasonable $\bitsphase = \bitsamp = 5$ bits with the understanding that higher resolution phase shifters and attenuators can significantly benefit our design, depending on our choice of design parameters.


% only makes significant difference here when $\Deltatx^2 = \Deltarx^2 \leq -5$ dB.

% For each dB afforded in $\Deltatx^2 = \Deltarx^2$, we can see nearly twice the rate of reduction in $E$ versus the conventional codebooks.
% This is because the degrees of freedom made available when decreasing $\Deltatx^2$ and $\Deltarx^2$ can be used to mitigate self-interference rather than for beamforming gain.



% When $\Deltatx^2, \Deltarx^2 \leq -6$ dB, we can see the gains in reducing $E$ diminish severely.
% One would expect the return on $E$ per dB in $\Deltatx^2 = \Deltarx^2$ to have a slope of two as with the o conventional codebooks since the trivial approach is to scale the beams down to reduce coupling.
% The reason we do not see such in our design is due to a floor caused by limited amplitude control, preventing us from scaling down our design indefinitely.\footnote{An additional variable attenuator before the transmit beamformer and one after the receive beamformer could be used to scale a beam design up or down.}
% This can be validated by \figref{fig:E-vs-delta-for-various-sigma-bits-b}, where we fix $\sigmatx^2 = \sigmarx^2 = -20$ dB and vary $\bitsphase$ and $\bitsamp$.
% The conventional codebooks shown are with $\bitsphase = \bitsamp = 8$ bits.
% The magenta lines have $\bitsamp = 3$ bits, the orange lines have $\bitsamp = 5$ bits, and the green lines have $\bitsamp = 8$ bits.
% The green lines with $\bitsamp = 8$ bits clearly can sustain the $2$ dB slope thanks to their wider dynamic range.
% It can be seen that $\bitsamp \leq 3$ bits is not sufficient and that $\bitsphase \leq 3$ is also not sufficient for appreciable performance.
% Increasing to $\bitsphase = \bitsamp = 5$ bits creates a regime where our design can begin offering significantly more isolation versus the conventional codebooks.
% Maintaining this gap is not sustainable with only $\bitsamp = 5$ bits due to its limited dynamic range as previously described.
% With $\bitsamp = 8$ bits, we can maintain the gap (to at least $\Deltatx^2 = \Deltarx^2 = -12$ dB). 
% At $\bitsphase = \bitsamp = 8$ bits, a dramatic increase can be seen below $\Deltatx^2 = \Deltarx^2 = -4$ dB.
% This is thanks to the fine phase granularity provided with $8$ bits.
% A gap of around $13$ dB can be seen versus only $\bitsphase = 5$ bits below $\Deltatx^2 = \Deltarx^2 = -7$ dB.

\begin{figure*}
	\centering
	\subfloat[$\bitsphase = \bitsamp = 5$ bits.]{\includegraphics[width=0.48\linewidth]{plots/v01/generate_v01_process_v01_fig_03}\label{fig:E-vs-delta-for-various-sigma-bits-a}}
	\quad
	\subfloat[$\sigmatx^2 = \sigmarx^2 = -20$ dB.]{\includegraphics[width=0.48\linewidth]{plots/v07/generate_v07_process_v01_fig_03}\label{fig:E-vs-delta-for-various-sigma-bits-b}}
	\caption{Average beam coupling $E$ versus $\Deltatx^2 = \Deltarx^2$. In (b), the conventional codebooks are shown with $\bitsphase = \bitsamp = 8$.}
	\label{fig:E-vs-delta-for-various-sigma-bits}
\end{figure*}

% \edit{Include half-duplex performance, distribution.}

% \edit{Include coverage plots.}

% -----------------------------------------------------------------------------------------------------------

\subsection{Are Our Codebooks Still Useful?}
We have shown that some choices of design parameters can significantly lessen the average coupling seen across beam pairs in our codebooks.
It is essential that we evaluate if our designs are in fact useful in providing coverage to our service region.
To do this, we begin by plotting the azimuth and elevation cuts of our transmit codebooks for various $\sigmatx^2$ when $\Deltatx^2 = 0$ dB in \figref{fig:az-el-cuts-ours}; each design used the same channel realization $\mH$.
The power of our design clearly lay in its use of side lobes to strategically mitigate self-interference.
This is a dramatically different approach than taken by the Taylor-windowed conventional codebooks, which blindly reduce side lobes; of course, conventional codebooks are not designed to reduce self-interference and are channel agnostic.
Our codebook's beams maintain fairly sharp beams with high gain, showing promise that they are in fact useful for delivering service to users.

With increased $\sigmatx^2$, we can see that the design takes advantage of the allotted variance by shrinking the gain of the main lobes and more creatively shaping its side lobes.
This is thanks to the degrees of freedom provided with more variance and can be explained simply.
With more variance tolerated, the beams need not strictly use their degrees of freedom to meet the target gain with little margin for error but can rather use them to shape their beams to reduce self-interference.

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_02.eps}
	\caption{Azimuth and elevation cuts of an example codebook produced by our design, where $\Deltatx^2 = \Deltarx^2 = 0$ dB.}
	\label{fig:az-el-cuts-ours}
\end{figure*}

%\begin{figure*}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_08.eps}
%	\caption{Azimuth cuts of the benchmark codebooks and example codebooks produced by our design, where $\Deltatx^2 = \Deltarx^2 = 0$ dB.}
%	\label{fig:}
%\end{figure*}

Having verified the beams making up our codebooks, we now look at quantifying the coverage of our design.
It is important that our design not leave significant portions of the service region without high gain.
To visualize the service provided over this region, we plot the gain delivered by our conventional codebooks versus our transmit codebook for various $\sigmatx^2$ when $\Deltatx^2 = 0$ dB in \figref{fig:coverage-space}.
The conventional codebooks have beams uniformly spread out of the service region in azimuth and elevation. 
CBF achieves full beamforming gain and those Taylor-windowed have reduced main lobe gain (around $2$--$3$ dB each) as shown prior in \figref{fig:benchmarks}.

Our design packs its beams across the service region to achieve the $\Mtx$ and $\Mrx$ coverage requirements explicitly accounted for in our design.
Other directions not included in $\dirtxset$ and $\dirrxset$ have the potential of not being served with certain gain.
As evidenced by \figref{fig:coverage-space}, some small gaps can be seen in our design.
Most gaps are on the order of those seen in the conventional codebooks.
A few slightly larger holes in coverage are apparent with our design.

%\begin{figure*}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_07.eps}
%	\caption{For a given channel realization, the gain offered by our transmit codebook design across the $\dirtxset$, shown here as its projection onto the $y$-$z$ plane, where $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits. Brightest yellow corresponds to $33$ dB and darkest blue corresponds to $20$ dB.}
%	\label{fig:coverage-space}
%\end{figure*}

To more accurately compare coverage of our design versus conventional codebooks, we plot their empirical \glspl{cdf} in \figref{fig:coverage-cdf}.
From here, it is clear that our design covers the service region on par with the conventional codebooks, other than the heavier left tails.
With $\sigmatx^2 \leq -15$ dB, our design provides coverage better than CBF+Tay-20 and CBF+Tay-40.
Even $\sigmatx^2 = -10$ dB outperforms CBF+Tay-40.
The holes in coverage can be seen as carrying very little weight in the \glspl{cdf} of \figref{fig:coverage-cdf}.
Aside from this, we can see the shape of the coverage \glspl{cdf} of our design closely resemble that of the conventional codebooks.

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_04}
%	\caption{The \glspl{cdf} of the coverage provided by our transmit codebook design (for a given channel realization) for various $\sigmatx^2 = \sigmarx^2$ compared to conventional codebooks, where $\Deltatx^2 = \Deltarx^2 = -3$ dB.}
%	\label{fig:coverage-cdf}
%\end{figure}


Still, it can be difficult to see how our design trades off reducing $E$ at the cost of coverage.
To better understand such, we use \figref{fig:E-vs-coverage}, which plots median coverage ($50$-th percentile of the coverage \glspl{cdf}) versus $E$. 
We can see that our design, shown as scatter points, does a much better job trading off coverage for reduction in $E$. 
This was somewhat expected and familiar from \figref{fig:E-vs-delta-for-various-sigma-bits-a} since reducing $\Deltatx^2$ and $\Deltarx^2$ will lead to reduced coverage.
From this, we can also see the design parameters that should be used for a desired level of $E$ or a desired median coverage.
Notice that this plot can be used for either mapping desired $E$ to median coverage or for mapping median coverage to $E$.

If we desire $E = 15$ dB, for example, we can see that our conventional codebooks would achieve around $24$ dB of median transmit gain.
Our design can achieve $E = 15$ dB with $30$ dB of median transmit gain.
You can see the gap is the largest at around $E = 10$ dB, offering over $8$ dB more transmit gain with our design.
If we desire a median transmit gain of $30$ dB, our design offers around $12$ dB lower $E$ than conventional codebooks.
The gap is widest at a median transmit gain of around $29$ dB, offering $15$ dB lower $E$.
For \textit{any} choice of $E$ and median transmit gain, our design does better than the conventional codebooks in delivering coverage while mitigating self-interference.

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v01/generate_v01_process_v01_fig_05}
%	\caption{Median transmit coverage versus median $E$.}
%	\label{fig:E-vs-coverage}
%\end{figure}


%\subsection{Analysis \#2: Varying $\bitsphase$ and $\bitsamp$.}
%To investigate the effect that limited phase and amplitude control have on our design, we evaluated it under a variety of $\bitsphase$-$\bitsamp$ pairs.
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v02/generate_v02_process_v01_fig_03}
%	\caption{Mean $E$ for various $\bitsphase$ and $\bitsamp$.}
%	\label{fig:}
%\end{figure}

\subsection{Varying Codebook Size $\Mtx$ and $\Mrx$}
One can imagine that the size of the codebooks, $\Mtx$ and $\Mrx$, can have significant impact on our design, considering it was clearly avoiding some portions of space as evident in \figref{fig:coverage-space}.
As a simple analysis, we varied the spacing of the $\dirtx\idx{i}$ and $\dirrx\idx{j}$ to adjust $\Mtx$ and $\Mrx$, preserving the service region spanning from $\pm60^\circ$ in azimuth and $\pm30^\circ$ in elevation.
We fixed $\Deltatx^2 = \Deltarx^2 = -3$ dB and $\bitsphase = \bitsamp = 5$ bits.
The results shown in \figref{fig:E-vs-Mtx-Mrx} verify that as $\Mtx = \Mrx$ increases, our design has difficulty reducing $E$; recall our previous numerical results had $\Mtx = \Mrx = 45$.
Having so many beams packed within the service region and requiring our codebooks to serve the region with more granularity, it is difficult to avoid coupling self-interference.
In other words, it is difficult to sufficiently span the spatial components of $\Atx$ and $\Arx$ with $\precbmat$ and $\comcbmat$ while desiring they live in the null spaces of $\comcbmat\ctrans \mH$ and $\mH \precbmat$, respectively.
Several dB in $E$ can be bought by reducing the codebooks from $45$ beams to $29$ beams, though this would likely be too sparse of coverage for practice.
Notice that the conventional codebooks offer an approximately fixed average coupling $E$ regardless of codebook sizes $\Mtx$, $\Mrx$.
With too many beams, one can ensure users see higher gain across the service region, though this is undesirable in regards to memory and beam alignment.
Of course, with too few beams, one would need to widen them appropriately to cover the service region, sacrificing gain.
$\Mtx = \Mrx = 45$ beams seems to be fairly balanced in its ability to deliver coverage and reduce $E$.

\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v05/generate_v05_process_v01_fig_01}
	\caption{$E$ as a function of $\Mtx$ and $\Mrx$ for various $\sigmatx^2$, $\sigmarx^2$ where $\Deltatx^2 = \Deltarx^2 = -3$ dB.}
	\label{fig:E-vs-Mtx-Mrx}
\end{figure}

\subsection{Impacts of Channel Estimation Error}
All of the results thus far have been under perfect channel knowledge ($\epsilon = 0$).
In this section, we consider $\epsilon > 0$ to investigate our design's performance under imperfect channel knowledge.
We denote $\epsilon_{\mathrm{trn}}$ as the value of $\epsilon$ used during design and $\epsilon_{\mathrm{eval}}$ as the value of epsilon used during evaluation (i.e., when manufacturing the error term $\mDelta$).
\figref{fig:E-vs-eps-eval-various-eps-trn} showcases our design's ability to reduce $E$ in the face of error $\mDelta : \normfro{\mDelta}^2 = \epsilon_{\mathrm{eval}}^2 \cdot \Nt \Nr$ when designed using various $\epsilon_{\mathrm{trn}}^2$.

Let us first look at \figref{fig:E-vs-eps-eval-various-eps-trn-20} where we have fixed $\Deltatx^2 = \Deltarx^2 = -3$ dB, $\sigmatx^2 = \sigmarx^2 = -20$ dB, and $\bitsphase = \bitsamp = 5$ bits.
As expected, when the actual channel error $\epsilon_{\mathrm{eval}}^2$ is low and the channel error on which the codebooks were design $\epsilon_{\mathrm{trn}}^2$ is low, performance is best, offering the lowest $E$.
Fixing $\epsilon_{\mathrm{eval}} = -30$ dB, we can see that increasing $\epsilon_{\mathrm{trn}}$ forces the design to sacrifice reduction in $E$ as it attempts to be robust to channel error.
Recall that our design was a worst-case approach, meaning the $E$-optimal $\epsilon_{\mathrm{trn}}$ will likely be less than $\epsilon_{\mathrm{eval}}$ on average.
Notice that $\epsilon_{\mathrm{trn}} = -30$ dB is the best choice for $\epsilon_{\mathrm{eval}} \leq -10$ dB.
From $-10 \geq \epsilon_{\mathrm{eval}} \geq -3$ dB, $\epsilon_{\mathrm{trn}} = -20$ dB is best.
Beyond this, $\epsilon_{\mathrm{trn}} = -10$ is the best choice.

In \figref{fig:E-vs-eps-eval-various-eps-trn-10}, we have instead used $\sigmatx^2 = \sigmarx^2 = -10$ dB.
We can immediately see that our design benefits from more variance when 

\begin{figure*}
	\centering
	\subfloat[$\sigmatx^2 = \sigmarx^2 = -30$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_03_-30}\label{fig:E-vs-eps-eval-various-eps-trn-20}}
	\quad
	\subfloat[$\sigmatx^2 = \sigmarx^2 = -20$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_03_-20}\label{fig:E-vs-eps-eval-various-eps-trn-20}}
	\\ \vspace{0.25cm}
	\subfloat[$\sigmatx^2 = \sigmarx^2 = -10$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_03_-10}\label{fig:E-vs-eps-eval-various-eps-trn-10}}
	\caption{Average coupling $E$ as a function of Frobenius channel error $\epsilon_{\mathrm{eval}}$ when designed on various $\epsilon_{\mathrm{trn}}$.}
	\label{fig:E-vs-eps-eval-various-eps-trn}
\end{figure*}


%\begin{figure*}
%	\centering
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -3$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_04_-15}\label{fig:E-vs-eps-eval-various-eps-trn-20}}
%	\quad
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -5$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_04_-25}\label{fig:E-vs-eps-eval-various-eps-trn-20}}
%	\\ \vspace{0.25cm}
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -7$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_04_-35}\label{fig:E-vs-eps-eval-various-eps-trn-10}}
%	\caption{Average coupling $E$ as a function of Frobenius channel error $\epsilon_{\mathrm{eval}}$ when designed on various $\epsilon_{\mathrm{trn}}$.}
%	\label{fig:E-vs-eps-eval-various-eps-trn}
%\end{figure*}

%\begin{figure*}
%	\centering
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -3$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_04_-15}\label{fig:E-vs-eps-eval-various-eps-trn-20}}
%	\quad
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -5$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_04_-25}\label{fig:E-vs-eps-eval-various-eps-trn-20}}
%	\\ \vspace{0.25cm}
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -7$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_04_-35}\label{fig:E-vs-eps-eval-various-eps-trn-10}}
%	\caption{Average coupling $E$ as a function of Frobenius channel error $\epsilon_{\mathrm{eval}}$ when designed on various $\epsilon_{\mathrm{trn}}$.}
%	\label{fig:E-vs-eps-eval-various-eps-trn}
%\end{figure*}
%
%
%\begin{figure*}
%	\centering
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -3$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_06_1-1}\label{fig:}}
%	\quad
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -5$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_06_2-1}\label{fig:}}
%	\\ \vspace{0.25cm}
%	\subfloat[$\Deltatx^2 = \Deltarx^2 = -7$ dB]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_06_3-1}\label{fig:}}
%	\caption{}
%	\label{fig:}
%\end{figure*}
%
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v12/generate_v12_process_v01_fig_07}\label{fig:E-vs-eps-eval-various-eps-trn-10}
%	\caption{Caption.}
%	\label{fig:}
%\end{figure}


%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v21/generate_v21_process_v01_fig_10}
%	\caption{Spherical-wave channel, arrays separated in azimuth.}
%	\label{fig:}
%\end{figure}

What we've learned:
\begin{itemize}
	\item our robust approach can resist the impacts of channel estimation error by appropriately choosing $\epsilon_{\mathrm{trn}}$; we can buy over $5$ dB of $E$ at error of $-10$ dB.
	\item channel uncertainty is a difficult task; we can't expect our design to do well if it doesn't know the SI channel
	\item we hope for a relatively static or slowly changing channel and that system calibration following installation can provide us a solid channel estimate; infrequent and high quality channel estimation (e.g., when the system usage is low) can drastically improve our design
	\item it is important to properly choose $\epsilon_{\mathrm{trn}}$, which can be chosen using the distribution of channel errors, for example, to avoid producing an overly-robust worst-case design
	\item decreasing $\Deltatx^2 = \Deltarx^2$ a little will give our design more flexibility and headroom versus conventional codebooks
\end{itemize}


\subsection{Summary of Key Takeaways and Findings}

% \subsection{Extra}

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v10/generate_v10_process_v01_fig_03_-10}
%	\caption{Caption.}
%	\label{fig:}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v10/generate_v10_process_v01_fig_03_-20}
%	\caption{Caption.}
%	\label{fig:}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=\textheight,keepaspectratio]{plots/v10/generate_v10_process_v01_fig_03_-30}
%	\caption{Caption.}
%	\label{fig:}
%\end{figure}

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v02/generate_v02_process_v01_fig_01}
%	\caption{Caption.}
%	\label{fig:}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth,height=0.4\textheight,keepaspectratio]{plots/v02/generate_v02_process_v01_fig_02}
%	\caption{Caption.}
%	\label{fig:}
%\end{figure}

==> sec-system-model-v2.tex <==
\section{System Model} \label{sec:system-model}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth,height=0.35\textheight,keepaspectratio]{fig/codebook_system_type_01}
	\caption{Block diagram of our full-duplex \mmwave transceiver with separate transmit and receive arrays.}
	\label{fig:system}
\end{figure}

In this work, we consider an in-band full-duplex \mmwave transceiver that employs separate, independently controlled arrays for transmission and reception.
Let $\Nt$ and $\Nr$ be the number of transmit and receive antennas, respectively, at the arrays of the full-duplex transceiver.
The transmit and receive array response vectors in the direction $\dir$ we denote as $\atx{\dir} \in \setvectorcomplex{\Nt}$ and $\arx{\dir} \in \setvectorcomplex{\Nr}$, respectively.
These array response vectors for arbitrary $\dir$ can be computed based on the transmit and receive array geometries.
We use the convention that our array response vectors are normalized such that $\normtwo{\atx{\dir}}^2 = \Nt$ and $\normtwo{\arx{\dir}}^2 = \Nr$.

For simplicity, we consider an analog-only beamforming system, though the codebook design herein can also be used by hybrid digital/analog beamforming systems.
Let $\vf \in \setvectorcomplex{\Nt}$ be the analog precoding vector used at the transmitter.
Let $\vw \in \setvectorcomplex{\Nr}$ be the analog combining vector used at the receiver.
Analog beamforming is implemented in hardware where a network of phase shifters and attenuators are used to realize a desired beamformer.
We consider the practical case where these phase shifters and attenuators are digitally-controlled.
Let $\bitsphase$ and $\bitsamp$ be the number of bits used to configure each phase shifter and attenuator in the transmit and receive beamforming networks, respectively.
In this work, we assume the set of all $2^\bitsphase$ possible phase shifter settings are uniformly distributed over the phase range $[0,2\pi)$ radians. 

Since transmit and receive beamforming networks are power-constrained \textit{per-antenna} (rather than enjoying an $\ell_2$-based \textit{total} power constraint), we enforce
\begin{gather}
\bars{\entry{\vf}{m}} \leq 1 \ \forall \ m = 1, \dots, \Nt \\
\bars{\entry{\vw}{n}} \leq 1 \ \forall \ n = 1, \dots, \Nr
\end{gather}
which can be understood by the fact that attenuators are used to implement amplitude control.
Consequently, we can see that $\normtwo{\vf}^2 \leq \Nt$ and $\normtwo{\vw}^2 \leq \Nr$.
With this being said, we assume the set of all $2^\bitsamp$ possible attenuator settings are either linearly or logarithmically distributed over the linear magnitude range $(0,1]$.
For example, it is common for digitally-stepped attenuators used in phased arrays to have a \gls{lsb} step size of $-0.25$ or $-0.5$ dB.
When amplitude control is not present, we can let $\bitsamp = 0$.
Capturing limited phase and amplitude control, let $\precb \subset \setvectorcomplex{\Nt}$ and $\comcb \subset \setvectorcomplex{\Nr}$ be the sets of all possible beamforming vectors $\vf$ and $\vw$, respectively; hence, $\vf \in \precb$ and $\vw \in \comcb$.
Note that the sets $\precb$ and $\comcb$ are equivalent when $\Nt = \Nr$ since we have assumed the same phase shifters and attenuators are used at both.



Since transmission and reception happen simultaneously and in-band, a self-interference channel $\mH \in \setmatrixcomplex{\Nr}{\Nt}$ manifests between the transmit and receive arrays of the full-duplex transceiver.
It is difficult to reliably assume a characterization or model for $\mH$.
% One may expect near-field coupling to dominate due to the close proximity of the arrays and the fact that reflections from the environment will undergo severe path loss at \mmwave.
At present, there has been little research investigating such a \mmwave self-interference channel, though sensible speculations have been made that assume it to be comprised of a direct coupling between the arrays along with reflections off of the environment.
This has, in fact, been the basis for a number of existing works on \mmwave full-duplex.
The highly idealized near-field model used therein, however, will likely not be present in practice due to the backplates, casings, enclosures, and infrastructure associated with actual arrays.
% Still, it is difficult to speculate what the channel will be comprised of since 
% The close proximity between the transmit array and receive array make it difficult to characterize $\mH$.
% At present, there has been little research investigating such a channel, though sensible speculations have been made that assume it to be comprised of a direct coupling between the arrays along with reflections off of the environment.
Given that a model has not yet been verified with measurements, we do not present a design based on a particular structure or assumption of $\mH$.
% We do, however, use the aforementioned channel model and others for $\mH$ to assess our design in \secref{sec:simulation-results} to evaluate how our approach generalizes across different types of self-interference channels.

% Let us assume that the channel matrix $\Hsi$ remains stationary across service to many users.

A transmitted symbol $s$ from the full-duplex transceiver will be injected into the self-interference channel $\mH$ by its transmit beam $\vf$ and transmit power gain $\Ptx$ then subsequently combined by its receive beam $\vw$.
To abstract out the large-scale gain of the self-interference channel and its spatial characteristics, we impose
\begin{align}
\ev{\normfro{\mH}^2} = \Nt \cdot \Nr
\end{align}
letting $G$ handle proper scaling of $\mH$ based on the isolation between the arrays.
The received self-interference $y$ can thus be written as
\begin{align}
y = \sqrt{\Ptx} \cdot G \cdot \vw\ctrans \mH \vf s 
\end{align}
It can be readily seen that decreasing the large-scale gain $G$ (increasing isolation) would reduce self-interference as well as strategically steering $\vf$ and $\vw$ according to the channel $\mH$.




==> sec-system-model.tex <==
\section{System Model} \label{sec:system-model}

%\begin{figure}[!t]
%	\centering
%	\subfloat[Analog precoding network.]{\includegraphics[width=0.8\linewidth,height=0.2\textheight,keepaspectratio]{fig/hdx_mmwave_analog_precoder_v2}
%		\label{fig:analog-network-a}}
%	% \quad
%	\\
%	\subfloat[Analog combining network.]{\includegraphics[width=0.8\linewidth,height=0.2\textheight,keepaspectratio]{fig/hdx_mmwave_analog_combiner_v2}
%		\label{fig:analog-network-b}}
%	\caption{Fully-connected analog beamforming connects each \rf chain to each antenna via a phase shifter and possibly attenuator. Each phase shifter is digitally controlled with $\bitsphase$ bits and each attenuator with $\bitsamp$ bits.}
%	\label{fig:analog-network}
%\end{figure}

In this work, we consider an in-band full-duplex \mmwave transceiver that employs separate, independently controlled arrays for transmission and reception.
We assume hybrid precoding and combining take place at the transmitter and receiver, where the case of analog-only beamforming takes place when a single \rf chain is used.
Let $\Lt$ and $\Lr$ be the number of \rf chains at the transmitter and receiver, respectively.
Let $\Nt$ and $\Nr$ be the number of transmit antennas and receive antennas, respectively.

Let $\prerf \in \setmatrixcomplex{\Nt}{\Lt}$ be the analog precoding matrix used at the transmitter.
Let $\comrf \in \setmatrixcomplex{\Nr}{\Lr}$ be the analog combining matrix used at the receiver.
Analog beamforming is implemented in hardware, taking place at \rf, where a network of phase shifters and attenuators are used to realize a desired beamformer.
These phase shifters and attenuators are typically digitally-controlled with finite resolution, constraining which beams can be physically realized.
Let $\bitsphase$ and $\bitsamp$ be the number of bits used to configure each phase shifter and attenuator, respectively.
In this work, we assume the set of all $2^\bitsphase$ possible phase shifter settings are uniformly distributed over the phase range $[0,2\pi)$ radians and assume the set of all $2^\bitsamp$ possible attenuator settings are arbitrarily distributed over the linear amplitude range $(0,1]$.
We will assume, for the sake of simplicity, that the precoder and combiner use the same phase shifters and attenuators and that they're controlled with the same degrees of resolution $\bitsphase$ and $\bitsamp$.

Capturing these hardware constraints, let $\prerfcb$ and $\comrfcb$ be the set of all possible beamforming \textit{vectors} comprising $\prerf$ and $\comrf$.
That is,
\begin{gather}
\entry{\prerf}{:,\ell} \in \prerfcb, \ \ell = 1, \dots, \Lt \\
\entry{\comrf}{:,\ell} \in \comrfcb, \ \ell = 1, \dots, \Lr 
\end{gather}

Since transmission and reception happen simultaneously and in-band, a self-interference channel $\Hsi \in \setmatrixcomplex{\Nr}{\Nt}$ manifests between the transmit and receive arrays of the full-duplex transceiver.
The close proximity between the transmit array and receive array make it difficult to characterize $\Hsi$.
At present, there has been little research investigating such a channel, though sensible speculations have been made that assume it to be comprised of a direct coupling between the arrays along with reflections off of the environment.
Given that this model has not yet been verified with measurements, we do not present a design based on a particular structure or assumption of $\Hsi$.
We do, however, use the aforementioned channel model and others for $\Hsi$ to assess our design in \secref{sec:simulation-results} to evaluate how our approach generalizes across different types of self-interference channels.
Let us assume that the channel matrix $\Hsi$ remains stationary across service to many users.


